LLP-Bench: A Large Scale Tabular Benchmark for Learning from Label Proportions

In the task of Learning from Label Proportions (LLP), a model is trained on groups (a.k.a bags) of instances and their corresponding label proportions to predict labels for individual instances. LLP has been applied pre-dominantly on two types of datasets - image and tabular. In image LLP, bags of fixed size are created by randomly sampling instances from an underlying dataset. Bags created via this methodology are called random bags. Experimentation on Image LLP has been mostly on random bags on CIFAR-* and MNIST datasets. Despite being a very crucial task in privacy sensitive applications, tabular LLP does not yet have a open, large scale LLP benchmark. One of the unique properties of tabular LLP is the ability to create feature bags where all the instances in a bag have the same value for a given feature. It has been shown in prior research that feature bags are very common in practical, real world applications [Chen et. al '23, Saket et. al. '22]. In this paper, we address the lack of a open, large scale tabular benchmark. First we propose LLP-Bench, a suite of 70 LLP datasets (62 feature bag and 8 random bag datasets) created from the Criteo CTR prediction and the Criteo Sponsored Search Conversion Logs datasets, the former a classification and the latter a regression dataset. These LLP datasets represent diverse ways in which bags can be constructed from underlying tabular data. To the best of our knowledge, LLP-Bench is the first large scale tabular LLP benchmark with an extensive diversity in constituent datasets. Second, we propose four metrics that characterize and quantify the hardness of a LLP dataset. Using these four metrics we present deep analysis of the 62 feature bag datasets in LLP-Bench. Finally we present the performance of 9 SOTA and popular tabular LLP techniques on all the 62 datasets.

==> algo.tex <==
\begin{algorithm}
    \caption{LLP Model Training Procedure}\label{alg:training}
    \KwData{Bags $(B_1, \dots, B_M)$, params. $b, S, R$, bag loss ${\sf L}$.}
    \KwResult{Trained model $\mc{M}$.}
    \For{$r = 1,\dots, R$}{
        (optionally) randomly permute $(B_1, \dots, B_M)$. \\
        \For{$s = 1\dots, S$}{
            Minibatch $\mc{S} = \{B_{(s-1)b+1}, \dots B_{sb}\}$. \\
            Apply $\mc{M}$ on $\mb{X}_B$ to get $\hat{y}_B$, $B \in \mc{S}$. \\
            ${\sf Loss} = \sum_{B\in \mc{S}} {\sf L}(B, y_B, \hat{y}_B)$. \\
            Backpropagate to update weights of $\mc{M}$.
        }     
    }
    Output $\mc{M}$.
\end{algorithm}

==> anomalies_table.tex <==
\begin{table}[]
\scriptsize
\centering
\begin{tabular}{llccclll}
\toprule
\textbf{Col1} & \textbf{Col2} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}\% inst.\\ left\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}No. \\ bags\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Mean\\ bag size\end{tabular}}} & \textbf{Tail Size} & \textbf{\begin{tabular}[c]{@{}l@{}}Stddev\\ Label Prop\end{tabular}} & \textbf{Bag Separation} \\ \midrule
\textit{C1} & \textit{C7} & 37.91 & 55937 & 310.69 & Long-tailed & Very Low & Well-seperated \\
\textit{C1} & \textit{C10} & 32.44 & 55528 & 267.81 & Short-tailed & Very Low & Less-seperated \\
\textit{C2} & \textit{C7} & 48.74 & 78261 & 285.51 & Short-tailed & Low & Well-seperated \\
\textit{C6} & \textit{C7} & 35.84 & 38449 & 427.31 & Very Long-tailed & Very Low & Well-seperated \\
\textit{C7} & \textit{C8} & 33.37 & 45042 & 339.57 & Long-tailed & Very Low & Well-seperated \\
\textit{C7} & \textit{C10} & 40.52 & 56575 & 328.31 & Long-tailed & Very Low & Well-seperated \\
\textit{C10} & \textit{C15} & 44.66 & 102841 & 199.07 & Very Short-tailed & Medium & Medium-seperated \\
\textit{C10} & \textit{C17} & 30.74 & 44463 & 316.96 & Long-tailed & Very Low & Medium-seperated \\
\textit{C10} & \textit{C18} & 42.31 & 90181 & 215.05 & Very Short-tailed & Low & Medium-seperated \\
\textit{C10} & \textit{C26} & 31.38 & 65658 & 219.1 & Very Short-tailed & Medium & Medium-seperated \\ \bottomrule
\end{tabular}
\caption{Characteristics of Anomalous Datasets}
\label{tab:anomalies}
\end{table}

==> bag_distribution_analysis.tex <==
\section{Bag Distribution Analysis} \label{sec:bag_dist_analysis}
\input{table_mean_bag_size_percentile}
\input{table_avg_ll_ranges}
\input{table_ratio_ranges}
\input{table_flagship_groupings}
We perform the bag distribution analysis for all $308$ clipped groupings which contain more than $500$ bags.
\subsection{Characterising the distribution of Bag Sizes}
\label{bag_size_char}
Since we have only have a label proportion for each bag, informally speaking, the larger the bag size the lower the amount of label supervision for that bag. The bag sizes for any grouping are characterized by their cumulative distribution function which plots the fraction of bags of size at most $t$ for all $t \geq 1$. In all the groupings, it is observed that the density of bags drops steeply with the increase in bag size in the histograms of bag sizes. 
Thus, we compute the bag sizes at the $50$, $70$, $85$ and $95$ percentile of cumulative distribution plot, for each grouping.


Hence, we can naturally classify the groupings we obtain into \textit{long-tailed} and \textit{short-tailed} distributions. Short-tailed distributions have most bags of small size and a very few large sized bags whereas Long-tailed distributions contain many bags of large sizes. Bags of large sizes provide a very little label information for a lot of feature level information. Hence, they can be used for learning representations but are less useful in supervised training.\\
In order to classify the groupings created into \textit{long-tailed} and \textit{short-tailed}, we compute the threshold bag sizes at which we attain $50$, $70$, $85$ and $95$ percentile of the bags for each clipped grouping. We normalize these values and obtain $4$-dimensional vectors for each clipped grouping. Applying $k$-Means on these vectors we cluster the clipped groupings into $4$ clusters. As shown in Table \ref{tab:mean_bag_size_percentile}, the mean $t$-percentile bag size, give the same cluster  ordering for $t = 50, 70, 85, 95$. Hence, we name the clusters in increasing order of these mean bag sizes as \textit{Very Short-tailed}, \textit{Short-tailed}, \textit{Long-tailed} and \textit{Very Long-tailed} bag size distributions. Appendix \ref{appendix:bag_size_dist} contains threshold bag sizes and cluster labels based on them for all groupings.

\subsection{Characterising the distribution of Label Sums}
\label{label_prop_char}
We model the distribution of label sums in a grouping as a binomial distribution, with bias as the label proportion of the grouping. We compute for each grouping its $\tn{AvgBagLL}$ value. The higher the value, the closer the grouping is to having randomly distributed label proportions. Refer to Sec. \ref{sec:prelims} for the definitions of $\tn{AvgBagLL}$ and bias of the dataset.\\
We perform $k$-Means on these values and classify our groupings into groupings having \textit{High}, \textit{Medium}, \textit{Low} and \textit{Very Low} $\tn{AvgBagLL}$. The ranges of $\tn{AvgBagLL}$ values for each of these clusters are listed in Table \ref{tab:avg_ll_ranges}. Appendix \ref{appendix:avg_ll_dist} contains the $\tn{AvgBagLL}$ values as well as the clusters labels based on them for all groupings. 
\subsection{Bag separation analysis}
\label{bag_dist_char}
As defined in Sec. \ref{sec:prelims}, higher ${\sf InterIntraRatio}$ indicates bags are clustered. %
First, we obtain an embedding of the feature-vectors by training an instance level AutoInt Model\footnote{80\% instances used for training and rest for validation.} on \textit{Criteo} dataset and extract it's embedding layer using which we transform the instances into this embedding space. We compute the ${\sf InterIntraRatio}$ and other ${\sf BagSep}$ quantities for all $308$ clipped groupings in this embedding space. We then perform $k$-Means on ${\sf InterIntraRatio}$ to classify our groupings into \textit{Less-separated}, \textit{Medium-separated}, \textit{Well-separated} and \textit{Far-separated} bag distributions.\\
The Ranges of ${\sf InterIntraRatio}$ for each of the clusters are listed in Table  \ref{tab:ratio_ranges}. Appendix \ref{appendix:bag_sep_stats} contains the ${\sf BagSep}$ quantities for all the groupings along with the clusters they are classified into. Appendix \ref{appendix:sq_l2_bag_sep} contains simplification of ${\sf BagSep}$ computation with $\ell_2^2$-distance. 

\subsection{LLP-Bench: A representative collection of LLP datasets}\label{sec:llpbench}
Table \ref{tab:flagship_stats_and_clusters} provides a representative set of groupings, with their cluster assignments (as per the various analyses above) along with bag-level statistics. Several of these groupings are also used for the LLP model training and analysis presented below. We propose LLP-Bench as collection of LLP datasets with naturally constructed bags which simulate real-world LLP use-cases and can be used for evaluating LLP techniques.


==> best_methods_table.tex <==
\begin{table}[]
\centering
\scriptsize
\begin{tabular}{lllcccc}
\toprule
\textbf{Tail size} & \textbf{Stddev. Label Prop} & \textbf{Bag Separation} & \textbf{No. datasets} & \textbf{DLLP BCE} & \textbf{DLLP MSE} & \textbf{Sim LLP} \\ \midrule
\textit{Very Short-tailed} & \textit{High} & \textit{Well-separated} & 10 & 0 & 0 & 10 \\
\textit{Very Short-tailed} & \textit{High} & \textit{Far-separated} & 5 & 0 & 0 & 5 \\
\textit{Very Short-tailed} & \textit{Medium} & \textit{Medium-separated} & 11 & 0 & 0 & 11 \\
\textit{Very Short-tailed} & \textit{Medium} & \textit{Well-separated} & 3 & 0 & 0 & 3 \\
\textit{Very Short-tailed} & \textit{Medium} & \textit{Far-separated} & 4 & 0 & 0 & 4 \\
\textit{Very Short-tailed} & \textit{Low} & \textit{Medium-separated} & 1 & 0 & 0 & 1 \\
\textit{Short-tailed} & \textit{Medium} & \textit{Less-separated} & 1 & 0 & 0 & 1 \\
\textit{Short-tailed} & \textit{Medium} & \textit{Medium-separated} & 1 & 0 & 0 & 1 \\
\textit{Short-tailed} & \textit{Medium} & \textit{Well-separated} & 1 & 0 & 0 & 1 \\
\textit{Short-tailed} & \textit{Low} & \textit{Less-separated} & 1 & 1 & 0 & 0 \\
\textit{Short-tailed} & \textit{Low} & \textit{Well-separated} & 1 & 0 & 0 & 1 \\
\textit{Short-tailed} & \textit{Very Low} & \textit{Less-separated} & 1 & 1 & 0 & 0 \\
\textit{Long-tailed} & \textit{Low} & \textit{Medium-separated} & 2 & 0 & 0 & 2 \\
\textit{Long-tailed} & \textit{Very Low} & \textit{Less-separated} & 3 & 0 & 3 & 0 \\
\textit{Long-tailed} & \textit{Very Low} & \textit{Medium-separated} & 1 & 1 & 0 & 0 \\
\textit{Long-tailed} & \textit{Very Low} & \textit{Well-separated} & 3 & 2 & 1 & 0 \\
\textit{Very Long-tailed} & \textit{Low} & \textit{Well-separated} & 1 & 0 & 1 & 0 \\
\textit{Very Long-tailed} & \textit{Very Low} & \textit{Well-separated} & 2 & 0 & 1 & 1 \\ \bottomrule
\end{tabular}
\caption{No. of times each method performs the best for each category of datasets.}
\label{tab:best_methods}
\end{table}

==> checklist.tex <==
\section*{Checklist}

The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Lines 400-406.} 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{There are no conceivable negative societal impacts of our work.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Appendix \ref{sec:bagseplemma}, \ref{appendix:meanbag}, \ref{appendix:a3}, \ref{appendix:sq_l2_bag_sep} and \ref{sec:example}.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See Appendix \ref{sec:bagseplemma}, \ref{appendix:meanbag}, \ref{appendix:a3}, \ref{appendix:sq_l2_bag_sep} and \ref{sec:example}.}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{Yes, we have included the anonymized code for the experiments in the updated Supplementary Material. The code will be made publicly available along with the camera ready version of the paper.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section \ref{sec:llpbench-performance} and Appendix \ref{sec:additional-experiment-details}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Tables \ref{tab:auc_baselines}, \ref{tab:feature_rand_auc} and \ref{tab:rand_feat_bags_std}}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We use the Criteo Dataset for Kaggle display advertising challenge which is cited as \cite{Criteo:2014}.}
  \item Did you mention the license of the assets?
    \answerYes{} The url provided in the Criteo Dataset citation \cite{Criteo:2014} links to its license. 
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{We use an already curated Criteo Dataset to propose our benchmark. The license of the Criteo Dataset (see \cite{Criteo:2014}) permits non-commercial use.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{We mention in Sec. \ref{sec:dataset_creation} that the data is anonymized.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}



==> dllp_model_training.tex <==
\subsection{LLP model training}
\label{train_perlimnaries}
In order to train a model on an LLP  dataset, we apply common loss functions at the bag level. In this work we experiment with the \emph{binary cross entropy} loss ${\sf L}_{\tn{bce}}$, \emph{mean-squared error} loss ${\sf L}_{\tn{mse}}$ and also \emph{mean-absolute error} loss ${\sf L}_{\tn{mae}}$, which are define for a bag $B$ with with average label $z_B := y_B/|B|$ and average label prediction $\hat{z}_B := \hat{y}_B/|B|$ as: 
\begin{equation}
    {\sf L}_{\tn{bce}}(B, z_B, \hat{z}_B) := -\left(z_B\log \hat{z}_B + (1-z_B)\log (1-\hat{z}_B)\right) \ \ \nonumber ,
\end{equation}
\begin{equation}
    \ \ {\sf L}_{\tn{mse}}(B, y_B, \hat{y}_B) := |y_B - \hat{y}_B|^2 \ \ , \ \ {\sf L}_{\tn{mae}}(B, y_B, \hat{y}_B) := |y_B - \hat{y}_B|. \nonumber
\end{equation}
Note that all the above losses are minimized when $\hat{y}_B = y_B$.

In our experiments we use mini-batch based model training on LLP dataset. A mini-batch here consists of $k$ bags $B_1, \dots, B_k$ and their corresponding label sum $y_{B_1}, \dots, y_{B_k}$. The model predicts on all the instances in the bags of the minibatch are aggregated into the predicted label sums $\hat{y}_{B_1}, \dots \hat{y}_{B_k}$. The batch-level loss is given by sum of the bag-level losses over the for the mini-batch bags. 

==> fixed_bags.tex <==
\subsection{Fixed size bags}\label{sec:training_fixed_size}
The training on fixed sized bags is similar the above. In this case however, since we are not doing any clipping, we use the same $5$-fold instance-level split across the groupings. Here, for each grouping and fixed bag size $q = \{64, 128, 256, 512\}$, the train instances are randomly ordered with the constraint that those having the same values for the grouping features must occur contiguously. From the ordering $q$-sized sequences are included into bags numbering the (no. of train-set instances) divided by $q$. 

Since we wish to compare the performance across different $q$, we make sure that each minibatch has the same number of instances, thus each epoch has the same number of steps. In particular, we set the minibatch size $S$ to be $b = 4096/q$ bags, and thus the number of steps would be (no. of train-set instances) divided by $4096$. We train $2$-layer MLP and the AutoInt models as described above, while the rest of the hyperparameters including the optimizer, learning rate and the number of epochs remain the same as for the grouping based bags. Appendix \ref{appendix:feature_random_train} contains the AUC scores of training 2-Layer MLP and AutoInt models on fixed size bags created using all trainable groupings. Tables \ref{tab:feature_rand_mlp_llp_bench} and \ref{tab:feature_rand_autoint_llp_bench} contain the same for fixed size bags created using \textit{LLP-Bench} groupings.

\input{table_feature_random_mlp_llp_bench}
\input{table_feature_random_autoint_llp_bench}


\subsubsection{Fixed sized bags.}
We report the AUC scores of training 2-Layer MLP and AutoInt on fixed size bags created from the \textit{LLP-Bench} groupings in Tables \ref{tab:feature_rand_mlp_llp_bench} \ref{tab:feature_rand_autoint_llp_bench} respectively (see Sec. \ref{sec:training_fixed_size}). We make the following observations.
\begin{itemize}
    \item [1.] Models perform worse when trained on bags of larger sizes. This can be seen across models and choice of loss functions. This is expected since larger bag sizes would amount to more loss in label information.
    \item [2.] The performance of AutoInt model degrades sharply with increase in bag size. 
    \item [3.] The $(C7, C21)$ grouping yields the best performing fixed size bag datasets across the choice of models and loss function.
\end{itemize}


\medskip
\noindent

==> model_performance_analysis.tex <==
\section{Model performance on trainable groupings} \label{sec:model_training}
\label{sec:train_results}
In this section we describe our model training experiments on the bags given by the $52$ groupings selected Sec. \ref{filter_sec}. Additionally, we train on collections of bags of fixed size $q \in \{64, 128, 256, 512\}$ which are derived from these $52$, allowing us to precisely infer how the trained model's predictive performance changes with bag sizes for different groupings. Before we describe the datasets and the details of the model architecture and training hyperparameters, we first abstract out the model training loop on bags.

\subsection{Training Procedure on Bags}
Given a collection of bags $\{B_1, \dots, B_M\}$ and a bag minibatch size $b$, in each training step $b$ bags are included into the minibatch. Using the bag label sum and the model predictions -- on all the feature-vectors in the bags of the minibatch -- the loss for each bag is computed. The minibatch loss is the sum of the losses over all the included bags, and the usual back-propagation updates the model's weights. The process is repeated for $S$ steps per epoch for $R$ epochs. Algorithm \ref{alg:training} formalizes this procedure, keeping for simplicity the gradient based optimizer and its hyperparameters implicit.




\subsection{Grouping Based Bags}
\label{model_train_sec}
We train on $52$ clipped groupings which pass the filters in Sec. \ref{filter_sec}, for which we create the train and test sets as follows.
For each grouping,  we recreate the instance-level dataset from the clipped bag-level dataset and the original labels. On this truncated instance-level dataset we perform a $5$-fold split, and for each split we obtain the training bags dataset by grouping the train set on the same categorical features. The test sets remain at the instance-level.

We train $1$-Layer MLP, $2$-Layer MLP\footnote{$1$-Layer MLP has $64$ hidden units, $2$-Layer MLP has $128$ and $64$ units in successive layers, tanh activation} and the AutoInt model. Preprocessing mentioned in \ref{sec:contributions} ensures that all features have non-negative integers. We use a multihot layer whose output is passed to the MLP models. AutoInt has a $16$-dimensional trainable embedding layer for each feature\footnote{Embedding Layer for categorical features, numerical features multiplied by trainable 16-dim vector}. Output layer has one unit with sigmoid activation.

We apply minibatch training (Alg. \ref{alg:training}) on the bags with minibatch size $b = 8$,  number of steps $S$ being the number of bags in the train set divided by $b$, and $R = 50$ epochs. We use the Adam optimizer with learning rate $1e-5$ for initial $15$ epochs and $1e-6$ for the subsequent.

We use the test AUC score as our evaluation metric, quantifying the tractability of an LLP dataset. For the MLP models %
we use the maximum reported AUC score. On the other hand, AutoInt has an increasing trend for both optimizers but it is not (even locally) monotonic, hence for it we use the average of last 5 epochs of training.

The specifications of experiments are in Table \ref{tab:expt_legend}. 
The AUC score (averaged over the 5 splits) for trainable groupings in \textit{LLP-Bench} and the various experiments (see in conjunction with Table \ref{tab:expt_legend}) are listed in \ref{tab:auc_llp_bench_mlp}. AUC score for all trainable groupings are listed in Table \ref{tab:auc_scores}. Appendix \ref{appendix:instance_level_training} contains details of instance-level training which we perform for completeness.
\input{table_auc_llp_bench_mlp}
\input{table_expt_legend}


\subsection{Experimental Results} \label{sec:experiment_results}

We compute the Pearson correlation between the AUC scores and the bag level statistics computed in Sec. \ref{sec:bag_dist_analysis}. These are visualised in Fig. \ref{fig:heatmap}. Some observations from these scores are:
 
 \noindent
    {\bf 1.} Positive correlation with number of bags and number of instances. This is as  expected as each bag adds to the label information and each instance adds to feature information available to the classifier. 
    
    \noindent
    {\bf 2.} Negative correlation with the mean bag size and percentile bag size thresholds. This is intuitively consistent with larger bags having less label supervision (for the same label proportion) than smaller bags, and typically the model performance would degrade when the groupings have larger bags. 
    
    \noindent
    {\bf 3.} Negative correlation with the label proportion log likelihood. A lower log likelihood indicates that labels proportions in the dataset are highly skewed. This means that those groupings where the positive labels are concentrated in fewer bags have better training performance. In this case, the bag grouping features provide significant supervision which the model can leverage. We can infer the same from highly positive correlation with standard deviation of label proportion.
    \item[4.] Positive correlation with the {\sf InterIntraRatio}. Higher ratio indicates a good separation between the bags in input space. Hence, positive correlation indicates that models perform better when bags are separable in input space. This can be explained as follows
    \begin{itemize}
        \item The distribution of label proportions are skewed as the maximum log-likelihood exhibited is $-3.26$. Hence, substantial label information is present at the bag-level.
        \item If the {\sf InterIntraRatio} is high, much of the discriminative information at the bag-level  lies in the input space itself. If the {\sf InterIntraRatio} is low, most of this information is in some latent space that the model needs to learn.
    \end{itemize}
 
\begin{figure}[h!]
  \caption{Correlation Heatmap}
  \label{fig:heatmap}
  \includegraphics[scale=0.6]{new_corelation_heatmap (1).pdf}
\end{figure}



\emph{Experimental Code.} Our methods were implemented in python and our model training used TensorFlow 2. Our code for the LLP dataset creation, analysis and model training will be publicly released in due course of the publication of this paper.

==> table_2.tex <==
\begin{small}
\begin{centering}
\begin{longtable}{|l|l|l|l|l|l|l|}
\caption{Threshold bag size values below which 50, 70, 85, 95\% of bags present and clustering based on this distribution}
\label{tab:bag_dist_clustering}
\hline
\textbf{Col1} & \textbf{Col2} & \textbf{\begin{tabular}[c]{@{}l@{}}Bag size below\\ which 50\% bags\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Bag size below\\ which 70\% bags\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Bag size below\\ which 85\% bags\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Bag size below\\ which 95\% bags\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Clusters assigned on\\ bag size distribution\end{tabular}} \\ \hline
\textit{C1} & \textit{-} & 70 & 210 & 420 & 1130 & Very Short-tailed \\ \hline
\textit{C3} & \textit{-} & 101 & 172 & 335 & 812 & Very Short-tailed \\ \hline
\textit{C4} & \textit{-} & 117 & 212 & 430 & 1019 & Very Short-tailed \\ \hline
\textit{C7} & \textit{-} & 502 & 951 & 1499 & 2076 & Very Long-tailed \\ \hline
\textit{C8} & \textit{-} & 110 & 210 & 510 & 1383 & Short-tailed \\ \hline
\textit{C10} & \textit{-} & 175 & 365 & 764 & 1533 & Short-tailed \\ \hline
\textit{C11} & \textit{-} & 637 & 1155 & 1699 & 2194 & Very Long-tailed \\ \hline
\textit{C12} & \textit{-} & 103 & 175 & 341 & 821 & Very Short-tailed \\ \hline
\textit{C13} & \textit{-} & 1044 & 1498 & 1976 & 2349 & Very Long-tailed \\ \hline
\textit{C15} & \textit{-} & 264 & 564 & 1121 & 1829 & Long-tailed \\ \hline
\textit{C16} & \textit{-} & 106 & 184 & 364 & 890 & Very Short-tailed \\ \hline
\textit{C18} & \textit{-} & 327 & 697 & 1271 & 1983 & Long-tailed \\ \hline
\textit{C19} & \textit{-} & 456 & 917 & 1454 & 2153 & Very Long-tailed \\ \hline
\textit{C21} & \textit{-} & 104 & 180 & 352 & 835 & Very Short-tailed \\ \hline
\textit{C24} & \textit{-} & 136 & 264 & 559 & 1279 & Short-tailed \\ \hline
\textit{C26} & \textit{-} & 136 & 256 & 538 & 1203 & Short-tailed \\ \hline
\textit{C1} & \textit{C2} & 151 & 308 & 671 & 1455 & Short-tailed \\ \hline
\textit{C1} & \textit{C3} & 103 & 171 & 335 & 825 & Very Short-tailed \\ \hline
\textit{C1} & \textit{C4} & 108 & 184 & 361 & 872 & Very Short-tailed \\ \hline
\textit{C1} & \textit{C5} & 70 & 190 & 415 & 1050 & Very Short-tailed \\ \hline
\textit{C1} & \textit{C6} & 142 & 286 & 647 & 1449 & Short-tailed \\ \hline
\textit{C1} & \textit{C7} & 140 & 271 & 569 & 1270 & Short-tailed \\ \hline
\textit{C1} & \textit{C8} & 70 & 140 & 361 & 1010 & Very Short-tailed \\ \hline
\textit{C1} & \textit{C9} & 91 & 197 & 449 & 1168 & Very Short-tailed \\ \hline
\textit{C1} & \textit{C10} & 122 & 224 & 454 & 1068 & Very Short-tailed \\ \hline
\textit{C1} & \textit{C11} & 145 & 290 & 624 & 1374 & Short-tailed \\ \hline
\textit{C1} & \textit{C12} & 103 & 172 & 338 & 829 & Very Short-tailed \\ \hline
\textit{C1} & \textit{C13} & 148 & 299 & 643 & 1397 & Short-tailed \\ \hline
\textit{C1} & \textit{C14} & 142 & 289 & 633 & 1461 & Short-tailed \\ \hline
\textit{C1} & \textit{C15} & 137 & 265 & 566 & 1267 & Short-tailed \\ \hline
\textit{C1} & \textit{C16} & 104 & 176 & 347 & 854 & Very Short-tailed \\ \hline
\textit{C1} & \textit{C17} & 151 & 302 & 655 & 1443 & Short-tailed \\ \hline
\textit{C1} & \textit{C18} & 142 & 281 & 606 & 1333 & Short-tailed \\ \hline
\textit{C1} & \textit{C19} & 140 & 272 & 575 & 1292 & Short-tailed \\ \hline
\textit{C1} & \textit{C20} & 138 & 277 & 645 & 1419 & Short-tailed \\ \hline
\textit{C1} & \textit{C21} & 103 & 174 & 339 & 830 & Very Short-tailed \\ \hline
\textit{C1} & \textit{C22} & 109 & 224 & 525 & 1247 & Short-tailed \\ \hline
\textit{C1} & \textit{C23} & 142 & 293 & 652 & 1456 & Short-tailed \\ \hline
\textit{C1} & \textit{C24} & 116 & 209 & 422 & 1006 & Very Short-tailed \\ \hline
\textit{C1} & \textit{C25} & 148 & 297 & 658 & 1417 & Short-tailed \\ \hline
\textit{C1} & \textit{C26} & 114 & 200 & 404 & 964 & Very Short-tailed \\ \hline
\textit{C2} & \textit{C3} & 102 & 176 & 344 & 837 & Very Short-tailed \\ \hline
\textit{C2} & \textit{C4} & 112 & 201 & 404 & 984 & Very Short-tailed \\ \hline
\textit{C2} & \textit{C5} & 175 & 377 & 816 & 1622 & Short-tailed \\ \hline
\textit{C2} & \textit{C6} & 419 & 878 & 1499 & 2112 & Very Long-tailed \\ \hline
\textit{C2} & \textit{C7} & 136 & 253 & 503 & 1102 & Very Short-tailed \\ \hline
\textit{C2} & \textit{C8} & 164 & 344 & 742 & 1523 & Short-tailed \\ \hline
\textit{C2} & \textit{C10} & 119 & 210 & 420 & 957 & Very Short-tailed \\ \hline
\textit{C2} & \textit{C11} & 157 & 311 & 637 & 1329 & Short-tailed \\ \hline
\textit{C2} & \textit{C12} & 103 & 177 & 347 & 842 & Very Short-tailed \\ \hline
\textit{C2} & \textit{C13} & 165 & 334 & 688 & 1398 & Short-tailed \\ \hline
\textit{C2} & \textit{C14} & 613 & 1139 & 1701 & 2229 & Very Long-tailed \\ \hline
\textit{C2} & \textit{C15} & 264 & 564 & 1121 & 1829 & Long-tailed \\ \hline
\textit{C2} & \textit{C16} & 105 & 183 & 364 & 903 & Very Short-tailed \\ \hline
\textit{C2} & \textit{C17} & 479 & 855 & 1413 & 2010 & Very Long-tailed \\ \hline
\textit{C2} & \textit{C18} & 327 & 696 & 1271 & 1983 & Long-tailed \\ \hline
\textit{C2} & \textit{C19} & 151 & 304 & 630 & 1413 & Short-tailed \\ \hline
\textit{C2} & \textit{C21} & 104 & 180 & 353 & 853 & Very Short-tailed \\ \hline
\textit{C2} & \textit{C22} & 304 & 664 & 1245 & 2019 & Long-tailed \\ \hline
\textit{C2} & \textit{C23} & 395 & 788 & 1351 & 1992 & Long-tailed \\ \hline
\textit{C2} & \textit{C24} & 124 & 232 & 484 & 1171 & Very Short-tailed \\ \hline
\textit{C2} & \textit{C25} & 210 & 506 & 1041 & 1813 & Long-tailed \\ \hline
\textit{C2} & \textit{C26} & 122 & 224 & 458 & 1089 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C4} & 103 & 175 & 335 & 803 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C5} & 103 & 174 & 336 & 819 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C6} & 102 & 170 & 334 & 837 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C7} & 103 & 173 & 334 & 804 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C8} & 103 & 173 & 336 & 832 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C9} & 102 & 175 & 341 & 827 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C10} & 100 & 164 & 312 & 753 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C11} & 105 & 179 & 351 & 853 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C12} & 101 & 172 & 334 & 810 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C13} & 106 & 180 & 357 & 864 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C14} & 103 & 175 & 337 & 836 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C15} & 109 & 193 & 402 & 1030 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C16} & 100 & 166 & 316 & 764 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C17} & 103 & 175 & 344 & 846 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C18} & 104 & 183 & 371 & 950 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C19} & 102 & 175 & 350 & 858 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C20} & 103 & 175 & 340 & 820 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C21} & 100 & 167 & 322 & 786 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C22} & 102 & 172 & 338 & 837 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C23} & 103 & 174 & 340 & 834 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C24} & 107 & 185 & 364 & 875 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C25} & 103 & 175 & 339 & 826 & Very Short-tailed \\ \hline
\textit{C3} & \textit{C26} & 107 & 185 & 365 & 877 & Very Short-tailed \\ \hline
\textit{C4} & \textit{C5} & 110 & 192 & 382 & 912 & Very Short-tailed \\ \hline
\textit{C4} & \textit{C6} & 110 & 190 & 373 & 895 & Very Short-tailed \\ \hline
\textit{C4} & \textit{C7} & 100 & 161 & 296 & 685 & Very Short-tailed \\ \hline
\textit{C4} & \textit{C8} & 109 & 188 & 372 & 895 & Very Short-tailed \\ \hline
\textit{C4} & \textit{C9} & 116 & 207 & 418 & 987 & Very Short-tailed \\ \hline
\textit{C4} & \textit{C10} & 97 & 157 & 290 & 669 & Very Short-tailed \\ \hline
\textit{C4} & \textit{C11} & 104 & 174 & 333 & 780 & Very Short-tailed \\ \hline
\textit{C4} & \textit{C12} & 103 & 175 & 337 & 804 & Very Short-tailed \\ \hline
\textit{C4} & \textit{C13} & 106 & 177 & 341 & 800 & Very Short-tailed \\ \hline
\textit{C4} & \textit{C14} & 114 & 200 & 397 & 945 & Very Short-tailed \\ \hline
\textit{C4} & \textit{C15} & 114 & 203 & 417 & 1030 & Very Short-tailed \\ \hline
\textit{C4} & \textit{C16} & 104 & 177 & 349 & 843 & Very Short-tailed \\ \hline
\textit{C4} & \textit{C17} & 110 & 189 & 374 & 892 & Very Short-tailed \\ \hline
\textit{C4} & \textit{C18} & 114 & 205 & 413 & 1020 & Very Short-tailed \\ \hline
\textit{C4} & \textit{C19} & 111 & 196 & 392 & 953 & Very Short-tailed \\ \hline
\textit{C4} & \textit{C20} & 114 & 202 & 407 & 965 & Very Short-tailed \\ \hline
\textit{C4} & \textit{C21} & 103 & 175 & 337 & 793 & Very Short-tailed \\ \hline
\textit{C4} & \textit{C22} & 113 & 199 & 400 & 964 & Very Short-tailed \\ \hline
\textit{C4} & \textit{C23} & 110 & 192 & 384 & 904 & Very Short-tailed \\ \hline
\textit{C4} & \textit{C24} & 113 & 202 & 408 & 976 & Very Short-tailed \\ \hline
\textit{C4} & \textit{C25} & 116 & 208 & 418 & 1012 & Very Short-tailed \\ \hline
\textit{C4} & \textit{C26} & 114 & 202 & 406 & 983 & Very Short-tailed \\ \hline
\textit{C5} & \textit{C6} & 176 & 358 & 821 & 1641 & Short-tailed \\ \hline
\textit{C5} & \textit{C7} & 163 & 331 & 702 & 1465 & Short-tailed \\ \hline
\textit{C5} & \textit{C8} & 70 & 210 & 470 & 1210 & Very Short-tailed \\ \hline
\textit{C5} & \textit{C10} & 133 & 253 & 523 & 1192 & Short-tailed \\ \hline
\textit{C5} & \textit{C11} & 169 & 356 & 765 & 1556 & Short-tailed \\ \hline
\textit{C5} & \textit{C12} & 103 & 174 & 338 & 825 & Very Short-tailed \\ \hline
\textit{C5} & \textit{C13} & 173 & 368 & 791 & 1582 & Short-tailed \\ \hline
\textit{C5} & \textit{C14} & 179 & 373 & 825 & 1638 & Short-tailed \\ \hline
\textit{C5} & \textit{C15} & 153 & 310 & 667 & 1416 & Short-tailed \\ \hline
\textit{C5} & \textit{C16} & 105 & 180 & 355 & 860 & Very Short-tailed \\ \hline
\textit{C5} & \textit{C17} & 180 & 392 & 789 & 1699 & Short-tailed \\ \hline
\textit{C5} & \textit{C18} & 162 & 334 & 720 & 1498 & Short-tailed \\ \hline
\textit{C5} & \textit{C19} & 162 & 339 & 712 & 1506 & Short-tailed \\ \hline
\textit{C5} & \textit{C21} & 104 & 177 & 344 & 833 & Very Short-tailed \\ \hline
\textit{C5} & \textit{C23} & 174 & 367 & 821 & 1705 & Short-tailed \\ \hline
\textit{C5} & \textit{C24} & 122 & 223 & 459 & 1093 & Very Short-tailed \\ \hline
\textit{C5} & \textit{C25} & 173 & 372 & 772 & 1589 & Short-tailed \\ \hline
\textit{C5} & \textit{C26} & 119 & 215 & 440 & 1034 & Very Short-tailed \\ \hline
\textit{C6} & \textit{C7} & 222 & 443 & 854 & 1600 & Short-tailed \\ \hline
\textit{C6} & \textit{C8} & 165 & 343 & 729 & 1534 & Short-tailed \\ \hline
\textit{C6} & \textit{C10} & 144 & 271 & 567 & 1246 & Short-tailed \\ \hline
\textit{C6} & \textit{C11} & 310 & 640 & 1172 & 1872 & Long-tailed \\ \hline
\textit{C6} & \textit{C12} & 102 & 171 & 335 & 839 & Very Short-tailed \\ \hline
\textit{C6} & \textit{C13} & 367 & 728 & 1274 & 1944 & Long-tailed \\ \hline
\textit{C6} & \textit{C15} & 190 & 400 & 837 & 1645 & Short-tailed \\ \hline
\textit{C6} & \textit{C16} & 106 & 180 & 355 & 872 & Very Short-tailed \\ \hline
\textit{C6} & \textit{C18} & 217 & 464 & 937 & 1730 & Long-tailed \\ \hline
\textit{C6} & \textit{C19} & 211 & 422 & 822 & 1578 & Short-tailed \\ \hline
\textit{C6} & \textit{C21} & 103 & 173 & 338 & 840 & Very Short-tailed \\ \hline
\textit{C6} & \textit{C24} & 124 & 228 & 459 & 1091 & Very Short-tailed \\ \hline
\textit{C6} & \textit{C26} & 119 & 216 & 436 & 1066 & Very Short-tailed \\ \hline
\textit{C7} & \textit{C8} & 153 & 303 & 646 & 1383 & Short-tailed \\ \hline
\textit{C7} & \textit{C9} & 502 & 951 & 1499 & 2076 & Very Long-tailed \\ \hline
\textit{C7} & \textit{C10} & 151 & 296 & 613 & 1316 & Short-tailed \\ \hline
\textit{C7} & \textit{C11} & 419 & 832 & 1392 & 2019 & Very Long-tailed \\ \hline
\textit{C7} & \textit{C12} & 103 & 173 & 329 & 787 & Very Short-tailed \\ \hline
\textit{C7} & \textit{C13} & 502 & 951 & 1499 & 2076 & Very Long-tailed \\ \hline
\textit{C7} & \textit{C14} & 205 & 417 & 833 & 1577 & Short-tailed \\ \hline
\textit{C7} & \textit{C15} & 103 & 168 & 306 & 696 & Very Short-tailed \\ \hline
\textit{C7} & \textit{C16} & 102 & 168 & 311 & 727 & Very Short-tailed \\ \hline
\textit{C7} & \textit{C17} & 284 & 581 & 1076 & 1791 & Long-tailed \\ \hline
\textit{C7} & \textit{C18} & 110 & 188 & 360 & 830 & Very Short-tailed \\ \hline
\textit{C7} & \textit{C19} & 133 & 273 & 619 & 1384 & Short-tailed \\ \hline
\textit{C7} & \textit{C20} & 261 & 523 & 977 & 1703 & Long-tailed \\ \hline
\textit{C7} & \textit{C21} & 103 & 171 & 321 & 761 & Very Short-tailed \\ \hline
\textit{C7} & \textit{C22} & 223 & 467 & 929 & 1670 & Long-tailed \\ \hline
\textit{C7} & \textit{C23} & 210 & 450 & 918 & 1676 & Long-tailed \\ \hline
\textit{C7} & \textit{C24} & 104 & 172 & 322 & 748 & Very Short-tailed \\ \hline
\textit{C7} & \textit{C25} & 209 & 450 & 916 & 1700 & Long-tailed \\ \hline
\textit{C7} & \textit{C26} & 106 & 181 & 364 & 887 & Very Short-tailed \\ \hline
\textit{C8} & \textit{C9} & 121 & 220 & 596 & 1443 & Short-tailed \\ \hline
\textit{C8} & \textit{C10} & 128 & 238 & 491 & 1132 & Very Short-tailed \\ \hline
\textit{C8} & \textit{C11} & 159 & 326 & 705 & 1486 & Short-tailed \\ \hline
\textit{C8} & \textit{C12} & 104 & 174 & 339 & 833 & Very Short-tailed \\ \hline
\textit{C8} & \textit{C13} & 162 & 337 & 727 & 1516 & Short-tailed \\ \hline
\textit{C8} & \textit{C14} & 156 & 348 & 719 & 1505 & Short-tailed \\ \hline
\textit{C8} & \textit{C15} & 146 & 288 & 619 & 1350 & Short-tailed \\ \hline
\textit{C8} & \textit{C16} & 105 & 179 & 352 & 860 & Very Short-tailed \\ \hline
\textit{C8} & \textit{C17} & 158 & 344 & 748 & 1552 & Short-tailed \\ \hline
\textit{C8} & \textit{C18} & 154 & 308 & 667 & 1422 & Short-tailed \\ \hline
\textit{C8} & \textit{C19} & 150 & 306 & 646 & 1381 & Short-tailed \\ \hline
\textit{C8} & \textit{C20} & 161 & 330 & 754 & 1537 & Short-tailed \\ \hline
\textit{C8} & \textit{C21} & 104 & 176 & 342 & 839 & Very Short-tailed \\ \hline
\textit{C8} & \textit{C22} & 121 & 268 & 660 & 1473 & Short-tailed \\ \hline
\textit{C8} & \textit{C23} & 160 & 343 & 737 & 1580 & Short-tailed \\ \hline
\textit{C8} & \textit{C24} & 119 & 216 & 441 & 1049 & Very Short-tailed \\ \hline
\textit{C8} & \textit{C25} & 158 & 334 & 743 & 1529 & Short-tailed \\ \hline
\textit{C8} & \textit{C26} & 116 & 209 & 426 & 998 & Very Short-tailed \\ \hline
\textit{C9} & \textit{C10} & 168 & 344 & 709 & 1468 & Short-tailed \\ \hline
\textit{C9} & \textit{C11} & 610 & 1119 & 1671 & 2185 & Very Long-tailed \\ \hline
\textit{C9} & \textit{C12} & 103 & 177 & 346 & 834 & Very Short-tailed \\ \hline
\textit{C9} & \textit{C13} & 925 & 1394 & 1903 & 2298 & Very Long-tailed \\ \hline
\textit{C9} & \textit{C15} & 223 & 482 & 966 & 1749 & Long-tailed \\ \hline
\textit{C9} & \textit{C16} & 106 & 183 & 364 & 890 & Very Short-tailed \\ \hline
\textit{C9} & \textit{C18} & 264 & 560 & 1079 & 1863 & Long-tailed \\ \hline
\textit{C9} & \textit{C19} & 284 & 620 & 1162 & 1923 & Long-tailed \\ \hline
\textit{C9} & \textit{C21} & 105 & 181 & 355 & 845 & Very Short-tailed \\ \hline
\textit{C9} & \textit{C24} & 133 & 256 & 538 & 1245 & Short-tailed \\ \hline
\textit{C9} & \textit{C26} & 130 & 244 & 512 & 1156 & Very Short-tailed \\ \hline
\textit{C10} & \textit{C11} & 177 & 365 & 763 & 1523 & Short-tailed \\ \hline
\textit{C10} & \textit{C12} & 99 & 163 & 309 & 744 & Very Short-tailed \\ \hline
\textit{C10} & \textit{C13} & 177 & 372 & 777 & 1548 & Short-tailed \\ \hline
\textit{C10} & \textit{C14} & 141 & 272 & 557 & 1233 & Short-tailed \\ \hline
\textit{C10} & \textit{C15} & 101 & 164 & 303 & 705 & Very Short-tailed \\ \hline
\textit{C10} & \textit{C16} & 98 & 158 & 296 & 697 & Very Short-tailed \\ \hline
\textit{C10} & \textit{C17} & 145 & 280 & 581 & 1281 & Short-tailed \\ \hline
\textit{C10} & \textit{C18} & 105 & 176 & 338 & 786 & Very Short-tailed \\ \hline
\textit{C10} & \textit{C19} & 118 & 218 & 454 & 1081 & Very Short-tailed \\ \hline
\textit{C10} & \textit{C20} & 151 & 295 & 614 & 1342 & Short-tailed \\ \hline
\textit{C10} & \textit{C21} & 99 & 161 & 302 & 721 & Very Short-tailed \\ \hline
\textit{C10} & \textit{C22} & 147 & 290 & 614 & 1336 & Short-tailed \\ \hline
\textit{C10} & \textit{C23} & 149 & 289 & 595 & 1300 & Short-tailed \\ \hline
\textit{C10} & \textit{C24} & 100 & 165 & 310 & 728 & Very Short-tailed \\ \hline
\textit{C10} & \textit{C25} & 144 & 281 & 589 & 1294 & Short-tailed \\ \hline
\textit{C10} & \textit{C26} & 104 & 176 & 341 & 833 & Very Short-tailed \\ \hline
\textit{C11} & \textit{C12} & 106 & 181 & 356 & 857 & Very Short-tailed \\ \hline
\textit{C11} & \textit{C13} & 636 & 1151 & 1698 & 2192 & Very Long-tailed \\ \hline
\textit{C11} & \textit{C14} & 265 & 545 & 1067 & 1810 & Long-tailed \\ \hline
\textit{C11} & \textit{C15} & 110 & 188 & 355 & 810 & Very Short-tailed \\ \hline
\textit{C11} & \textit{C16} & 106 & 180 & 349 & 830 & Very Short-tailed \\ \hline
\textit{C11} & \textit{C17} & 312 & 647 & 1181 & 1872 & Long-tailed \\ \hline
\textit{C11} & \textit{C18} & 119 & 211 & 417 & 951 & Very Short-tailed \\ \hline
\textit{C11} & \textit{C19} & 117 & 223 & 505 & 1304 & Short-tailed \\ \hline
\textit{C11} & \textit{C20} & 402 & 793 & 1345 & 1979 & Long-tailed \\ \hline
\textit{C11} & \textit{C21} & 106 & 181 & 353 & 852 & Very Short-tailed \\ \hline
\textit{C11} & \textit{C22} & 251 & 560 & 1071 & 1812 & Long-tailed \\ \hline
\textit{C11} & \textit{C23} & 233 & 507 & 1021 & 1809 & Long-tailed \\ \hline
\textit{C11} & \textit{C24} & 109 & 187 & 364 & 859 & Very Short-tailed \\ \hline
\textit{C11} & \textit{C25} & 189 & 435 & 957 & 1783 & Long-tailed \\ \hline
\textit{C11} & \textit{C26} & 106 & 181 & 356 & 884 & Very Short-tailed \\ \hline
\textit{C12} & \textit{C13} & 107 & 183 & 362 & 871 & Very Short-tailed \\ \hline
\textit{C12} & \textit{C14} & 103 & 175 & 336 & 830 & Very Short-tailed \\ \hline
\textit{C12} & \textit{C15} & 108 & 191 & 395 & 1023 & Very Short-tailed \\ \hline
\textit{C12} & \textit{C16} & 100 & 167 & 318 & 772 & Very Short-tailed \\ \hline
\textit{C12} & \textit{C17} & 103 & 175 & 344 & 844 & Very Short-tailed \\ \hline
\textit{C12} & \textit{C18} & 104 & 183 & 369 & 936 & Very Short-tailed \\ \hline
\textit{C12} & \textit{C19} & 103 & 177 & 353 & 868 & Very Short-tailed \\ \hline
\textit{C12} & \textit{C20} & 103 & 176 & 342 & 821 & Very Short-tailed \\ \hline
\textit{C12} & \textit{C21} & 101 & 171 & 332 & 798 & Very Short-tailed \\ \hline
\textit{C12} & \textit{C22} & 103 & 174 & 341 & 842 & Very Short-tailed \\ \hline
\textit{C12} & \textit{C23} & 103 & 175 & 342 & 836 & Very Short-tailed \\ \hline
\textit{C12} & \textit{C24} & 107 & 186 & 366 & 873 & Very Short-tailed \\ \hline
\textit{C12} & \textit{C25} & 104 & 177 & 342 & 833 & Very Short-tailed \\ \hline
\textit{C12} & \textit{C26} & 108 & 186 & 366 & 876 & Very Short-tailed \\ \hline
\textit{C13} & \textit{C14} & 302 & 618 & 1157 & 1882 & Long-tailed \\ \hline
\textit{C13} & \textit{C15} & 113 & 195 & 374 & 868 & Very Short-tailed \\ \hline
\textit{C13} & \textit{C16} & 107 & 182 & 359 & 854 & Very Short-tailed \\ \hline
\textit{C13} & \textit{C17} & 367 & 733 & 1279 & 1960 & Long-tailed \\ \hline
\textit{C13} & \textit{C18} & 122 & 220 & 436 & 997 & Very Short-tailed \\ \hline
\textit{C13} & \textit{C19} & 114 & 214 & 482 & 1264 & Short-tailed \\ \hline
\textit{C13} & \textit{C20} & 527 & 951 & 1491 & 2074 & Very Long-tailed \\ \hline
\textit{C13} & \textit{C21} & 107 & 183 & 361 & 869 & Very Short-tailed \\ \hline
\textit{C13} & \textit{C22} & 276 & 626 & 1157 & 1902 & Long-tailed \\ \hline
\textit{C13} & \textit{C23} & 252 & 553 & 1085 & 1854 & Long-tailed \\ \hline
\textit{C13} & \textit{C24} & 111 & 191 & 373 & 880 & Very Short-tailed \\ \hline
\textit{C13} & \textit{C25} & 194 & 460 & 1002 & 1819 & Long-tailed \\ \hline
\textit{C13} & \textit{C26} & 107 & 183 & 357 & 890 & Very Short-tailed \\ \hline
\textit{C14} & \textit{C15} & 264 & 565 & 1120 & 1829 & Long-tailed \\ \hline
\textit{C14} & \textit{C16} & 107 & 185 & 362 & 882 & Very Short-tailed \\ \hline
\textit{C14} & \textit{C18} & 291 & 618 & 1180 & 1883 & Long-tailed \\ \hline
\textit{C14} & \textit{C19} & 188 & 379 & 761 & 1507 & Short-tailed \\ \hline
\textit{C14} & \textit{C21} & 106 & 181 & 349 & 839 & Very Short-tailed \\ \hline
\textit{C14} & \textit{C24} & 131 & 248 & 513 & 1163 & Very Short-tailed \\ \hline
\textit{C14} & \textit{C26} & 127 & 235 & 485 & 1134 & Very Short-tailed \\ \hline
\textit{C15} & \textit{C16} & 111 & 196 & 403 & 1017 & Very Short-tailed \\ \hline
\textit{C15} & \textit{C17} & 185 & 381 & 792 & 1592 & Short-tailed \\ \hline
\textit{C15} & \textit{C18} & 263 & 563 & 1120 & 1825 & Long-tailed \\ \hline
\textit{C15} & \textit{C19} & 142 & 284 & 610 & 1335 & Short-tailed \\ \hline
\textit{C15} & \textit{C20} & 272 & 588 & 1168 & 1885 & Long-tailed \\ \hline
\textit{C15} & \textit{C21} & 109 & 192 & 396 & 1011 & Very Short-tailed \\ \hline
\textit{C15} & \textit{C22} & 192 & 407 & 884 & 1662 & Short-tailed \\ \hline
\textit{C15} & \textit{C23} & 184 & 384 & 789 & 1580 & Short-tailed \\ \hline
\textit{C15} & \textit{C24} & 125 & 235 & 494 & 1181 & Very Short-tailed \\ \hline
\textit{C15} & \textit{C25} & 227 & 494 & 993 & 1746 & Long-tailed \\ \hline
\textit{C15} & \textit{C26} & 129 & 246 & 534 & 1252 & Short-tailed \\ \hline
\textit{C16} & \textit{C17} & 105 & 180 & 357 & 861 & Very Short-tailed \\ \hline
\textit{C16} & \textit{C18} & 108 & 191 & 389 & 966 & Very Short-tailed \\ \hline
\textit{C16} & \textit{C19} & 105 & 182 & 366 & 898 & Very Short-tailed \\ \hline
\textit{C16} & \textit{C20} & 106 & 182 & 360 & 869 & Very Short-tailed \\ \hline
\textit{C16} & \textit{C21} & 101 & 171 & 330 & 792 & Very Short-tailed \\ \hline
\textit{C16} & \textit{C22} & 106 & 183 & 362 & 890 & Very Short-tailed \\ \hline
\textit{C16} & \textit{C23} & 106 & 182 & 359 & 861 & Very Short-tailed \\ \hline
\textit{C16} & \textit{C24} & 107 & 184 & 364 & 881 & Very Short-tailed \\ \hline
\textit{C16} & \textit{C25} & 107 & 184 & 363 & 901 & Very Short-tailed \\ \hline
\textit{C16} & \textit{C26} & 108 & 186 & 369 & 899 & Very Short-tailed \\ \hline
\textit{C17} & \textit{C18} & 215 & 456 & 910 & 1695 & Long-tailed \\ \hline
\textit{C17} & \textit{C19} & 184 & 367 & 737 & 1477 & Short-tailed \\ \hline
\textit{C17} & \textit{C21} & 104 & 176 & 345 & 842 & Very Short-tailed \\ \hline
\textit{C17} & \textit{C24} & 122 & 223 & 458 & 1066 & Very Short-tailed \\ \hline
\textit{C17} & \textit{C26} & 118 & 213 & 441 & 1022 & Very Short-tailed \\ \hline
\textit{C18} & \textit{C19} & 166 & 348 & 742 & 1558 & Short-tailed \\ \hline
\textit{C18} & \textit{C20} & 335 & 712 & 1292 & 2002 & Long-tailed \\ \hline
\textit{C18} & \textit{C21} & 106 & 185 & 374 & 936 & Very Short-tailed \\ \hline
\textit{C18} & \textit{C22} & 211 & 454 & 958 & 1722 & Long-tailed \\ \hline
\textit{C18} & \textit{C23} & 217 & 460 & 918 & 1684 & Long-tailed \\ \hline
\textit{C18} & \textit{C24} & 126 & 238 & 497 & 1204 & Very Short-tailed \\ \hline
\textit{C18} & \textit{C25} & 264 & 564 & 1119 & 1860 & Long-tailed \\ \hline
\textit{C18} & \textit{C26} & 130 & 251 & 528 & 1253 & Short-tailed \\ \hline
\textit{C19} & \textit{C20} & 287 & 573 & 1076 & 1773 & Long-tailed \\ \hline
\textit{C19} & \textit{C21} & 104 & 180 & 358 & 870 & Very Short-tailed \\ \hline
\textit{C19} & \textit{C22} & 206 & 453 & 888 & 1648 & Long-tailed \\ \hline
\textit{C19} & \textit{C23} & 193 & 391 & 779 & 1526 & Short-tailed \\ \hline
\textit{C19} & \textit{C24} & 120 & 225 & 473 & 1125 & Very Short-tailed \\ \hline
\textit{C19} & \textit{C25} & 166 & 344 & 724 & 1575 & Short-tailed \\ \hline
\textit{C19} & \textit{C26} & 116 & 205 & 417 & 1004 & Very Short-tailed \\ \hline
\textit{C20} & \textit{C21} & 104 & 179 & 348 & 830 & Very Short-tailed \\ \hline
\textit{C20} & \textit{C24} & 130 & 247 & 516 & 1171 & Very Short-tailed \\ \hline
\textit{C20} & \textit{C26} & 130 & 241 & 498 & 1140 & Very Short-tailed \\ \hline
\textit{C21} & \textit{C22} & 104 & 177 & 345 & 848 & Very Short-tailed \\ \hline
\textit{C21} & \textit{C23} & 104 & 177 & 346 & 846 & Very Short-tailed \\ \hline
\textit{C21} & \textit{C24} & 108 & 187 & 368 & 864 & Very Short-tailed \\ \hline
\textit{C21} & \textit{C25} & 105 & 180 & 349 & 845 & Very Short-tailed \\ \hline
\textit{C21} & \textit{C26} & 108 & 186 & 366 & 875 & Very Short-tailed \\ \hline
\textit{C22} & \textit{C24} & 127 & 237 & 504 & 1170 & Very Short-tailed \\ \hline
\textit{C22} & \textit{C26} & 124 & 230 & 482 & 1124 & Very Short-tailed \\ \hline
\textit{C23} & \textit{C24} & 123 & 226 & 467 & 1079 & Very Short-tailed \\ \hline
\textit{C23} & \textit{C26} & 122 & 221 & 445 & 1039 & Very Short-tailed \\ \hline
\textit{C24} & \textit{C25} & 133 & 255 & 537 & 1257 & Short-tailed \\ \hline
\textit{C24} & \textit{C26} & 134 & 256 & 540 & 1255 & Short-tailed \\ \hline
\textit{C25} & \textit{C26} & 133 & 250 & 523 & 1197 & Short-tailed \\ \hline
\textit{C2} & \textit{-} & 934 & 1443 & 1846 & 2283 & - \\ \hline
\textit{C5} & \textit{-} & 140 & 280 & 630 & 1550 & - \\ \hline
\textit{C6} & \textit{-} & 573 & 1362 & 2079 & 2079 & - \\ \hline
\textit{C14} & \textit{-} & 1657 & 1657 & 1657 & 1657 & - \\ \hline
\textit{C17} & \textit{-} & 1292 & 1292 & 1292 & 1292 & - \\ \hline
\textit{C22} & \textit{-} & 117 & 180 & 496 & 496 & - \\ \hline
\textit{C23} & \textit{-} & 62 & 62 & 62 & 62 & - \\ \hline
\textit{C25} & \textit{-} & 190 & 408 & 591 & 730 & - \\ \hline
\textit{C2} & \textit{C9} & 544 & 993 & 1642 & 2277 & - \\ \hline
\textit{C2} & \textit{C20} & 801 & 1200 & 1713 & 2249 & - \\ \hline
\textit{C5} & \textit{C9} & 143 & 303 & 726 & 1509 & - \\ \hline
\textit{C5} & \textit{C20} & 168 & 346 & 793 & 1708 & - \\ \hline
\textit{C5} & \textit{C22} & 154 & 327 & 712 & 1467 & - \\ \hline
\textit{C6} & \textit{C9} & 459 & 771 & 1236 & 1852 & - \\ \hline
\textit{C6} & \textit{C14} & 259 & 608 & 1545 & 2127 & - \\ \hline
\textit{C6} & \textit{C17} & 209 & 353 & 620 & 864 & - \\ \hline
\textit{C6} & \textit{C20} & 336 & 747 & 1060 & 1738 & - \\ \hline
\textit{C6} & \textit{C22} & 413 & 573 & 1362 & 1869 & - \\ \hline
\textit{C6} & \textit{C23} & 358 & 717 & 1006 & 1902 & - \\ \hline
\textit{C6} & \textit{C25} & 355 & 817 & 1475 & 2060 & - \\ \hline
\textit{C9} & \textit{C14} & 613 & 1046 & 1657 & 2380 & - \\ \hline
\textit{C9} & \textit{C17} & 660 & 1513 & 1877 & 2286 & - \\ \hline
\textit{C9} & \textit{C20} & 773 & 1902 & 1902 & 1902 & - \\ \hline
\textit{C9} & \textit{C22} & 457 & 1115 & 1169 & 1302 & - \\ \hline
\textit{C9} & \textit{C23} & 294 & 917 & 1526 & 2323 & - \\ \hline
\textit{C9} & \textit{C25} & 302 & 641 & 1361 & 2223 & - \\ \hline
\textit{C14} & \textit{C17} & 822 & 1320 & 1792 & 2134 & - \\ \hline
\textit{C14} & \textit{C20} & 530 & 737 & 1657 & 1988 & - \\ \hline
\textit{C14} & \textit{C22} & 296 & 958 & 1527 & 2076 & - \\ \hline
\textit{C14} & \textit{C23} & 574 & 944 & 1781 & 2305 & - \\ \hline
\textit{C14} & \textit{C25} & 299 & 700 & 1304 & 1909 & - \\ \hline
\textit{C17} & \textit{C20} & 367 & 367 & 513 & 513 & - \\ \hline
\textit{C17} & \textit{C22} & 369 & 580 & 830 & 1655 & - \\ \hline
\textit{C17} & \textit{C23} & 247 & 619 & 912 & 1733 & - \\ \hline
\textit{C17} & \textit{C25} & 471 & 885 & 1691 & 2262 & - \\ \hline
\textit{C20} & \textit{C22} & 812 & 1482 & 2174 & 2180 & - \\ \hline
\textit{C20} & \textit{C23} & 1016 & 1386 & 1700 & 1700 & - \\ \hline
\textit{C20} & \textit{C25} & 297 & 834 & 1605 & 2243 & - \\ \hline
\textit{C22} & \textit{C23} & 476 & 768 & 1291 & 1899 & - \\ \hline
\textit{C22} & \textit{C25} & 310 & 536 & 1147 & 1903 & - \\ \hline
\textit{C23} & \textit{C25} & 348 & 740 & 1327 & 2105 & - \\ \hline
\end{longtable}
\end{centering}
\end{small}

==> table_3.tex <==
\begin{small}
\begin{centering}
\begin{longtable}{|l|l|l|l|l|l|}
\caption{Average Log Likelihood of Label Distribution of all grouping and it's clusters}
\label{tab:avg_ll}
\hline
\textbf{Col1} & \textbf{Col2} & \textbf{\begin{tabular}[c]{@{}l@{}}Standard deviation\\ of label proportions\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Label bias of\\ the grouping\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Average Log likelihood\\ of label sum distribution\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Clusters assigned on label \\ sum distribution\end{tabular}} \\ \hline
\textit{C1} & \textit{-} & 0.05 & 0.26 & -3.31 & High \\ \hline
\textit{C3} & \textit{-} & 0.17 & 0.26 & -17.26 & Low \\ \hline
\textit{C4} & \textit{-} & 0.16 & 0.26 & -18.24 & Low \\ \hline
\textit{C7} & \textit{-} & 0.11 & 0.22 & -25.85 & Very Low \\ \hline
\textit{C8} & \textit{-} & 0.05 & 0.26 & -3.33 & High \\ \hline
\textit{C10} & \textit{-} & 0.1 & 0.25 & -11.68 & Medium \\ \hline
\textit{C11} & \textit{-} & 0.1 & 0.21 & -29.13 & Very Low \\ \hline
\textit{C12} & \textit{-} & 0.17 & 0.26 & -17.29 & Low \\ \hline
\textit{C13} & \textit{-} & 0.09 & 0.21 & -32.14 & Very Low \\ \hline
\textit{C15} & \textit{-} & 0.16 & 0.27 & -34.69 & Very Low \\ \hline
\textit{C16} & \textit{-} & 0.16 & 0.26 & -17.37 & Low \\ \hline
\textit{C18} & \textit{-} & 0.15 & 0.29 & -35.47 & Very Low \\ \hline
\textit{C19} & \textit{-} & 0.07 & 0.26 & -10.9 & Medium \\ \hline
\textit{C21} & \textit{-} & 0.16 & 0.26 & -17.33 & Low \\ \hline
\textit{C24} & \textit{-} & 0.14 & 0.26 & -19.06 & Low \\ \hline
\textit{C26} & \textit{-} & 0.14 & 0.25 & -17.84 & Low \\ \hline
\textit{C1} & \textit{C2} & 0.1 & 0.26 & -11.58 & Medium \\ \hline
\textit{C1} & \textit{C3} & 0.16 & 0.26 & -15.35 & Medium \\ \hline
\textit{C1} & \textit{C4} & 0.15 & 0.26 & -14.82 & Medium \\ \hline
\textit{C1} & \textit{C5} & 0.05 & 0.26 & -3.29 & High \\ \hline
\textit{C1} & \textit{C6} & 0.05 & 0.26 & -3.86 & High \\ \hline
\textit{C1} & \textit{C7} & 0.12 & 0.24 & -14.11 & Medium \\ \hline
\textit{C1} & \textit{C8} & 0.05 & 0.26 & -3.26 & High \\ \hline
\textit{C1} & \textit{C9} & 0.08 & 0.24 & -6.41 & High \\ \hline
\textit{C1} & \textit{C10} & 0.1 & 0.26 & -9.17 & High \\ \hline
\textit{C1} & \textit{C11} & 0.11 & 0.24 & -13.62 & Medium \\ \hline
\textit{C1} & \textit{C12} & 0.16 & 0.26 & -15.3 & Medium \\ \hline
\textit{C1} & \textit{C13} & 0.11 & 0.24 & -12.79 & Medium \\ \hline
\textit{C1} & \textit{C14} & 0.1 & 0.26 & -10.68 & Medium \\ \hline
\textit{C1} & \textit{C15} & 0.14 & 0.27 & -17.63 & Low \\ \hline
\textit{C1} & \textit{C16} & 0.15 & 0.26 & -14.98 & Medium \\ \hline
\textit{C1} & \textit{C17} & 0.09 & 0.23 & -9.84 & Medium \\ \hline
\textit{C1} & \textit{C18} & 0.14 & 0.27 & -16.43 & Low \\ \hline
\textit{C1} & \textit{C19} & 0.08 & 0.26 & -6.54 & High \\ \hline
\textit{C1} & \textit{C20} & 0.05 & 0.25 & -3.74 & High \\ \hline
\textit{C1} & \textit{C21} & 0.16 & 0.26 & -15.25 & Medium \\ \hline
\textit{C1} & \textit{C22} & 0.05 & 0.26 & -3.47 & High \\ \hline
\textit{C1} & \textit{C23} & 0.08 & 0.25 & -8.35 & High \\ \hline
\textit{C1} & \textit{C24} & 0.14 & 0.26 & -15.09 & Medium \\ \hline
\textit{C1} & \textit{C25} & 0.06 & 0.27 & -4.95 & High \\ \hline
\textit{C1} & \textit{C26} & 0.14 & 0.25 & -14.47 & Medium \\ \hline
\textit{C2} & \textit{C3} & 0.17 & 0.26 & -18.51 & Low \\ \hline
\textit{C2} & \textit{C4} & 0.16 & 0.25 & -18.73 & Low \\ \hline
\textit{C2} & \textit{C5} & 0.1 & 0.26 & -13.44 & Medium \\ \hline
\textit{C2} & \textit{C6} & 0.12 & 0.26 & -25.47 & Very Low \\ \hline
\textit{C2} & \textit{C7} & 0.14 & 0.24 & -17.67 & Low \\ \hline
\textit{C2} & \textit{C8} & 0.1 & 0.26 & -12.51 & Medium \\ \hline
\textit{C2} & \textit{C10} & 0.13 & 0.26 & -12.53 & Medium \\ \hline
\textit{C2} & \textit{C11} & 0.14 & 0.24 & -19.45 & Low \\ \hline
\textit{C2} & \textit{C12} & 0.17 & 0.26 & -18.55 & Low \\ \hline
\textit{C2} & \textit{C13} & 0.14 & 0.24 & -19.35 & Low \\ \hline
\textit{C2} & \textit{C14} & 0.13 & 0.23 & -38.88 & Very Low \\ \hline
\textit{C2} & \textit{C15} & 0.16 & 0.27 & -34.68 & Very Low \\ \hline
\textit{C2} & \textit{C16} & 0.17 & 0.26 & -18.51 & Low \\ \hline
\textit{C2} & \textit{C17} & 0.12 & 0.22 & -30.65 & Very Low \\ \hline
\textit{C2} & \textit{C18} & 0.15 & 0.29 & -35.45 & Very Low \\ \hline
\textit{C2} & \textit{C19} & 0.1 & 0.26 & -10.64 & Medium \\ \hline
\textit{C2} & \textit{C21} & 0.17 & 0.26 & -18.49 & Low \\ \hline
\textit{C2} & \textit{C22} & 0.12 & 0.27 & -20.9 & Low \\ \hline
\textit{C2} & \textit{C23} & 0.13 & 0.23 & -31.79 & Very Low \\ \hline
\textit{C2} & \textit{C24} & 0.15 & 0.25 & -19.33 & Low \\ \hline
\textit{C2} & \textit{C25} & 0.11 & 0.27 & -16.42 & Low \\ \hline
\textit{C2} & \textit{C26} & 0.15 & 0.24 & -17.86 & Low \\ \hline
\textit{C3} & \textit{C4} & 0.16 & 0.26 & -16.04 & Low \\ \hline
\textit{C3} & \textit{C5} & 0.16 & 0.26 & -16.29 & Low \\ \hline
\textit{C3} & \textit{C6} & 0.17 & 0.26 & -17 & Low \\ \hline
\textit{C3} & \textit{C7} & 0.18 & 0.25 & -17.95 & Low \\ \hline
\textit{C3} & \textit{C8} & 0.16 & 0.26 & -15.91 & Medium \\ \hline
\textit{C3} & \textit{C9} & 0.17 & 0.26 & -18.56 & Low \\ \hline
\textit{C3} & \textit{C10} & 0.16 & 0.26 & -14.44 & Medium \\ \hline
\textit{C3} & \textit{C11} & 0.18 & 0.25 & -18.57 & Low \\ \hline
\textit{C3} & \textit{C12} & 0.17 & 0.26 & -17.24 & Low \\ \hline
\textit{C3} & \textit{C13} & 0.18 & 0.24 & -18.5 & Low \\ \hline
\textit{C3} & \textit{C14} & 0.18 & 0.26 & -19.68 & Low \\ \hline
\textit{C3} & \textit{C15} & 0.18 & 0.26 & -21.58 & Low \\ \hline
\textit{C3} & \textit{C16} & 0.16 & 0.26 & -16.08 & Low \\ \hline
\textit{C3} & \textit{C17} & 0.18 & 0.26 & -19.53 & Low \\ \hline
\textit{C3} & \textit{C18} & 0.17 & 0.26 & -19.44 & Low \\ \hline
\textit{C3} & \textit{C19} & 0.16 & 0.26 & -16.79 & Low \\ \hline
\textit{C3} & \textit{C20} & 0.17 & 0.26 & -18.1 & Low \\ \hline
\textit{C3} & \textit{C21} & 0.17 & 0.26 & -16.86 & Low \\ \hline
\textit{C3} & \textit{C22} & 0.17 & 0.26 & -17.05 & Low \\ \hline
\textit{C3} & \textit{C23} & 0.18 & 0.26 & -19.2 & Low \\ \hline
\textit{C3} & \textit{C24} & 0.16 & 0.26 & -16.42 & Low \\ \hline
\textit{C3} & \textit{C25} & 0.17 & 0.26 & -17.98 & Low \\ \hline
\textit{C3} & \textit{C26} & 0.16 & 0.26 & -17.63 & Low \\ \hline
\textit{C4} & \textit{C5} & 0.15 & 0.26 & -15.94 & Medium \\ \hline
\textit{C4} & \textit{C6} & 0.16 & 0.26 & -16.48 & Low \\ \hline
\textit{C4} & \textit{C7} & 0.18 & 0.26 & -17.39 & Low \\ \hline
\textit{C4} & \textit{C8} & 0.15 & 0.26 & -15.44 & Medium \\ \hline
\textit{C4} & \textit{C9} & 0.16 & 0.25 & -19.17 & Low \\ \hline
\textit{C4} & \textit{C10} & 0.16 & 0.27 & -14.9 & Medium \\ \hline
\textit{C4} & \textit{C11} & 0.17 & 0.26 & -17.92 & Low \\ \hline
\textit{C4} & \textit{C12} & 0.16 & 0.26 & -15.98 & Medium \\ \hline
\textit{C4} & \textit{C13} & 0.17 & 0.26 & -17.93 & Low \\ \hline
\textit{C4} & \textit{C14} & 0.16 & 0.26 & -19.6 & Low \\ \hline
\textit{C4} & \textit{C15} & 0.17 & 0.26 & -20.63 & Low \\ \hline
\textit{C4} & \textit{C16} & 0.16 & 0.26 & -16.51 & Low \\ \hline
\textit{C4} & \textit{C17} & 0.16 & 0.26 & -18.79 & Low \\ \hline
\textit{C4} & \textit{C18} & 0.16 & 0.26 & -19.2 & Low \\ \hline
\textit{C4} & \textit{C19} & 0.15 & 0.26 & -17 & Low \\ \hline
\textit{C4} & \textit{C20} & 0.16 & 0.26 & -18.48 & Low \\ \hline
\textit{C4} & \textit{C21} & 0.16 & 0.26 & -15.96 & Medium \\ \hline
\textit{C4} & \textit{C22} & 0.16 & 0.26 & -17.34 & Low \\ \hline
\textit{C4} & \textit{C23} & 0.17 & 0.26 & -19.01 & Low \\ \hline
\textit{C4} & \textit{C24} & 0.15 & 0.26 & -17.38 & Low \\ \hline
\textit{C4} & \textit{C25} & 0.16 & 0.26 & -18.53 & Low \\ \hline
\textit{C4} & \textit{C26} & 0.16 & 0.26 & -18.41 & Low \\ \hline
\textit{C5} & \textit{C6} & 0.05 & 0.26 & -4.13 & High \\ \hline
\textit{C5} & \textit{C7} & 0.12 & 0.23 & -15.47 & Medium \\ \hline
\textit{C5} & \textit{C8} & 0.05 & 0.26 & -3.29 & High \\ \hline
\textit{C5} & \textit{C10} & 0.1 & 0.26 & -9.8 & Medium \\ \hline
\textit{C5} & \textit{C11} & 0.11 & 0.23 & -15.13 & Medium \\ \hline
\textit{C5} & \textit{C12} & 0.16 & 0.26 & -16.24 & Low \\ \hline
\textit{C5} & \textit{C13} & 0.11 & 0.23 & -13.94 & Medium \\ \hline
\textit{C5} & \textit{C14} & 0.11 & 0.26 & -13.34 & Medium \\ \hline
\textit{C5} & \textit{C15} & 0.15 & 0.27 & -20.47 & Low \\ \hline
\textit{C5} & \textit{C16} & 0.16 & 0.26 & -16.02 & Low \\ \hline
\textit{C5} & \textit{C17} & 0.09 & 0.23 & -11.8 & Medium \\ \hline
\textit{C5} & \textit{C18} & 0.14 & 0.28 & -19.16 & Low \\ \hline
\textit{C5} & \textit{C19} & 0.07 & 0.26 & -7.35 & High \\ \hline
\textit{C5} & \textit{C21} & 0.16 & 0.26 & -16.28 & Low \\ \hline
\textit{C5} & \textit{C23} & 0.08 & 0.24 & -9.94 & Medium \\ \hline
\textit{C5} & \textit{C24} & 0.14 & 0.26 & -16.28 & Low \\ \hline
\textit{C5} & \textit{C25} & 0.06 & 0.27 & -5.53 & High \\ \hline
\textit{C5} & \textit{C26} & 0.14 & 0.25 & -15.58 & Medium \\ \hline
\textit{C6} & \textit{C7} & 0.12 & 0.23 & -18.8 & Low \\ \hline
\textit{C6} & \textit{C8} & 0.05 & 0.26 & -3.94 & High \\ \hline
\textit{C6} & \textit{C10} & 0.1 & 0.26 & -10.84 & Medium \\ \hline
\textit{C6} & \textit{C11} & 0.11 & 0.23 & -21.32 & Low \\ \hline
\textit{C6} & \textit{C12} & 0.16 & 0.26 & -16.94 & Low \\ \hline
\textit{C6} & \textit{C13} & 0.1 & 0.23 & -20.68 & Low \\ \hline
\textit{C6} & \textit{C15} & 0.16 & 0.27 & -26.42 & Very Low \\ \hline
\textit{C6} & \textit{C16} & 0.16 & 0.26 & -16.72 & Low \\ \hline
\textit{C6} & \textit{C18} & 0.16 & 0.29 & -26.28 & Very Low \\ \hline
\textit{C6} & \textit{C19} & 0.08 & 0.26 & -8.89 & High \\ \hline
\textit{C6} & \textit{C21} & 0.16 & 0.26 & -16.91 & Low \\ \hline
\textit{C6} & \textit{C24} & 0.15 & 0.26 & -17.56 & Low \\ \hline
\textit{C6} & \textit{C26} & 0.15 & 0.25 & -16.74 & Low \\ \hline
\textit{C7} & \textit{C8} & 0.12 & 0.24 & -14.95 & Medium \\ \hline
\textit{C7} & \textit{C9} & 0.11 & 0.22 & -25.84 & Very Low \\ \hline
\textit{C7} & \textit{C10} & 0.11 & 0.24 & -13.29 & Medium \\ \hline
\textit{C7} & \textit{C11} & 0.11 & 0.22 & -25.75 & Very Low \\ \hline
\textit{C7} & \textit{C12} & 0.17 & 0.25 & -17.65 & Low \\ \hline
\textit{C7} & \textit{C13} & 0.11 & 0.22 & -25.85 & Very Low \\ \hline
\textit{C7} & \textit{C14} & 0.14 & 0.23 & -21.55 & Low \\ \hline
\textit{C7} & \textit{C15} & 0.17 & 0.25 & -17.15 & Low \\ \hline
\textit{C7} & \textit{C16} & 0.17 & 0.25 & -17.37 & Low \\ \hline
\textit{C7} & \textit{C17} & 0.11 & 0.21 & -20.27 & Low \\ \hline
\textit{C7} & \textit{C18} & 0.16 & 0.24 & -17.44 & Low \\ \hline
\textit{C7} & \textit{C19} & 0.14 & 0.24 & -16.64 & Low \\ \hline
\textit{C7} & \textit{C20} & 0.12 & 0.22 & -20.59 & Low \\ \hline
\textit{C7} & \textit{C21} & 0.18 & 0.25 & -17.68 & Low \\ \hline
\textit{C7} & \textit{C22} & 0.12 & 0.24 & -19.64 & Low \\ \hline
\textit{C7} & \textit{C23} & 0.12 & 0.23 & -20 & Low \\ \hline
\textit{C7} & \textit{C24} & 0.17 & 0.26 & -16.83 & Low \\ \hline
\textit{C7} & \textit{C25} & 0.12 & 0.23 & -19.57 & Low \\ \hline
\textit{C7} & \textit{C26} & 0.17 & 0.25 & -17.49 & Low \\ \hline
\textit{C8} & \textit{C9} & 0.08 & 0.23 & -7.1 & High \\ \hline
\textit{C8} & \textit{C10} & 0.1 & 0.26 & -9.48 & High \\ \hline
\textit{C8} & \textit{C11} & 0.11 & 0.24 & -14.45 & Medium \\ \hline
\textit{C8} & \textit{C12} & 0.16 & 0.26 & -15.84 & Medium \\ \hline
\textit{C8} & \textit{C13} & 0.11 & 0.24 & -13.45 & Medium \\ \hline
\textit{C8} & \textit{C14} & 0.1 & 0.26 & -12.16 & Medium \\ \hline
\textit{C8} & \textit{C15} & 0.14 & 0.27 & -19.11 & Low \\ \hline
\textit{C8} & \textit{C16} & 0.16 & 0.26 & -15.6 & Medium \\ \hline
\textit{C8} & \textit{C17} & 0.09 & 0.23 & -10.55 & Medium \\ \hline
\textit{C8} & \textit{C18} & 0.14 & 0.28 & -17.86 & Low \\ \hline
\textit{C8} & \textit{C19} & 0.08 & 0.26 & -6.9 & High \\ \hline
\textit{C8} & \textit{C20} & 0.05 & 0.25 & -3.84 & High \\ \hline
\textit{C8} & \textit{C21} & 0.16 & 0.26 & -15.87 & Medium \\ \hline
\textit{C8} & \textit{C22} & 0.05 & 0.26 & -3.54 & High \\ \hline
\textit{C8} & \textit{C23} & 0.08 & 0.24 & -9 & High \\ \hline
\textit{C8} & \textit{C24} & 0.14 & 0.26 & -15.74 & Medium \\ \hline
\textit{C8} & \textit{C25} & 0.06 & 0.27 & -5.27 & High \\ \hline
\textit{C8} & \textit{C26} & 0.14 & 0.25 & -15.18 & Medium \\ \hline
\textit{C9} & \textit{C10} & 0.1 & 0.24 & -12.92 & Medium \\ \hline
\textit{C9} & \textit{C11} & 0.1 & 0.2 & -30.29 & Very Low \\ \hline
\textit{C9} & \textit{C12} & 0.17 & 0.26 & -18.55 & Low \\ \hline
\textit{C9} & \textit{C13} & 0.1 & 0.19 & -33.86 & Very Low \\ \hline
\textit{C9} & \textit{C15} & 0.16 & 0.25 & -34.98 & Very Low \\ \hline
\textit{C9} & \textit{C16} & 0.17 & 0.26 & -18.45 & Low \\ \hline
\textit{C9} & \textit{C18} & 0.16 & 0.26 & -35.17 & Very Low \\ \hline
\textit{C9} & \textit{C19} & 0.1 & 0.23 & -15.93 & Medium \\ \hline
\textit{C9} & \textit{C21} & 0.17 & 0.26 & -18.52 & Low \\ \hline
\textit{C9} & \textit{C24} & 0.15 & 0.25 & -20.43 & Low \\ \hline
\textit{C9} & \textit{C26} & 0.14 & 0.24 & -18.93 & Low \\ \hline
\textit{C10} & \textit{C11} & 0.1 & 0.24 & -13.61 & Medium \\ \hline
\textit{C10} & \textit{C12} & 0.16 & 0.26 & -14.31 & Medium \\ \hline
\textit{C10} & \textit{C13} & 0.1 & 0.24 & -12.8 & Medium \\ \hline
\textit{C10} & \textit{C14} & 0.12 & 0.26 & -13.33 & Medium \\ \hline
\textit{C10} & \textit{C15} & 0.15 & 0.26 & -14.08 & Medium \\ \hline
\textit{C10} & \textit{C16} & 0.16 & 0.26 & -14.35 & Medium \\ \hline
\textit{C10} & \textit{C17} & 0.1 & 0.25 & -11.73 & Medium \\ \hline
\textit{C10} & \textit{C18} & 0.15 & 0.26 & -13.55 & Medium \\ \hline
\textit{C10} & \textit{C19} & 0.12 & 0.26 & -11.26 & Medium \\ \hline
\textit{C10} & \textit{C20} & 0.1 & 0.26 & -11.43 & Medium \\ \hline
\textit{C10} & \textit{C21} & 0.16 & 0.26 & -14.4 & Medium \\ \hline
\textit{C10} & \textit{C22} & 0.1 & 0.26 & -11.19 & Medium \\ \hline
\textit{C10} & \textit{C23} & 0.11 & 0.26 & -12.46 & Medium \\ \hline
\textit{C10} & \textit{C24} & 0.15 & 0.27 & -13.68 & Medium \\ \hline
\textit{C10} & \textit{C25} & 0.11 & 0.26 & -11.28 & Medium \\ \hline
\textit{C10} & \textit{C26} & 0.15 & 0.26 & -13.96 & Medium \\ \hline
\textit{C11} & \textit{C12} & 0.18 & 0.25 & -18.45 & Low \\ \hline
\textit{C11} & \textit{C13} & 0.1 & 0.21 & -29.1 & Very Low \\ \hline
\textit{C11} & \textit{C14} & 0.14 & 0.23 & -25.74 & Very Low \\ \hline
\textit{C11} & \textit{C15} & 0.16 & 0.24 & -17.9 & Low \\ \hline
\textit{C11} & \textit{C16} & 0.17 & 0.25 & -18.17 & Low \\ \hline
\textit{C11} & \textit{C17} & 0.11 & 0.21 & -20.9 & Low \\ \hline
\textit{C11} & \textit{C18} & 0.16 & 0.24 & -18.61 & Low \\ \hline
\textit{C11} & \textit{C19} & 0.13 & 0.25 & -14.39 & Medium \\ \hline
\textit{C11} & \textit{C20} & 0.11 & 0.22 & -23.87 & Low \\ \hline
\textit{C11} & \textit{C21} & 0.18 & 0.25 & -18.6 & Low \\ \hline
\textit{C11} & \textit{C22} & 0.12 & 0.23 & -20.17 & Low \\ \hline
\textit{C11} & \textit{C23} & 0.12 & 0.23 & -21 & Low \\ \hline
\textit{C11} & \textit{C24} & 0.17 & 0.25 & -17.53 & Low \\ \hline
\textit{C11} & \textit{C25} & 0.12 & 0.23 & -18.45 & Low \\ \hline
\textit{C11} & \textit{C26} & 0.17 & 0.25 & -17.67 & Low \\ \hline
\textit{C12} & \textit{C13} & 0.17 & 0.25 & -18.42 & Low \\ \hline
\textit{C12} & \textit{C14} & 0.18 & 0.26 & -19.52 & Low \\ \hline
\textit{C12} & \textit{C15} & 0.18 & 0.26 & -21.37 & Low \\ \hline
\textit{C12} & \textit{C16} & 0.16 & 0.26 & -16.1 & Low \\ \hline
\textit{C12} & \textit{C17} & 0.17 & 0.26 & -19.4 & Low \\ \hline
\textit{C12} & \textit{C18} & 0.17 & 0.26 & -19.37 & Low \\ \hline
\textit{C12} & \textit{C19} & 0.16 & 0.26 & -16.82 & Low \\ \hline
\textit{C12} & \textit{C20} & 0.17 & 0.26 & -18.09 & Low \\ \hline
\textit{C12} & \textit{C21} & 0.16 & 0.26 & -16.99 & Low \\ \hline
\textit{C12} & \textit{C22} & 0.16 & 0.26 & -17.03 & Low \\ \hline
\textit{C12} & \textit{C23} & 0.18 & 0.26 & -19.21 & Low \\ \hline
\textit{C12} & \textit{C24} & 0.16 & 0.26 & -16.4 & Low \\ \hline
\textit{C12} & \textit{C25} & 0.17 & 0.26 & -18.02 & Low \\ \hline
\textit{C12} & \textit{C26} & 0.16 & 0.26 & -17.62 & Low \\ \hline
\textit{C13} & \textit{C14} & 0.13 & 0.23 & -26.13 & Very Low \\ \hline
\textit{C13} & \textit{C15} & 0.16 & 0.24 & -18.38 & Low \\ \hline
\textit{C13} & \textit{C16} & 0.17 & 0.25 & -18.16 & Low \\ \hline
\textit{C13} & \textit{C17} & 0.1 & 0.21 & -20.48 & Low \\ \hline
\textit{C13} & \textit{C18} & 0.16 & 0.24 & -18.75 & Low \\ \hline
\textit{C13} & \textit{C19} & 0.13 & 0.25 & -13.32 & Medium \\ \hline
\textit{C13} & \textit{C20} & 0.1 & 0.22 & -24.19 & Low \\ \hline
\textit{C13} & \textit{C21} & 0.17 & 0.25 & -18.56 & Low \\ \hline
\textit{C13} & \textit{C22} & 0.11 & 0.23 & -19.33 & Low \\ \hline
\textit{C13} & \textit{C23} & 0.12 & 0.23 & -20.39 & Low \\ \hline
\textit{C13} & \textit{C24} & 0.16 & 0.25 & -17.45 & Low \\ \hline
\textit{C13} & \textit{C25} & 0.12 & 0.23 & -17.36 & Low \\ \hline
\textit{C13} & \textit{C26} & 0.17 & 0.25 & -17.96 & Low \\ \hline
\textit{C14} & \textit{C15} & 0.16 & 0.27 & -34.64 & Very Low \\ \hline
\textit{C14} & \textit{C16} & 0.17 & 0.26 & -19.62 & Low \\ \hline
\textit{C14} & \textit{C18} & 0.15 & 0.27 & -34.77 & Very Low \\ \hline
\textit{C14} & \textit{C19} & 0.11 & 0.25 & -13.26 & Medium \\ \hline
\textit{C14} & \textit{C21} & 0.18 & 0.26 & -19.73 & Low \\ \hline
\textit{C14} & \textit{C24} & 0.16 & 0.26 & -21 & Low \\ \hline
\textit{C14} & \textit{C26} & 0.15 & 0.25 & -19.3 & Low \\ \hline
\textit{C15} & \textit{C16} & 0.17 & 0.26 & -21.13 & Low \\ \hline
\textit{C15} & \textit{C17} & 0.16 & 0.25 & -29.03 & Very Low \\ \hline
\textit{C15} & \textit{C18} & 0.16 & 0.27 & -34.66 & Very Low \\ \hline
\textit{C15} & \textit{C19} & 0.13 & 0.26 & -17.46 & Low \\ \hline
\textit{C15} & \textit{C20} & 0.16 & 0.27 & -34.75 & Very Low \\ \hline
\textit{C15} & \textit{C21} & 0.18 & 0.26 & -21.28 & Low \\ \hline
\textit{C15} & \textit{C22} & 0.16 & 0.28 & -26.58 & Very Low \\ \hline
\textit{C15} & \textit{C23} & 0.16 & 0.26 & -30.28 & Very Low \\ \hline
\textit{C15} & \textit{C24} & 0.16 & 0.25 & -21.78 & Low \\ \hline
\textit{C15} & \textit{C25} & 0.15 & 0.27 & -28.49 & Very Low \\ \hline
\textit{C15} & \textit{C26} & 0.16 & 0.25 & -21.96 & Low \\ \hline
\textit{C16} & \textit{C17} & 0.17 & 0.26 & -18.97 & Low \\ \hline
\textit{C16} & \textit{C18} & 0.17 & 0.26 & -19.3 & Low \\ \hline
\textit{C16} & \textit{C19} & 0.16 & 0.26 & -16.83 & Low \\ \hline
\textit{C16} & \textit{C20} & 0.17 & 0.26 & -18.13 & Low \\ \hline
\textit{C16} & \textit{C21} & 0.16 & 0.26 & -16.43 & Low \\ \hline
\textit{C16} & \textit{C22} & 0.16 & 0.26 & -17.16 & Low \\ \hline
\textit{C16} & \textit{C23} & 0.17 & 0.26 & -19.05 & Low \\ \hline
\textit{C16} & \textit{C24} & 0.16 & 0.26 & -16.29 & Low \\ \hline
\textit{C16} & \textit{C25} & 0.16 & 0.26 & -17.99 & Low \\ \hline
\textit{C16} & \textit{C26} & 0.16 & 0.26 & -17.68 & Low \\ \hline
\textit{C17} & \textit{C18} & 0.16 & 0.26 & -30.52 & Very Low \\ \hline
\textit{C17} & \textit{C19} & 0.1 & 0.24 & -13 & Medium \\ \hline
\textit{C17} & \textit{C21} & 0.17 & 0.26 & -19.25 & Low \\ \hline
\textit{C17} & \textit{C24} & 0.16 & 0.25 & -20.31 & Low \\ \hline
\textit{C17} & \textit{C26} & 0.15 & 0.24 & -18.47 & Low \\ \hline
\textit{C18} & \textit{C19} & 0.12 & 0.27 & -15.5 & Medium \\ \hline
\textit{C18} & \textit{C20} & 0.15 & 0.28 & -35.7 & Very Low \\ \hline
\textit{C18} & \textit{C21} & 0.17 & 0.26 & -19.29 & Low \\ \hline
\textit{C18} & \textit{C22} & 0.15 & 0.29 & -25.63 & Very Low \\ \hline
\textit{C18} & \textit{C23} & 0.16 & 0.26 & -32.27 & Very Low \\ \hline
\textit{C18} & \textit{C24} & 0.15 & 0.25 & -20.08 & Low \\ \hline
\textit{C18} & \textit{C25} & 0.14 & 0.28 & -28.31 & Very Low \\ \hline
\textit{C18} & \textit{C26} & 0.15 & 0.25 & -20 & Low \\ \hline
\textit{C19} & \textit{C20} & 0.08 & 0.26 & -10.84 & Medium \\ \hline
\textit{C19} & \textit{C21} & 0.16 & 0.26 & -16.92 & Low \\ \hline
\textit{C19} & \textit{C22} & 0.08 & 0.26 & -8.94 & High \\ \hline
\textit{C19} & \textit{C23} & 0.1 & 0.25 & -12.29 & Medium \\ \hline
\textit{C19} & \textit{C24} & 0.14 & 0.25 & -16.5 & Low \\ \hline
\textit{C19} & \textit{C25} & 0.09 & 0.26 & -10.23 & Medium \\ \hline
\textit{C19} & \textit{C26} & 0.14 & 0.25 & -14.99 & Medium \\ \hline
\textit{C20} & \textit{C21} & 0.17 & 0.26 & -18.19 & Low \\ \hline
\textit{C20} & \textit{C24} & 0.15 & 0.25 & -19.38 & Low \\ \hline
\textit{C20} & \textit{C26} & 0.15 & 0.25 & -18.09 & Low \\ \hline
\textit{C21} & \textit{C22} & 0.16 & 0.26 & -17.08 & Low \\ \hline
\textit{C21} & \textit{C23} & 0.18 & 0.26 & -19.2 & Low \\ \hline
\textit{C21} & \textit{C24} & 0.16 & 0.26 & -16.34 & Low \\ \hline
\textit{C21} & \textit{C25} & 0.17 & 0.26 & -17.94 & Low \\ \hline
\textit{C21} & \textit{C26} & 0.16 & 0.26 & -17.63 & Low \\ \hline
\textit{C22} & \textit{C24} & 0.15 & 0.26 & -18.31 & Low \\ \hline
\textit{C22} & \textit{C26} & 0.14 & 0.25 & -17.29 & Low \\ \hline
\textit{C23} & \textit{C24} & 0.16 & 0.26 & -20.12 & Low \\ \hline
\textit{C23} & \textit{C26} & 0.15 & 0.24 & -18.82 & Low \\ \hline
\textit{C24} & \textit{C25} & 0.15 & 0.25 & -19.27 & Low \\ \hline
\textit{C24} & \textit{C26} & 0.15 & 0.25 & -20.44 & Low \\ \hline
\textit{C25} & \textit{C26} & 0.14 & 0.24 & -18.44 & Low \\ \hline
\textit{C2} & \textit{-} & 0.13 & 0.28 & -47.05 & - \\ \hline
\textit{C5} & \textit{-} & 0.05 & 0.26 & -3.41 & - \\ \hline
\textit{C6} & \textit{-} & 0.09 & 0.25 & -12.4 & - \\ \hline
\textit{C14} & \textit{-} & 0.12 & 0.29 & -33.6 & - \\ \hline
\textit{C17} & \textit{-} & 0 & 0.06 & -3.09 & - \\ \hline
\textit{C22} & \textit{-} & 0.05 & 0.26 & -3.24 & - \\ \hline
\textit{C23} & \textit{-} & 0 & 0.11 & -1.84 & - \\ \hline
\textit{C25} & \textit{-} & 0.08 & 0.26 & -5.81 & - \\ \hline
\textit{C2} & \textit{C9} & 0.12 & 0.21 & -36.84 & - \\ \hline
\textit{C2} & \textit{C20} & 0.13 & 0.27 & -42.36 & - \\ \hline
\textit{C5} & \textit{C9} & 0.08 & 0.22 & -8.52 & - \\ \hline
\textit{C5} & \textit{C20} & 0.04 & 0.25 & -3.93 & - \\ \hline
\textit{C5} & \textit{C22} & 0.05 & 0.27 & -3.67 & - \\ \hline
\textit{C6} & \textit{C9} & 0.09 & 0.19 & -16.45 & - \\ \hline
\textit{C6} & \textit{C14} & 0.13 & 0.23 & -32.2 & - \\ \hline
\textit{C6} & \textit{C17} & 0.09 & 0.2 & -11.09 & - \\ \hline
\textit{C6} & \textit{C20} & 0.07 & 0.23 & -5.86 & - \\ \hline
\textit{C6} & \textit{C22} & 0.15 & 0.27 & -9.38 & - \\ \hline
\textit{C6} & \textit{C23} & 0.11 & 0.2 & -21.74 & - \\ \hline
\textit{C6} & \textit{C25} & 0.08 & 0.28 & -9.46 & - \\ \hline
\textit{C9} & \textit{C14} & 0.11 & 0.22 & -36.01 & - \\ \hline
\textit{C9} & \textit{C17} & 0.06 & 0.11 & -16.34 & - \\ \hline
\textit{C9} & \textit{C20} & 0.03 & 0.11 & -10.53 & - \\ \hline
\textit{C9} & \textit{C22} & 0.08 & 0.18 & -7.53 & - \\ \hline
\textit{C9} & \textit{C23} & 0.04 & 0.12 & -10.5 & - \\ \hline
\textit{C9} & \textit{C25} & 0.1 & 0.16 & -21.25 & - \\ \hline
\textit{C14} & \textit{C17} & 0.14 & 0.22 & -65.29 & - \\ \hline
\textit{C14} & \textit{C20} & 0.13 & 0.2 & -38.31 & - \\ \hline
\textit{C14} & \textit{C22} & 0.15 & 0.26 & -37.84 & - \\ \hline
\textit{C14} & \textit{C23} & 0.16 & 0.24 & -66.83 & - \\ \hline
\textit{C14} & \textit{C25} & 0.13 & 0.26 & -26.84 & - \\ \hline
\textit{C17} & \textit{C20} & 0.02 & 0.06 & -3.74 & - \\ \hline
\textit{C17} & \textit{C22} & 0.11 & 0.25 & -15.52 & - \\ \hline
\textit{C17} & \textit{C23} & 0.06 & 0.09 & -10.64 & - \\ \hline
\textit{C17} & \textit{C25} & 0.11 & 0.21 & -25.85 & - \\ \hline
\textit{C20} & \textit{C22} & 0.05 & 0.29 & -4.91 & - \\ \hline
\textit{C20} & \textit{C23} & 0.16 & 0.11 & -78.7 & - \\ \hline
\textit{C20} & \textit{C25} & 0.08 & 0.25 & -11.92 & - \\ \hline
\textit{C22} & \textit{C23} & 0.11 & 0.26 & -21.53 & - \\ \hline
\textit{C22} & \textit{C25} & 0.08 & 0.31 & -9.01 & - \\ \hline
\textit{C23} & \textit{C25} & 0.12 & 0.24 & -27.2 & - \\ \hline
\end{longtable}
\end{centering}
\end{small}

==> table_4.tex <==
\begin{centering}
\begin{small}
\begin{longtable}{|l|l|l|l|l|l|}
\caption{Bag Separation Statistics and their clusters on all groupings}
\label{tab:bag_sep_stats}
\hline
\textbf{Col1} & \textbf{Col2} & \textbf{MeanInterBagSep} & \textbf{MeanIntraBagSep} & \textbf{InterIntraRatio} & \textbf{Clusters assigned based on InterIntraRatio distribution} \\ \hline
\textit{C1} & \textit{-} & 0.83 & 0.82 & 1.02 & Less-separated \\ \hline
\textit{C3} & \textit{-} & 0.81 & 0.7 & 1.16 & Medium-separated \\ \hline
\textit{C4} & \textit{-} & 0.81 & 0.7 & 1.16 & Medium-separated \\ \hline
\textit{C7} & \textit{-} & 0.81 & 0.61 & 1.33 & Well-separated \\ \hline
\textit{C8} & \textit{-} & 0.83 & 0.81 & 1.02 & Less-separated \\ \hline
\textit{C10} & \textit{-} & 0.82 & 0.7 & 1.18 & Medium-separated \\ \hline
\textit{C11} & \textit{-} & 0.75 & 0.63 & 1.2 & Medium-separated \\ \hline
\textit{C12} & \textit{-} & 0.81 & 0.7 & 1.16 & Medium-separated \\ \hline
\textit{C13} & \textit{-} & 0.72 & 0.65 & 1.1 & Less-separated \\ \hline
\textit{C15} & \textit{-} & 0.8 & 0.7 & 1.15 & Medium-separated \\ \hline
\textit{C16} & \textit{-} & 0.81 & 0.7 & 1.16 & Medium-separated \\ \hline
\textit{C18} & \textit{-} & 0.79 & 0.71 & 1.12 & Medium-separated \\ \hline
\textit{C19} & \textit{-} & 0.78 & 0.76 & 1.03 & Less-separated \\ \hline
\textit{C21} & \textit{-} & 0.81 & 0.7 & 1.16 & Medium-separated \\ \hline
\textit{C24} & \textit{-} & 0.82 & 0.72 & 1.14 & Medium-separated \\ \hline
\textit{C26} & \textit{-} & 0.79 & 0.7 & 1.12 & Medium-separated \\ \hline
\textit{C1} & \textit{C2} & 0.81 & 0.74 & 1.1 & Less-separated \\ \hline
\textit{C1} & \textit{C3} & 0.83 & 0.72 & 1.15 & Medium-separated \\ \hline
\textit{C1} & \textit{C4} & 0.82 & 0.72 & 1.14 & Medium-separated \\ \hline
\textit{C1} & \textit{C5} & 0.83 & 0.81 & 1.02 & Less-separated \\ \hline
\textit{C1} & \textit{C6} & 0.82 & 0.79 & 1.03 & Less-separated \\ \hline
\textit{C1} & \textit{C7} & 0.81 & 0.6 & 1.34 & Well-separated \\ \hline
\textit{C1} & \textit{C8} & 0.83 & 0.81 & 1.02 & Less-separated \\ \hline
\textit{C1} & \textit{C9} & 0.9 & 0.8 & 1.12 & Medium-separated \\ \hline
\textit{C1} & \textit{C10} & 0.82 & 0.73 & 1.14 & Medium-separated \\ \hline
\textit{C1} & \textit{C11} & 0.79 & 0.68 & 1.17 & Medium-separated \\ \hline
\textit{C1} & \textit{C12} & 0.83 & 0.72 & 1.15 & Medium-separated \\ \hline
\textit{C1} & \textit{C13} & 0.79 & 0.7 & 1.13 & Medium-separated \\ \hline
\textit{C1} & \textit{C14} & 0.82 & 0.78 & 1.05 & Less-separated \\ \hline
\textit{C1} & \textit{C15} & 0.82 & 0.72 & 1.14 & Medium-separated \\ \hline
\textit{C1} & \textit{C16} & 0.82 & 0.72 & 1.15 & Medium-separated \\ \hline
\textit{C1} & \textit{C17} & 0.86 & 0.73 & 1.17 & Medium-separated \\ \hline
\textit{C1} & \textit{C18} & 0.81 & 0.73 & 1.12 & Medium-separated \\ \hline
\textit{C1} & \textit{C19} & 0.8 & 0.77 & 1.04 & Less-separated \\ \hline
\textit{C1} & \textit{C20} & 0.83 & 0.81 & 1.03 & Less-separated \\ \hline
\textit{C1} & \textit{C21} & 0.83 & 0.72 & 1.15 & Medium-separated \\ \hline
\textit{C1} & \textit{C22} & 0.83 & 0.81 & 1.02 & Less-separated \\ \hline
\textit{C1} & \textit{C23} & 0.84 & 0.8 & 1.05 & Less-separated \\ \hline
\textit{C1} & \textit{C24} & 0.83 & 0.73 & 1.13 & Medium-separated \\ \hline
\textit{C1} & \textit{C25} & 0.83 & 0.8 & 1.04 & Less-separated \\ \hline
\textit{C1} & \textit{C26} & 0.81 & 0.72 & 1.12 & Medium-separated \\ \hline
\textit{C2} & \textit{C3} & 0.82 & 0.69 & 1.19 & Medium-separated \\ \hline
\textit{C2} & \textit{C4} & 0.82 & 0.69 & 1.18 & Medium-separated \\ \hline
\textit{C2} & \textit{C5} & 0.81 & 0.73 & 1.1 & Less-separated \\ \hline
\textit{C2} & \textit{C6} & 0.74 & 0.66 & 1.13 & Medium-separated \\ \hline
\textit{C2} & \textit{C7} & 0.78 & 0.55 & 1.44 & Far-separated \\ \hline
\textit{C2} & \textit{C8} & 0.81 & 0.74 & 1.1 & Less-separated \\ \hline
\textit{C2} & \textit{C10} & 0.81 & 0.67 & 1.21 & Medium-separated \\ \hline
\textit{C2} & \textit{C11} & 0.76 & 0.6 & 1.26 & Well-separated \\ \hline
\textit{C2} & \textit{C12} & 0.82 & 0.69 & 1.19 & Medium-separated \\ \hline
\textit{C2} & \textit{C13} & 0.75 & 0.62 & 1.22 & Medium-separated \\ \hline
\textit{C2} & \textit{C14} & 0.76 & 0.68 & 1.13 & Medium-separated \\ \hline
\textit{C2} & \textit{C15} & 0.8 & 0.7 & 1.15 & Medium-separated \\ \hline
\textit{C2} & \textit{C16} & 0.82 & 0.69 & 1.18 & Medium-separated \\ \hline
\textit{C2} & \textit{C17} & 0.81 & 0.6 & 1.34 & Well-separated \\ \hline
\textit{C2} & \textit{C18} & 0.79 & 0.71 & 1.12 & Medium-separated \\ \hline
\textit{C2} & \textit{C19} & 0.78 & 0.72 & 1.09 & Less-separated \\ \hline
\textit{C2} & \textit{C21} & 0.82 & 0.69 & 1.19 & Medium-separated \\ \hline
\textit{C2} & \textit{C22} & 0.77 & 0.69 & 1.12 & Medium-separated \\ \hline
\textit{C2} & \textit{C23} & 0.79 & 0.66 & 1.2 & Medium-separated \\ \hline
\textit{C2} & \textit{C24} & 0.83 & 0.71 & 1.17 & Medium-separated \\ \hline
\textit{C2} & \textit{C25} & 0.85 & 0.78 & 1.09 & Less-separated \\ \hline
\textit{C2} & \textit{C26} & 0.8 & 0.7 & 1.14 & Medium-separated \\ \hline
\textit{C3} & \textit{C4} & 0.8 & 0.69 & 1.16 & Medium-separated \\ \hline
\textit{C3} & \textit{C5} & 0.82 & 0.71 & 1.16 & Medium-separated \\ \hline
\textit{C3} & \textit{C6} & 0.82 & 0.7 & 1.18 & Medium-separated \\ \hline
\textit{C3} & \textit{C7} & 0.84 & 0.54 & 1.56 & Far-separated \\ \hline
\textit{C3} & \textit{C8} & 0.83 & 0.72 & 1.15 & Medium-separated \\ \hline
\textit{C3} & \textit{C9} & 0.83 & 0.64 & 1.3 & Well-separated \\ \hline
\textit{C3} & \textit{C10} & 0.83 & 0.67 & 1.25 & Well-separated \\ \hline
\textit{C3} & \textit{C11} & 0.84 & 0.62 & 1.35 & Well-separated \\ \hline
\textit{C3} & \textit{C12} & 0.81 & 0.7 & 1.16 & Medium-separated \\ \hline
\textit{C3} & \textit{C13} & 0.84 & 0.63 & 1.32 & Well-separated \\ \hline
\textit{C3} & \textit{C14} & 0.82 & 0.69 & 1.19 & Medium-separated \\ \hline
\textit{C3} & \textit{C15} & 0.83 & 0.69 & 1.21 & Medium-separated \\ \hline
\textit{C3} & \textit{C16} & 0.8 & 0.69 & 1.16 & Medium-separated \\ \hline
\textit{C3} & \textit{C17} & 0.83 & 0.64 & 1.28 & Well-separated \\ \hline
\textit{C3} & \textit{C18} & 0.82 & 0.69 & 1.19 & Medium-separated \\ \hline
\textit{C3} & \textit{C19} & 0.82 & 0.7 & 1.17 & Medium-separated \\ \hline
\textit{C3} & \textit{C20} & 0.82 & 0.69 & 1.18 & Medium-separated \\ \hline
\textit{C3} & \textit{C21} & 0.81 & 0.7 & 1.16 & Medium-separated \\ \hline
\textit{C3} & \textit{C22} & 0.82 & 0.7 & 1.17 & Medium-separated \\ \hline
\textit{C3} & \textit{C23} & 0.83 & 0.68 & 1.22 & Medium-separated \\ \hline
\textit{C3} & \textit{C24} & 0.81 & 0.7 & 1.16 & Medium-separated \\ \hline
\textit{C3} & \textit{C25} & 0.82 & 0.7 & 1.17 & Medium-separated \\ \hline
\textit{C3} & \textit{C26} & 0.81 & 0.69 & 1.17 & Medium-separated \\ \hline
\textit{C4} & \textit{C5} & 0.82 & 0.71 & 1.15 & Medium-separated \\ \hline
\textit{C4} & \textit{C6} & 0.81 & 0.69 & 1.17 & Medium-separated \\ \hline
\textit{C4} & \textit{C7} & 0.83 & 0.53 & 1.55 & Far-separated \\ \hline
\textit{C4} & \textit{C8} & 0.82 & 0.71 & 1.15 & Medium-separated \\ \hline
\textit{C4} & \textit{C9} & 0.85 & 0.64 & 1.33 & Well-separated \\ \hline
\textit{C4} & \textit{C10} & 0.83 & 0.66 & 1.26 & Well-separated \\ \hline
\textit{C4} & \textit{C11} & 0.82 & 0.62 & 1.34 & Well-separated \\ \hline
\textit{C4} & \textit{C12} & 0.8 & 0.69 & 1.16 & Medium-separated \\ \hline
\textit{C4} & \textit{C13} & 0.82 & 0.63 & 1.31 & Well-separated \\ \hline
\textit{C4} & \textit{C14} & 0.81 & 0.69 & 1.18 & Medium-separated \\ \hline
\textit{C4} & \textit{C15} & 0.82 & 0.68 & 1.2 & Medium-separated \\ \hline
\textit{C4} & \textit{C16} & 0.81 & 0.7 & 1.16 & Medium-separated \\ \hline
\textit{C4} & \textit{C17} & 0.82 & 0.64 & 1.28 & Well-separated \\ \hline
\textit{C4} & \textit{C18} & 0.82 & 0.69 & 1.18 & Medium-separated \\ \hline
\textit{C4} & \textit{C19} & 0.81 & 0.7 & 1.16 & Medium-separated \\ \hline
\textit{C4} & \textit{C20} & 0.81 & 0.69 & 1.17 & Medium-separated \\ \hline
\textit{C4} & \textit{C21} & 0.8 & 0.7 & 1.16 & Medium-separated \\ \hline
\textit{C4} & \textit{C22} & 0.82 & 0.7 & 1.16 & Medium-separated \\ \hline
\textit{C4} & \textit{C23} & 0.82 & 0.68 & 1.21 & Medium-separated \\ \hline
\textit{C4} & \textit{C24} & 0.81 & 0.7 & 1.15 & Medium-separated \\ \hline
\textit{C4} & \textit{C25} & 0.82 & 0.7 & 1.16 & Medium-separated \\ \hline
\textit{C4} & \textit{C26} & 0.81 & 0.69 & 1.17 & Medium-separated \\ \hline
\textit{C5} & \textit{C6} & 0.81 & 0.79 & 1.03 & Less-separated \\ \hline
\textit{C5} & \textit{C7} & 0.81 & 0.6 & 1.34 & Well-separated \\ \hline
\textit{C5} & \textit{C8} & 0.83 & 0.81 & 1.02 & Less-separated \\ \hline
\textit{C5} & \textit{C10} & 0.82 & 0.72 & 1.14 & Medium-separated \\ \hline
\textit{C5} & \textit{C11} & 0.79 & 0.67 & 1.17 & Medium-separated \\ \hline
\textit{C5} & \textit{C12} & 0.82 & 0.71 & 1.16 & Medium-separated \\ \hline
\textit{C5} & \textit{C13} & 0.78 & 0.7 & 1.12 & Medium-separated \\ \hline
\textit{C5} & \textit{C14} & 0.82 & 0.77 & 1.05 & Less-separated \\ \hline
\textit{C5} & \textit{C15} & 0.82 & 0.71 & 1.14 & Medium-separated \\ \hline
\textit{C5} & \textit{C16} & 0.82 & 0.71 & 1.15 & Medium-separated \\ \hline
\textit{C5} & \textit{C17} & 0.88 & 0.73 & 1.21 & Medium-separated \\ \hline
\textit{C5} & \textit{C18} & 0.81 & 0.72 & 1.12 & Medium-separated \\ \hline
\textit{C5} & \textit{C19} & 0.79 & 0.76 & 1.04 & Less-separated \\ \hline
\textit{C5} & \textit{C21} & 0.82 & 0.71 & 1.16 & Medium-separated \\ \hline
\textit{C5} & \textit{C23} & 0.84 & 0.8 & 1.06 & Less-separated \\ \hline
\textit{C5} & \textit{C24} & 0.83 & 0.73 & 1.14 & Medium-separated \\ \hline
\textit{C5} & \textit{C25} & 0.82 & 0.79 & 1.04 & Less-separated \\ \hline
\textit{C5} & \textit{C26} & 0.8 & 0.72 & 1.12 & Medium-separated \\ \hline
\textit{C6} & \textit{C7} & 0.78 & 0.58 & 1.36 & Well-separated \\ \hline
\textit{C6} & \textit{C8} & 0.82 & 0.79 & 1.03 & Less-separated \\ \hline
\textit{C6} & \textit{C10} & 0.81 & 0.7 & 1.17 & Medium-separated \\ \hline
\textit{C6} & \textit{C11} & 0.75 & 0.63 & 1.19 & Medium-separated \\ \hline
\textit{C6} & \textit{C12} & 0.82 & 0.69 & 1.18 & Medium-separated \\ \hline
\textit{C6} & \textit{C13} & 0.73 & 0.64 & 1.14 & Medium-separated \\ \hline
\textit{C6} & \textit{C15} & 0.79 & 0.67 & 1.17 & Medium-separated \\ \hline
\textit{C6} & \textit{C16} & 0.81 & 0.69 & 1.18 & Medium-separated \\ \hline
\textit{C6} & \textit{C18} & 0.77 & 0.67 & 1.15 & Medium-separated \\ \hline
\textit{C6} & \textit{C19} & 0.77 & 0.72 & 1.06 & Less-separated \\ \hline
\textit{C6} & \textit{C21} & 0.82 & 0.69 & 1.18 & Medium-separated \\ \hline
\textit{C6} & \textit{C24} & 0.82 & 0.7 & 1.16 & Medium-separated \\ \hline
\textit{C6} & \textit{C26} & 0.8 & 0.69 & 1.15 & Medium-separated \\ \hline
\textit{C7} & \textit{C8} & 0.81 & 0.6 & 1.34 & Well-separated \\ \hline
\textit{C7} & \textit{C9} & 0.81 & 0.61 & 1.33 & Well-separated \\ \hline
\textit{C7} & \textit{C10} & 0.84 & 0.6 & 1.41 & Far-separated \\ \hline
\textit{C7} & \textit{C11} & 0.81 & 0.6 & 1.35 & Well-separated \\ \hline
\textit{C7} & \textit{C12} & 0.84 & 0.54 & 1.56 & Far-separated \\ \hline
\textit{C7} & \textit{C13} & 0.81 & 0.61 & 1.33 & Well-separated \\ \hline
\textit{C7} & \textit{C14} & 0.79 & 0.57 & 1.38 & Well-separated \\ \hline
\textit{C7} & \textit{C15} & 0.81 & 0.53 & 1.54 & Far-separated \\ \hline
\textit{C7} & \textit{C16} & 0.83 & 0.54 & 1.56 & Far-separated \\ \hline
\textit{C7} & \textit{C17} & 0.83 & 0.58 & 1.43 & Far-separated \\ \hline
\textit{C7} & \textit{C18} & 0.8 & 0.53 & 1.51 & Far-separated \\ \hline
\textit{C7} & \textit{C19} & 0.82 & 0.58 & 1.4 & Well-separated \\ \hline
\textit{C7} & \textit{C20} & 0.8 & 0.58 & 1.38 & Well-separated \\ \hline
\textit{C7} & \textit{C21} & 0.84 & 0.54 & 1.56 & Far-separated \\ \hline
\textit{C7} & \textit{C22} & 0.81 & 0.6 & 1.36 & Well-separated \\ \hline
\textit{C7} & \textit{C23} & 0.82 & 0.59 & 1.4 & Well-separated \\ \hline
\textit{C7} & \textit{C24} & 0.83 & 0.54 & 1.53 & Far-separated \\ \hline
\textit{C7} & \textit{C25} & 0.8 & 0.59 & 1.36 & Well-separated \\ \hline
\textit{C7} & \textit{C26} & 0.84 & 0.55 & 1.54 & Far-separated \\ \hline
\textit{C8} & \textit{C9} & 0.92 & 0.81 & 1.14 & Medium-separated \\ \hline
\textit{C8} & \textit{C10} & 0.83 & 0.72 & 1.14 & Medium-separated \\ \hline
\textit{C8} & \textit{C11} & 0.79 & 0.68 & 1.17 & Medium-separated \\ \hline
\textit{C8} & \textit{C12} & 0.82 & 0.71 & 1.15 & Medium-separated \\ \hline
\textit{C8} & \textit{C13} & 0.78 & 0.7 & 1.12 & Medium-separated \\ \hline
\textit{C8} & \textit{C14} & 0.82 & 0.78 & 1.05 & Less-separated \\ \hline
\textit{C8} & \textit{C15} & 0.82 & 0.72 & 1.14 & Medium-separated \\ \hline
\textit{C8} & \textit{C16} & 0.82 & 0.71 & 1.15 & Medium-separated \\ \hline
\textit{C8} & \textit{C17} & 0.87 & 0.73 & 1.19 & Medium-separated \\ \hline
\textit{C8} & \textit{C18} & 0.81 & 0.72 & 1.12 & Medium-separated \\ \hline
\textit{C8} & \textit{C19} & 0.79 & 0.76 & 1.04 & Less-separated \\ \hline
\textit{C8} & \textit{C20} & 0.83 & 0.8 & 1.03 & Less-separated \\ \hline
\textit{C8} & \textit{C21} & 0.82 & 0.71 & 1.15 & Medium-separated \\ \hline
\textit{C8} & \textit{C22} & 0.83 & 0.81 & 1.02 & Less-separated \\ \hline
\textit{C8} & \textit{C23} & 0.84 & 0.8 & 1.05 & Less-separated \\ \hline
\textit{C8} & \textit{C24} & 0.83 & 0.73 & 1.13 & Medium-separated \\ \hline
\textit{C8} & \textit{C25} & 0.82 & 0.79 & 1.04 & Less-separated \\ \hline
\textit{C8} & \textit{C26} & 0.81 & 0.72 & 1.12 & Medium-separated \\ \hline
\textit{C9} & \textit{C10} & 0.88 & 0.6 & 1.46 & Far-separated \\ \hline
\textit{C9} & \textit{C11} & 0.86 & 0.58 & 1.48 & Far-separated \\ \hline
\textit{C9} & \textit{C12} & 0.83 & 0.64 & 1.3 & Well-separated \\ \hline
\textit{C9} & \textit{C13} & 0.88 & 0.6 & 1.48 & Far-separated \\ \hline
\textit{C9} & \textit{C15} & 0.97 & 0.68 & 1.44 & Far-separated \\ \hline
\textit{C9} & \textit{C16} & 0.84 & 0.64 & 1.31 & Well-separated \\ \hline
\textit{C9} & \textit{C18} & 0.98 & 0.71 & 1.38 & Well-separated \\ \hline
\textit{C9} & \textit{C19} & 0.99 & 0.69 & 1.44 & Far-separated \\ \hline
\textit{C9} & \textit{C21} & 0.83 & 0.64 & 1.3 & Well-separated \\ \hline
\textit{C9} & \textit{C24} & 0.9 & 0.66 & 1.36 & Well-separated \\ \hline
\textit{C9} & \textit{C26} & 0.86 & 0.63 & 1.37 & Well-separated \\ \hline
\textit{C10} & \textit{C11} & 0.83 & 0.68 & 1.22 & Medium-separated \\ \hline
\textit{C10} & \textit{C12} & 0.83 & 0.66 & 1.25 & Well-separated \\ \hline
\textit{C10} & \textit{C13} & 0.83 & 0.69 & 1.21 & Medium-separated \\ \hline
\textit{C10} & \textit{C14} & 0.82 & 0.7 & 1.17 & Medium-separated \\ \hline
\textit{C10} & \textit{C15} & 0.82 & 0.65 & 1.25 & Well-separated \\ \hline
\textit{C10} & \textit{C16} & 0.83 & 0.66 & 1.25 & Well-separated \\ \hline
\textit{C10} & \textit{C17} & 0.84 & 0.68 & 1.23 & Medium-separated \\ \hline
\textit{C10} & \textit{C18} & 0.81 & 0.66 & 1.23 & Medium-separated \\ \hline
\textit{C10} & \textit{C19} & 0.84 & 0.69 & 1.2 & Medium-separated \\ \hline
\textit{C10} & \textit{C20} & 0.83 & 0.7 & 1.18 & Medium-separated \\ \hline
\textit{C10} & \textit{C21} & 0.83 & 0.66 & 1.25 & Well-separated \\ \hline
\textit{C10} & \textit{C22} & 0.83 & 0.71 & 1.16 & Medium-separated \\ \hline
\textit{C10} & \textit{C23} & 0.84 & 0.68 & 1.24 & Medium-separated \\ \hline
\textit{C10} & \textit{C24} & 0.83 & 0.67 & 1.24 & Medium-separated \\ \hline
\textit{C10} & \textit{C25} & 0.82 & 0.7 & 1.18 & Medium-separated \\ \hline
\textit{C10} & \textit{C26} & 0.84 & 0.67 & 1.26 & Well-separated \\ \hline
\textit{C11} & \textit{C12} & 0.83 & 0.62 & 1.35 & Well-separated \\ \hline
\textit{C11} & \textit{C13} & 0.75 & 0.63 & 1.2 & Medium-separated \\ \hline
\textit{C11} & \textit{C14} & 0.75 & 0.62 & 1.2 & Medium-separated \\ \hline
\textit{C11} & \textit{C15} & 0.8 & 0.6 & 1.33 & Well-separated \\ \hline
\textit{C11} & \textit{C16} & 0.83 & 0.62 & 1.34 & Well-separated \\ \hline
\textit{C11} & \textit{C17} & 0.78 & 0.63 & 1.24 & Medium-separated \\ \hline
\textit{C11} & \textit{C18} & 0.78 & 0.6 & 1.32 & Well-separated \\ \hline
\textit{C11} & \textit{C19} & 0.79 & 0.65 & 1.2 & Medium-separated \\ \hline
\textit{C11} & \textit{C20} & 0.76 & 0.63 & 1.21 & Medium-separated \\ \hline
\textit{C11} & \textit{C21} & 0.83 & 0.62 & 1.35 & Well-separated \\ \hline
\textit{C11} & \textit{C22} & 0.77 & 0.65 & 1.19 & Medium-separated \\ \hline
\textit{C11} & \textit{C23} & 0.81 & 0.64 & 1.26 & Well-separated \\ \hline
\textit{C11} & \textit{C24} & 0.82 & 0.62 & 1.31 & Well-separated \\ \hline
\textit{C11} & \textit{C25} & 0.78 & 0.64 & 1.2 & Medium-separated \\ \hline
\textit{C11} & \textit{C26} & 0.83 & 0.63 & 1.31 & Well-separated \\ \hline
\textit{C12} & \textit{C13} & 0.83 & 0.63 & 1.32 & Well-separated \\ \hline
\textit{C12} & \textit{C14} & 0.82 & 0.69 & 1.18 & Medium-separated \\ \hline
\textit{C12} & \textit{C15} & 0.83 & 0.69 & 1.2 & Medium-separated \\ \hline
\textit{C12} & \textit{C16} & 0.8 & 0.69 & 1.16 & Medium-separated \\ \hline
\textit{C12} & \textit{C17} & 0.82 & 0.64 & 1.28 & Well-separated \\ \hline
\textit{C12} & \textit{C18} & 0.82 & 0.69 & 1.19 & Medium-separated \\ \hline
\textit{C12} & \textit{C19} & 0.81 & 0.7 & 1.17 & Medium-separated \\ \hline
\textit{C12} & \textit{C20} & 0.81 & 0.69 & 1.18 & Medium-separated \\ \hline
\textit{C12} & \textit{C21} & 0.81 & 0.7 & 1.16 & Medium-separated \\ \hline
\textit{C12} & \textit{C22} & 0.82 & 0.7 & 1.17 & Medium-separated \\ \hline
\textit{C12} & \textit{C23} & 0.83 & 0.68 & 1.22 & Medium-separated \\ \hline
\textit{C12} & \textit{C24} & 0.81 & 0.7 & 1.15 & Medium-separated \\ \hline
\textit{C12} & \textit{C25} & 0.82 & 0.7 & 1.17 & Medium-separated \\ \hline
\textit{C12} & \textit{C26} & 0.81 & 0.69 & 1.17 & Medium-separated \\ \hline
\textit{C13} & \textit{C14} & 0.74 & 0.64 & 1.15 & Medium-separated \\ \hline
\textit{C13} & \textit{C15} & 0.79 & 0.61 & 1.3 & Well-separated \\ \hline
\textit{C13} & \textit{C16} & 0.83 & 0.63 & 1.32 & Well-separated \\ \hline
\textit{C13} & \textit{C17} & 0.78 & 0.64 & 1.21 & Medium-separated \\ \hline
\textit{C13} & \textit{C18} & 0.78 & 0.61 & 1.28 & Well-separated \\ \hline
\textit{C13} & \textit{C19} & 0.78 & 0.66 & 1.18 & Medium-separated \\ \hline
\textit{C13} & \textit{C20} & 0.74 & 0.65 & 1.14 & Medium-separated \\ \hline
\textit{C13} & \textit{C21} & 0.83 & 0.63 & 1.32 & Well-separated \\ \hline
\textit{C13} & \textit{C22} & 0.76 & 0.67 & 1.13 & Medium-separated \\ \hline
\textit{C13} & \textit{C23} & 0.8 & 0.65 & 1.23 & Medium-separated \\ \hline
\textit{C13} & \textit{C24} & 0.82 & 0.64 & 1.28 & Well-separated \\ \hline
\textit{C13} & \textit{C25} & 0.77 & 0.67 & 1.15 & Medium-separated \\ \hline
\textit{C13} & \textit{C26} & 0.83 & 0.64 & 1.29 & Well-separated \\ \hline
\textit{C14} & \textit{C15} & 0.8 & 0.7 & 1.15 & Medium-separated \\ \hline
\textit{C14} & \textit{C16} & 0.82 & 0.69 & 1.18 & Medium-separated \\ \hline
\textit{C14} & \textit{C18} & 0.79 & 0.69 & 1.14 & Medium-separated \\ \hline
\textit{C14} & \textit{C19} & 0.78 & 0.72 & 1.07 & Less-separated \\ \hline
\textit{C14} & \textit{C21} & 0.82 & 0.69 & 1.19 & Medium-separated \\ \hline
\textit{C14} & \textit{C24} & 0.82 & 0.7 & 1.17 & Medium-separated \\ \hline
\textit{C14} & \textit{C26} & 0.8 & 0.69 & 1.15 & Medium-separated \\ \hline
\textit{C15} & \textit{C16} & 0.82 & 0.68 & 1.21 & Medium-separated \\ \hline
\textit{C15} & \textit{C17} & 0.82 & 0.61 & 1.35 & Well-separated \\ \hline
\textit{C15} & \textit{C18} & 0.8 & 0.7 & 1.15 & Medium-separated \\ \hline
\textit{C15} & \textit{C19} & 0.8 & 0.7 & 1.14 & Medium-separated \\ \hline
\textit{C15} & \textit{C20} & 0.81 & 0.7 & 1.15 & Medium-separated \\ \hline
\textit{C15} & \textit{C21} & 0.83 & 0.68 & 1.21 & Medium-separated \\ \hline
\textit{C15} & \textit{C22} & 0.81 & 0.7 & 1.16 & Medium-separated \\ \hline
\textit{C15} & \textit{C23} & 0.82 & 0.66 & 1.24 & Medium-separated \\ \hline
\textit{C15} & \textit{C24} & 0.83 & 0.7 & 1.19 & Medium-separated \\ \hline
\textit{C15} & \textit{C25} & 0.82 & 0.72 & 1.14 & Medium-separated \\ \hline
\textit{C15} & \textit{C26} & 0.82 & 0.7 & 1.18 & Medium-separated \\ \hline
\textit{C16} & \textit{C17} & 0.82 & 0.64 & 1.28 & Well-separated \\ \hline
\textit{C16} & \textit{C18} & 0.82 & 0.69 & 1.19 & Medium-separated \\ \hline
\textit{C16} & \textit{C19} & 0.82 & 0.7 & 1.17 & Medium-separated \\ \hline
\textit{C16} & \textit{C20} & 0.81 & 0.69 & 1.18 & Medium-separated \\ \hline
\textit{C16} & \textit{C21} & 0.81 & 0.7 & 1.16 & Medium-separated \\ \hline
\textit{C16} & \textit{C22} & 0.82 & 0.7 & 1.16 & Medium-separated \\ \hline
\textit{C16} & \textit{C23} & 0.82 & 0.68 & 1.22 & Medium-separated \\ \hline
\textit{C16} & \textit{C24} & 0.81 & 0.7 & 1.15 & Medium-separated \\ \hline
\textit{C16} & \textit{C25} & 0.82 & 0.7 & 1.17 & Medium-separated \\ \hline
\textit{C16} & \textit{C26} & 0.81 & 0.69 & 1.17 & Medium-separated \\ \hline
\textit{C17} & \textit{C18} & 0.81 & 0.6 & 1.34 & Well-separated \\ \hline
\textit{C17} & \textit{C19} & 0.81 & 0.7 & 1.16 & Medium-separated \\ \hline
\textit{C17} & \textit{C21} & 0.82 & 0.64 & 1.28 & Well-separated \\ \hline
\textit{C17} & \textit{C24} & 0.83 & 0.66 & 1.27 & Well-separated \\ \hline
\textit{C17} & \textit{C26} & 0.81 & 0.66 & 1.24 & Medium-separated \\ \hline
\textit{C18} & \textit{C19} & 0.79 & 0.71 & 1.11 & Medium-separated \\ \hline
\textit{C18} & \textit{C20} & 0.79 & 0.71 & 1.12 & Medium-separated \\ \hline
\textit{C18} & \textit{C21} & 0.82 & 0.69 & 1.19 & Medium-separated \\ \hline
\textit{C18} & \textit{C22} & 0.8 & 0.71 & 1.13 & Medium-separated \\ \hline
\textit{C18} & \textit{C23} & 0.81 & 0.67 & 1.21 & Medium-separated \\ \hline
\textit{C18} & \textit{C24} & 0.82 & 0.7 & 1.17 & Medium-separated \\ \hline
\textit{C18} & \textit{C25} & 0.83 & 0.74 & 1.12 & Medium-separated \\ \hline
\textit{C18} & \textit{C26} & 0.81 & 0.7 & 1.15 & Medium-separated \\ \hline
\textit{C19} & \textit{C20} & 0.78 & 0.73 & 1.06 & Less-separated \\ \hline
\textit{C19} & \textit{C21} & 0.82 & 0.7 & 1.17 & Medium-separated \\ \hline
\textit{C19} & \textit{C22} & 0.8 & 0.76 & 1.05 & Less-separated \\ \hline
\textit{C19} & \textit{C23} & 0.78 & 0.73 & 1.07 & Less-separated \\ \hline
\textit{C19} & \textit{C24} & 0.82 & 0.71 & 1.15 & Medium-separated \\ \hline
\textit{C19} & \textit{C25} & 0.78 & 0.72 & 1.08 & Less-separated \\ \hline
\textit{C19} & \textit{C26} & 0.8 & 0.7 & 1.13 & Medium-separated \\ \hline
\textit{C20} & \textit{C21} & 0.81 & 0.69 & 1.18 & Medium-separated \\ \hline
\textit{C20} & \textit{C24} & 0.82 & 0.7 & 1.16 & Medium-separated \\ \hline
\textit{C20} & \textit{C26} & 0.79 & 0.7 & 1.14 & Medium-separated \\ \hline
\textit{C21} & \textit{C22} & 0.82 & 0.7 & 1.17 & Medium-separated \\ \hline
\textit{C21} & \textit{C23} & 0.83 & 0.68 & 1.22 & Medium-separated \\ \hline
\textit{C21} & \textit{C24} & 0.81 & 0.7 & 1.15 & Medium-separated \\ \hline
\textit{C21} & \textit{C25} & 0.82 & 0.7 & 1.17 & Medium-separated \\ \hline
\textit{C21} & \textit{C26} & 0.81 & 0.69 & 1.17 & Medium-separated \\ \hline
\textit{C22} & \textit{C24} & 0.83 & 0.72 & 1.15 & Medium-separated \\ \hline
\textit{C22} & \textit{C26} & 0.8 & 0.71 & 1.14 & Medium-separated \\ \hline
\textit{C23} & \textit{C24} & 0.83 & 0.7 & 1.19 & Medium-separated \\ \hline
\textit{C23} & \textit{C26} & 0.8 & 0.68 & 1.18 & Medium-separated \\ \hline
\textit{C24} & \textit{C25} & 0.83 & 0.72 & 1.15 & Medium-separated \\ \hline
\textit{C24} & \textit{C26} & 0.82 & 0.71 & 1.16 & Medium-separated \\ \hline
\textit{C25} & \textit{C26} & 0.8 & 0.71 & 1.13 & Medium-separated \\ \hline
\textit{C2} & \textit{-} & 0.73 & 0.64 & 1.14 & - \\ \hline
\textit{C5} & \textit{-} & 0.82 & 0.8 & 1.02 & - \\ \hline
\textit{C6} & \textit{-} & 0.85 & 0.65 & 1.32 & - \\ \hline
\textit{C14} & \textit{-} & 0.78 & 0.71 & 1.11 & - \\ \hline
\textit{C17} & \textit{-} &  & 0.55 &  & - \\ \hline
\textit{C22} & \textit{-} & 0.87 & 0.84 & 1.04 & - \\ \hline
\textit{C23} & \textit{-} &  & 0.53 &  & - \\ \hline
\textit{C25} & \textit{-} & 0.82 & 0.78 & 1.05 & - \\ \hline
\textit{C2} & \textit{C9} & 0.96 & 0.68 & 1.42 & - \\ \hline
\textit{C2} & \textit{C20} & 0.76 & 0.67 & 1.13 & - \\ \hline
\textit{C5} & \textit{C9} & 0.94 & 0.82 & 1.14 & - \\ \hline
\textit{C5} & \textit{C20} & 0.83 & 0.81 & 1.03 & - \\ \hline
\textit{C5} & \textit{C22} & 0.82 & 0.81 & 1.02 & - \\ \hline
\textit{C6} & \textit{C9} & 1 & 0.77 & 1.29 & - \\ \hline
\textit{C6} & \textit{C14} & 0.78 & 0.69 & 1.13 & - \\ \hline
\textit{C6} & \textit{C17} & 1.15 & 0.67 & 1.71 & - \\ \hline
\textit{C6} & \textit{C20} & 0.83 & 0.74 & 1.12 & - \\ \hline
\textit{C6} & \textit{C22} & 0.92 & 0.83 & 1.12 & - \\ \hline
\textit{C6} & \textit{C23} & 0.87 & 0.76 & 1.15 & - \\ \hline
\textit{C6} & \textit{C25} & 0.76 & 0.71 & 1.08 & - \\ \hline
\textit{C9} & \textit{C14} & 0.82 & 0.51 & 1.6 & - \\ \hline
\textit{C9} & \textit{C17} & 0.98 & 0.56 & 1.75 & - \\ \hline
\textit{C9} & \textit{C20} & 0.63 & 0.6 & 1.04 & - \\ \hline
\textit{C9} & \textit{C22} & 1.06 & 0.93 & 1.14 & - \\ \hline
\textit{C9} & \textit{C23} & 0.73 & 0.57 & 1.28 & - \\ \hline
\textit{C9} & \textit{C25} & 1.08 & 0.87 & 1.24 & - \\ \hline
\textit{C14} & \textit{C17} & 0.99 & 0.6 & 1.64 & - \\ \hline
\textit{C14} & \textit{C20} & 0.87 & 0.77 & 1.13 & - \\ \hline
\textit{C14} & \textit{C22} & 0.79 & 0.71 & 1.11 & - \\ \hline
\textit{C14} & \textit{C23} & 0.83 & 0.67 & 1.23 & - \\ \hline
\textit{C14} & \textit{C25} & 0.75 & 0.7 & 1.07 & - \\ \hline
\textit{C17} & \textit{C20} & 0.55 & 0.53 & 1.04 & - \\ \hline
\textit{C17} & \textit{C22} & 1.23 & 0.7 & 1.75 & - \\ \hline
\textit{C17} & \textit{C23} & 1.39 & 0.59 & 2.35 & - \\ \hline
\textit{C17} & \textit{C25} & 0.88 & 0.64 & 1.38 & - \\ \hline
\textit{C20} & \textit{C22} & 0.88 & 0.85 & 1.04 & - \\ \hline
\textit{C20} & \textit{C23} & 0.86 & 0.74 & 1.16 & - \\ \hline
\textit{C20} & \textit{C25} & 0.82 & 0.77 & 1.06 & - \\ \hline
\textit{C22} & \textit{C23} & 0.85 & 0.77 & 1.11 & - \\ \hline
\textit{C22} & \textit{C25} & 0.8 & 0.75 & 1.06 & - \\ \hline
\textit{C23} & \textit{C25} & 0.81 & 0.73 & 1.11 & - \\ \hline
\end{longtable}
\end{small}
\end{centering}

==> table_5.tex <==

\begin{small}
\begin{centering}
\tabcolsep=4pt\relax
\begin{longtable}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\caption{AUC Scores obtained after different training configurations for all groupings}
\label{tab:auc_scores}
\hline
\textbf{Col1} & \textbf{Col2} & \textbf{Expt1} & \textbf{Expt2} & \textbf{Expt3} & \textbf{Expt4} & \textbf{Expt5} & \textbf{Expt6} & \textbf{Expt7} & \textbf{Expt8} & \textbf{Expt9} & \textbf{Expt10} & \textbf{Expt11} \\ \hline
\textit{C1} & \textit{C7} & 74.88±0.04 & 74.95±0.03 & 74.76±0.04 & 74.78±0.03 & 65.88±0.1 & 64.19±0.1 & 66.84±0.25 & 64.88±0.21 & 69.94±0.62 & 69.81±0.47 & 65.03±0.8 \\ \hline
\textit{C1} & \textit{C10} & 73.64±0.05 & 73.67±0.05 & 73.6±0.06 & 73.61±0.04 & 65.03±0.11 & 63.43±0.1 & 65.55±0.22 & 63.97±0.23 & 70.4±0.17 & 70.23±0.18 & 61.98±0.38 \\ \hline
\textit{C2} & \textit{C7} & 75.63±0.02 & 75.63±0.02 & 75.42±0.04 & 75.44±0.03 & 68.74±0.1 & 67.34±0.1 & 69.33±0.09 & 67.99±0.17 & 70.76±0.11 & 70.42±0.16 & 67.2±1.0 \\ \hline
\textit{C2} & \textit{C10} & 74.45±0.04 & 74.43±0.04 & 74.3±0.04 & 74.29±0.05 & 67.98±0.1 & 66.85±0.14 & 68.57±0.14 & 67.41±0.08 & 70.23±0.32 & 70.27±0.13 & 66.88±0.85 \\ \hline
\textit{C2} & \textit{C11} & 75.56±0.02 & 75.58±0.02 & 75.42±0.02 & 75.42±0.02 & 68.44±0.06 & 67.09±0.13 & 68.99±0.15 & 67.62±0.19 & 69.55±0.24 & 69.48±0.41 & 65.66±0.41 \\ \hline
\textit{C2} & \textit{C13} & 75.23±0.04 & 75.23±0.03 & 75.06±0.03 & 75.08±0.04 & 68.04±0.07 & 66.75±0.13 & 68.57±0.21 & 67.21±0.12 & 68.81±0.23 & 68.88±0.42 & 64.51±1.74 \\ \hline
\textit{C3} & \textit{C7} & 76.93±0.02 & 76.95±0.02 & 76.7±0.01 & 76.7±0.02 & 70.85±0.1 & 69.65±0.06 & 71.31±0.12 & 70.22±0.14 & 72.4±0.19 & 72.7±0.11 & 71.4±1.05 \\ \hline
\textit{C3} & \textit{C10} & 75.88±0.04 & 75.87±0.04 & 75.64±0.04 & 75.62±0.02 & 70.01±0.11 & 69.02±0.12 & 70.49±0.05 & 69.47±0.14 & 72.43±0.09 & 72.36±0.11 & 70.04±0.39 \\ \hline
\textit{C3} & \textit{C11} & 77.09±0.02 & 77.08±0.05 & 76.8±0.04 & 76.79±0.06 & 70.88±0.05 & 69.74±0.06 & 71.39±0.06 & 70.18±0.17 & 72.61±0.23 & 72.68±0.16 & 71.56±0.27 \\ \hline
\textit{C3} & \textit{C13} & 76.95±0.04 & 76.92±0.03 & 76.68±0.03 & 76.61±0.03 & 70.57±0.06 & 69.47±0.09 & 71.05±0.03 & 69.85±0.09 & 72.23±0.3 & 72.43±0.35 & 71.74±0.88 \\ \hline
\textit{C4} & \textit{C7} & 76.98±0.02 & 76.99±0.03 & 76.73±0.04 & 76.73±0.02 & 71.11±0.06 & 70.02±0.08 & 71.57±0.16 & 70.53±0.18 & 72.71±0.13 & 72.8±0.16 & 71.23±0.6 \\ \hline
\textit{C4} & \textit{C10} & 76.31±0.03 & 76.31±0.03 & 76.06±0.03 & 76.06±0.05 & 70.59±0.08 & 69.6±0.09 & 71.06±0.06 & 69.99±0.08 & 72.72±0.1 & 72.63±0.06 & 69.94±0.4 \\ \hline
\textit{C4} & \textit{C11} & 76.77±0.02 & 76.76±0.02 & 76.49±0.05 & 76.47±0.02 & 70.69±0.09 & 69.63±0.09 & 71.3±0.09 & 70.04±0.13 & 72.57±0.28 & 72.58±0.19 & 71.34±0.51 \\ \hline
\textit{C4} & \textit{C13} & 76.6±0.02 & 76.59±0.01 & 76.32±0.02 & 76.3±0.02 & 70.44±0.11 & 69.26±0.09 & 70.89±0.09 & 69.85±0.07 & 72.32±0.07 & 72.22±0.15 & 71.35±0.91 \\ \hline
\textit{C4} & \textit{C15} & 75.51±0.02 & 75.47±0.03 & 74.9±0.07 & 74.85±0.06 & 68.66±0.05 & 67.69±0.09 & 69.07±0.12 & 68.06±0.23 & 71.13±0.3 & 71.41±0.23 & 66.68±0.61 \\ \hline
\textit{C6} & \textit{C7} & 73.56±0.04 & 73.61±0.04 & 73.41±0.04 & 73.4±0.04 & 64.8±0.05 & 62.87±0.25 & 65.57±0.13 & 63.81±0.12 & 68.23±0.33 & 68.26±0.48 & 62.62±1.64 \\ \hline
\textit{C6} & \textit{C10} & 72.89±0.04 & 72.9±0.05 & 72.79±0.04 & 72.81±0.05 & 65.01±0.08 & 62.88±0.31 & 65.49±0.16 & 63.84±0.44 & 69.84±0.24 & 69.75±0.22 & 63.3±1.28 \\ \hline
\textit{C7} & \textit{C8} & 74.55±0.02 & 74.58±0.03 & 74.41±0.02 & 74.41±0.04 & 65.17±0.16 & 63.35±0.24 & 66.12±0.17 & 64.27±0.13 & 68.87±0.3 & 68.96±0.37 & 64.87±0.58 \\ \hline
\textit{C7} & \textit{C10} & 73.49±0.03 & 73.5±0.02 & 73.35±0.03 & 73.31±0.03 & 64.32±0.16 & 62.66±0.17 & 65.23±0.27 & 63.2±0.19 & 69.11±0.34 & 68.77±0.28 & 62.31±2.02 \\ \hline
\textit{C7} & \textit{C12} & 76.87±0.04 & 76.88±0.03 & 76.62±0.06 & 76.64±0.03 & 70.74±0.09 & 69.6±0.21 & 71.37±0.1 & 70.02±0.12 & 72.48±0.11 & 72.74±0.15 & 70.85±0.42 \\ \hline
\textit{C7} & \textit{C14} & 74.66±0.05 & 74.68±0.05 & 74.46±0.05 & 74.48±0.06 & 66.92±0.14 & 65.18±0.11 & 67.52±0.12 & 65.84±0.12 & 68.9±0.56 & 68.74±0.51 & 65.31±0.99 \\ \hline
\textit{C7} & \textit{C15} & 76.89±0.03 & 76.89±0.03 & 76.67±0.02 & 76.64±0.04 & 71.0±0.04 & 69.89±0.07 & 71.65±0.11 & 70.35±0.09 & 72.5±0.06 & 72.51±0.21 & 70.6±0.29 \\ \hline
\textit{C7} & \textit{C16} & 76.89±0.03 & 76.91±0.03 & 76.66±0.03 & 76.66±0.05 & 70.98±0.05 & 69.83±0.13 & 71.41±0.08 & 70.31±0.22 & 72.61±0.11 & 72.72±0.14 & 70.95±0.18 \\ \hline
\textit{C7} & \textit{C18} & 76.56±0.03 & 76.55±0.03 & 76.34±0.05 & 76.31±0.04 & 70.4±0.1 & 69.31±0.07 & 70.85±0.05 & 69.75±0.15 & 71.87±0.16 & 71.86±0.07 & 70.06±0.44 \\ \hline
\textit{C7} & \textit{C20} & 74.43±0.06 & 74.46±0.06 & 74.28±0.05 & 74.28±0.08 & 64.65±0.12 & 63.09±0.2 & 65.21±0.2 & 63.64±0.1 & 67.98±0.82 & 67.79±0.24 & 63.06±0.89 \\ \hline
\textit{C7} & \textit{C21} & 76.89±0.04 & 76.91±0.03 & 76.64±0.04 & 76.67±0.06 & 70.87±0.08 & 69.76±0.18 & 71.48±0.05 & 70.38±0.13 & 72.5±0.11 & 72.84±0.16 & 71.49±1.01 \\ \hline
\textit{C7} & \textit{C24} & 76.38±0.04 & 76.35±0.03 & 76.11±0.03 & 76.04±0.06 & 70.39±0.05 & 69.28±0.17 & 70.74±0.12 & 69.78±0.09 & 72.3±0.16 & 72.18±0.06 & 70.9±0.87 \\ \hline
\textit{C7} & \textit{C26} & 75.45±0.02 & 75.42±0.04 & 75.14±0.03 & 75.11±0.04 & 69.64±0.07 & 68.4±0.11 & 70.0±0.04 & 68.97±0.12 & 71.23±0.04 & 71.14±0.08 & 69.27±0.4 \\ \hline
\textit{C10} & \textit{C12} & 75.91±0.04 & 75.9±0.04 & 75.67±0.04 & 75.66±0.04 & 70.04±0.07 & 69.1±0.1 & 70.44±0.08 & 69.4±0.11 & 72.43±0.32 & 72.31±0.17 & 70.52±0.22 \\ \hline
\textit{C10} & \textit{C14} & 73.59±0.04 & 73.6±0.04 & 73.53±0.04 & 73.48±0.05 & 66.77±0.1 & 65.36±0.18 & 67.27±0.09 & 65.86±0.26 & 69.69±0.29 & 69.64±0.19 & 65.08±0.73 \\ \hline
\textit{C10} & \textit{C15} & 75.76±0.04 & 75.75±0.04 & 75.58±0.05 & 75.56±0.04 & 70.07±0.05 & 68.83±0.11 & 70.63±0.08 & 69.51±0.17 & 71.88±0.11 & 71.93±0.02 & 69.52±0.19 \\ \hline
\textit{C10} & \textit{C16} & 76.03±0.02 & 76.03±0.03 & 75.76±0.03 & 75.77±0.04 & 70.2±0.09 & 69.25±0.06 & 70.79±0.06 & 69.66±0.1 & 72.48±0.13 & 72.44±0.11 & 70.24±0.56 \\ \hline
\textit{C10} & \textit{C17} & 73.18±0.04 & 73.18±0.04 & 73.12±0.04 & 73.06±0.02 & 63.66±0.13 & 62.33±0.21 & 64.55±0.14 & 62.78±0.18 & 68.94±0.19 & 69.23±0.3 & 62.02±1.2 \\ \hline
\textit{C10} & \textit{C18} & 75.29±0.03 & 75.28±0.03 & 75.12±0.03 & 75.09±0.05 & 69.24±0.1 & 68.29±0.09 & 69.8±0.07 & 68.66±0.09 & 71.26±0.19 & 71.21±0.14 & 68.77±0.45 \\ \hline
\textit{C10} & \textit{C20} & 73.41±0.04 & 73.4±0.04 & 73.36±0.04 & 73.29±0.05 & 65.07±0.19 & 63.46±0.22 & 65.75±0.18 & 64.13±0.24 & 69.35±0.52 & 69.53±0.29 & 62.98±0.61 \\ \hline
\textit{C10} & \textit{C21} & 76.02±0.03 & 76.01±0.04 & 75.77±0.05 & 75.76±0.04 & 70.11±0.09 & 69.23±0.09 & 70.7±0.09 & 69.62±0.2 & 72.38±0.08 & 72.46±0.09 & 70.54±0.67 \\ \hline
\textit{C10} & \textit{C24} & 75.4±0.03 & 75.37±0.01 & 75.18±0.02 & 75.11±0.04 & 69.72±0.04 & 68.83±0.08 & 70.12±0.09 & 69.24±0.1 & 72.35±0.1 & 71.95±0.14 & 69.32±0.51 \\ \hline
\textit{C10} & \textit{C26} & 74.73±0.03 & 74.72±0.03 & 74.48±0.06 & 74.46±0.05 & 69.05±0.11 & 67.94±0.08 & 69.43±0.06 & 68.44±0.15 & 71.03±0.26 & 70.78±0.25 & 68.03±0.97 \\ \hline
\textit{C11} & \textit{C12} & 76.98±0.05 & 76.98±0.03 & 76.71±0.04 & 76.72±0.03 & 70.72±0.09 & 69.57±0.1 & 71.37±0.14 & 69.96±0.15 & 72.59±0.13 & 72.65±0.13 & 71.47±0.18 \\ \hline
\textit{C11} & \textit{C15} & 76.85±0.02 & 76.83±0.01 & 76.61±0.01 & 76.66±0.04 & 70.76±0.08 & 69.68±0.08 & 71.37±0.1 & 70.1±0.09 & 72.39±0.11 & 72.32±0.16 & 71.1±0.42 \\ \hline
\textit{C11} & \textit{C16} & 76.87±0.03 & 76.86±0.04 & 76.6±0.02 & 76.59±0.03 & 70.81±0.08 & 69.65±0.06 & 71.39±0.03 & 70.08±0.06 & 72.69±0.3 & 72.51±0.11 & 71.53±0.58 \\ \hline
\textit{C11} & \textit{C18} & 76.54±0.05 & 76.55±0.06 & 76.33±0.05 & 76.33±0.04 & 70.24±0.09 & 69.05±0.11 & 70.68±0.11 & 69.46±0.09 & 71.69±0.17 & 71.78±0.14 & 70.3±0.78 \\ \hline
\textit{C11} & \textit{C21} & 77.0±0.02 & 76.99±0.01 & 76.73±0.02 & 76.72±0.02 & 70.92±0.09 & 69.73±0.11 & 71.48±0.1 & 70.28±0.16 & 72.71±0.17 & 72.78±0.18 & 72.04±1.24 \\ \hline
\textit{C11} & \textit{C24} & 76.31±0.03 & 76.27±0.03 & 76.01±0.04 & 75.93±0.04 & 70.15±0.07 & 69.09±0.08 & 70.57±0.07 & 69.46±0.09 & 72.07±0.14 & 72.15±0.19 & 70.98±0.44 \\ \hline
\textit{C11} & \textit{C26} & 75.89±0.03 & 75.86±0.04 & 75.6±0.05 & 75.58±0.04 & 69.85±0.07 & 68.67±0.29 & 70.37±0.11 & 69.25±0.09 & 71.24±0.16 & 71.42±0.1 & 69.18±0.39 \\ \hline
\textit{C12} & \textit{C13} & 76.83±0.04 & 76.82±0.05 & 76.55±0.05 & 76.54±0.04 & 70.4±0.05 & 69.41±0.06 & 71.0±0.08 & 69.71±0.1 & 72.01±0.16 & 72.38±0.07 & 71.26±0.42 \\ \hline
\textit{C13} & \textit{C15} & 76.82±0.02 & 76.8±0.02 & 76.61±0.03 & 76.57±0.04 & 70.58±0.06 & 69.44±0.15 & 71.03±0.12 & 69.91±0.1 & 71.99±0.11 & 72.04±0.2 & 70.7±0.3 \\ \hline
\textit{C13} & \textit{C16} & 76.71±0.02 & 76.71±0.02 & 76.44±0.05 & 76.42±0.02 & 70.51±0.07 & 69.42±0.09 & 71.06±0.14 & 69.86±0.15 & 72.36±0.21 & 72.24±0.12 & 72.07±0.53 \\ \hline
\textit{C13} & \textit{C18} & 76.33±0.03 & 76.32±0.04 & 76.11±0.02 & 76.11±0.04 & 69.99±0.1 & 68.8±0.11 & 70.41±0.07 & 69.17±0.1 & 71.18±0.13 & 71.38±0.19 & 68.88±0.66 \\ \hline
\textit{C13} & \textit{C21} & 76.83±0.02 & 76.83±0.02 & 76.57±0.02 & 76.56±0.02 & 70.57±0.03 & 69.47±0.09 & 71.06±0.15 & 69.82±0.07 & 72.32±0.12 & 72.46±0.14 & 71.5±0.23 \\ \hline
\textit{C13} & \textit{C24} & 76.13±0.03 & 76.09±0.02 & 75.81±0.02 & 75.8±0.02 & 69.89±0.02 & 68.91±0.07 & 70.2±0.06 & 69.29±0.12 & 71.94±0.11 & 71.77±0.13 & 70.35±0.41 \\ \hline
\textit{C13} & \textit{C26} & 75.96±0.02 & 75.92±0.03 & 75.68±0.05 & 75.59±0.04 & 69.85±0.07 & 68.47±0.15 & 70.29±0.05 & 69.13±0.19 & 71.53±0.14 & 71.34±0.19 & 69.16±0.61 \\ \hline
\end{longtable}
\end{centering}
\end{small}

==> table_6.tex <==
\begin{table}[]
\centering
\caption{AUC scores obtained by instance level training on Criteo}
\label{tab:instance_level_auc}
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Experiment} & \textbf{Model} & \textbf{Optimizer} & \textbf{Loss Function} & \textbf{AUC Score} \\ \hline
\textit{E1} & 1-Layer MLP & Adam & BCE & 79.23 \\ \hline
\textit{E2} & 1-Layer MLP & Adam & MSE & 79.2 \\ \hline
\textit{E3} & 2-Layer MLP & Adam & BCE & 80.1 \\ \hline
\textit{E4} & 2-Layer MLP & Adam & MSE & 79.94 \\ \hline
\textit{E5} & 1-Layer MLP & SGD & BCE & 80.7 \\ \hline
\textit{E6} & 1-Layer MLP & SGD & MSE & 80.54 \\ \hline
\textit{E7} & 2-Layer MLP & SGD & BCE & 79.17 \\ \hline
\textit{E8} & 2-Layer MLP & SGD & MSE & 80.56 \\ \hline
\textit{E9} & AutoInt & Adam & BCE & 80.66 \\ \hline
\textit{E10} & AutoInt & Adam & MSE & 80.7 \\ \hline
\textit{E11} & AutoInt & Adam & MSE & 79.02 \\ \hline
\end{tabular}
}
\end{table}

==> table_auc_llp_bench_autoint.tex <==
\begin{table}[]
\scriptsize
\centering
\caption{\small AUC Scores of AutoInt obtained on LLP-Bench Groupings}
\label{tab:auc_llp_bench_autoint}
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Col1} & \textbf{Col2} & \textbf{E9} & \textbf{E10} & \textbf{E11} \\ \hline
\textit{C1} & \textit{C10} & 70.4±0.17 & 70.23±0.18 & 61.98±0.38 \\ \hline
\textit{C6} & \textit{C10} & 69.84±0.24 & 69.75±0.22 & 63.3±1.28 \\ \hline
\textit{C2} & \textit{C13} & 68.81±0.23 & 68.88±0.42 & 64.51±1.74 \\ \hline
\textit{C7} & \textit{C10} & 69.11±0.34 & 68.77±0.28 & 62.31±2.02 \\ \hline
\textit{C10} & \textit{C15} & 71.88±0.11 & 71.93±0.02 & 69.52±0.19 \\ \hline
\textit{C7} & \textit{C21} & 72.5±0.11 & 72.84±0.16 & 71.49±1.01 \\ \hline
\textit{C7} & \textit{C10} & 69.11±0.34 & 68.77±0.28 & 62.31±2.02 \\ \hline
\textit{C7} & \textit{C20} & 67.98±0.82 & 67.79±0.24 & 63.06±0.89 \\ \hline
\end{tabular}
\end{table}


==> table_auc_llp_bench_mlp.tex <==
\begin{table*}[]
\normalsize
\centering
\caption{\small AUC Scores obtained on LLP-Bench Groupings}
\label{tab:auc_llp_bench_mlp}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{Col1} & \textbf{Col2} & \textbf{E1} & \textbf{E2} & \textbf{E3} & \textbf{E4} & \textbf{E5} & \textbf{E6} \\ \hline
\textit{C1} & \textit{C10} & 73.64±0.05 & 73.67±0.05 & 73.6±0.06 & 73.61±0.04 & 70.4±0.17 & 70.23±0.18 \\ \hline
\textit{C6} & \textit{C10} & 72.89±0.04 & 72.9±0.05 & 72.79±0.04 & 72.81±0.05 & 69.84±0.24 & 69.75±0.22 \\ \hline
\textit{C2} & \textit{C13} & 75.23±0.04 & 75.23±0.03 & 75.06±0.03 & 75.08±0.04 & 68.81±0.23 & 68.88±0.42 \\ \hline
\textit{C7} & \textit{C10} & 73.49±0.03 & 73.5±0.02 & 73.35±0.03 & 73.31±0.03 & 69.11±0.34 & 68.77±0.28 \\ \hline
\textit{C10} & \textit{C15} & 75.76±0.04 & 75.75±0.04 & 75.58±0.05 & 75.56±0.04 & 71.88±0.11 & 71.93±0.02 \\ \hline
\textit{C7} & \textit{C21} & 76.89±0.04 & 76.91±0.03 & 76.64±0.04 & 76.67±0.06 & 72.5±0.11 & 72.84±0.16 \\ \hline
\textit{C7} & \textit{C20} & 74.43±0.06 & 74.46±0.06 & 74.28±0.05 & 74.28±0.08 & 67.98±0.82 & 67.79±0.24 \\ \hline
\end{tabular}
\end{table*}

==> table_avg_ll_ranges.tex <==
\begin{table}
\caption{\small Clustering on $\tn{AvgBagLL}$.}
\normalsize
\centering
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{\begin{tabular}[c]{@{}l@{}} Cluster\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}\# Groupings\end{tabular}} & \textbf{Min LL} & \textbf{Max LL} \\ \hline
\textit{High} & 26 & -9.48 & -3.26 \\ \hline
\textit{Medium} & 73 & -15.98 & -9.8 \\ \hline
\textit{Low} & 173 & -24.19 & -16.02 \\ \hline
\textit{Very Low} & 36 & -38.88 & -25.47 \\ \hline
\end{tabular}
\label{tab:avg_ll_ranges}
\end{table}

==> table_corr.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{Opt} & \textbf{Model}                                        & \textbf{Loss} & \textbf{\begin{tabular}[c]{@{}l@{}}MoM\\ Inter-\\ Bag\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Mean\\ Intra-\\ Bag\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Inter/\\ Intra\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}No. \\ Bags\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}No. \\ Inst\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Mean\\ BagSize\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Bag \\ Size \\ 50 \\ Percentile\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Bag\\ Size\\ 95 \\ Percentile\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Avg \\ Label\\ LL\end{tabular}} \\ \hline
SGD          & \begin{tabular}[c]{@{}l@{}}1-layer\\ MLP\end{tabular} & bce           & 0.375                                                               & -0.552                                                               & 0.647                                                           & 0.784                                                        & 0.506                                                        & -0.699                                                          & -0.619                                                                           & -0.747                                                                         & -0.467                                                             \\ \hline
SGD          & \begin{tabular}[c]{@{}l@{}}1-layer\\ MLP\end{tabular} & mse           & 0.459                                                               & -0.542                                                               & 0.664                                                           & 0.657                                                        & 0.362                                                        & -0.636                                                          & -0.566                                                                           & -0.677                                                                         & -0.452                                                             \\ \hline
SGD          & \begin{tabular}[c]{@{}l@{}}2-layer\\ MLP\end{tabular} & bce           & 0.353                                                               & -0.532                                                               & 0.623                                                           & 0.818                                                        & 0.542                                                        & -0.725                                                          & -0.645                                                                           & -0.773                                                                         & -0.429                                                             \\ \hline
SGD          & \begin{tabular}[c]{@{}l@{}}2-layer\\ MLP\end{tabular} & mse           & 0.427                                                               & -0.557                                                               & 0.67                                                            & 0.707                                                        & 0.408                                                        & -0.661                                                          & -0.583                                                                           & -0.708                                                                         & -0.456                                                             \\ \hline
Adam         & \begin{tabular}[c]{@{}l@{}}1-layer\\ MLP\end{tabular} & bce           & 0.179                                                               & -0.45                                                                & 0.475                                                           & 0.712                                                        & 0.459                                                        & -0.672                                                          & -0.605                                                                           & -0.713                                                                         & -0.6                                                               \\ \hline
Adam         & \begin{tabular}[c]{@{}l@{}}1-layer\\ MLP\end{tabular} & bce           & 0.235                                                               & -0.388                                                               & 0.43                                                            & 0.627                                                        & 0.329                                                        & -0.65                                                           & -0.581                                                                           & -0.693                                                                         & -0.608                                                             \\ \hline
Adam         & \begin{tabular}[c]{@{}l@{}}1-layer\\ MLP\end{tabular} & mse           & 0.173                                                               & -0.461                                                               & 0.484                                                           & 0.712                                                        & 0.464                                                        & -0.667                                                          & -0.6                                                                             & -0.707                                                                         & -0.601                                                             \\ \hline
Adam         & \begin{tabular}[c]{@{}l@{}}1-layer\\ MLP\end{tabular} & mse           & 0.226                                                               & -0.415                                                               & 0.453                                                           & 0.628                                                        & 0.343                                                        & -0.638                                                          & -0.569                                                                           & -0.68                                                                          & -0.618                                                             \\ \hline
Adam         & \begin{tabular}[c]{@{}l@{}}2-layer\\ MLP\end{tabular} & bce           & 0.162                                                               & -0.455                                                               & 0.475                                                           & 0.717                                                        & 0.471                                                        & -0.666                                                          & -0.598                                                                           & -0.708                                                                         & -0.587                                                             \\ \hline
Adam         & \begin{tabular}[c]{@{}l@{}}2-layer\\ MLP\end{tabular} & bce           & 0.322                                                               & -0.324                                                               & 0.398                                                           & 0.66                                                         & 0.302                                                        & -0.724                                                          & -0.648                                                                           & -0.769                                                                         & -0.491                                                             \\ \hline
Adam         & \begin{tabular}[c]{@{}l@{}}2-layer\\ MLP\end{tabular} & mse           & 0.149                                                               & -0.466                                                               & 0.483                                                           & 0.722                                                        & 0.486                                                        & -0.661                                                          & -0.593                                                                           & -0.703                                                                         & -0.588                                                             \\ \hline
Adam         & \begin{tabular}[c]{@{}l@{}}2-layer\\ MLP\end{tabular} & mse           & 0.323                                                               & -0.346                                                               & 0.419                                                           & 0.651                                                        & 0.3                                                          & -0.705                                                          & -0.626                                                                           & -0.753                                                                         & -0.503                                                             \\ \hline
\end{tabular}
\caption{Correlation scores of metrics with AUC scores obtained in these experiments.}
\label{tab:my-table}
\end{table}

==> table_expt_legend.tex <==
\begin{table}
\normalsize
\centering
\caption{\small Experiment Legend}
\label{tab:expt_legend}
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Expt.} & \textbf{Model} & \textbf{Opt.} & \textbf{Loss} \\ \hline
\textit{E1} & 1-Layer MLP & Adam & BCE \\ \hline
\textit{E2} & 1-Layer MLP & Adam & MSE \\ \hline
\textit{E3} & 2-Layer MLP & Adam & BCE \\ \hline
\textit{E4} & 2-Layer MLP & Adam & MSE \\ \hline
\textit{E5} & AutoInt & Adam & BCE \\ \hline
\textit{E6} & AutoInt & Adam & MSE \\ \hline
\end{tabular}
\end{table}

==> table_expt_legend_1.tex <==
\begin{table}
\normalsize
\centering
\caption{\small Experiment Legend}
\label{tab:expt_legend1}
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Expt.} & \textbf{Model} & \textbf{Opt.} & \textbf{Loss} \\ \hline
\textit{Expt1} & 1-Layer MLP & Adam & BCE \\ \hline
\textit{Expt2} & 1-Layer MLP & Adam & MSE \\ \hline
\textit{Expt3} & 2-Layer MLP & Adam & BCE \\ \hline
\textit{Expt4} & 2-Layer MLP & Adam & MSE \\ \hline
\textit{Expt5} & 1-Layer MLP & SGD & BCE \\ \hline
\textit{Expt6} & 1-Layer MLP & SGD & MSE \\ \hline
\textit{Expt7} & 2-Layer MLP & SGD & BCE \\ \hline
\textit{Expt8} & 2-Layer MLP & SGD & MSE \\ \hline
\textit{Expt9} & AutoInt & Adam & BCE \\ \hline
\textit{Expt10} & AutoInt & Adam & MSE \\ \hline
\textit{Expt11} & AutoInt & SGD & BCE \\ \hline
\end{tabular}
\end{table}

==> table_feature_random_MLP.tex <==
\begin{table}[]
\caption{Feature Random bags Training results using 2-Layer MLP}
\label{tab:feature_rand_mlp}
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textit{\textbf{Col1}} & \textit{\textbf{Col2}} & \textbf{BCE, 64} & \textbf{BCE, 128} & \textbf{BCE, 256} & \textbf{BCE, 512} & \textbf{MSE, 64} & \textbf{MSE, 128} & \textbf{MSE, 256} & \textbf{MSE, 512} & \textbf{MAE, 64} & \textbf{MAE, 128} & \textbf{MAE, 256} & \textbf{MAE, 512} \\ \hline
\textit{C1}            & \textit{C10}           & 77.11±0.01       & 76.3±0.02         & 75.25±0.02        & 74.1±0.03         & 77.06±0.03       & 76.3±0.02         & 75.28±0.02        & 74.14±0.04        & 76.87±0.03       & 76.12±0.03        & 75.16±0.02        & 74.14±0.06        \\ \hline
\textit{C2}            & \textit{C7}            & 76.89±0.01       & 76.31±0.01        & 75.84±0.02        & 75.44±0.02        & 76.89±0.01       & 76.34±0.03        & 75.85±0.01        & 75.48±0.01        & 76.87±0.0        & 76.38±0.02        & 75.96±0.03        & 75.62±0.01        \\ \hline
\textit{C2}            & \textit{C10}           & 76.85±0.03       & 76.11±0.01        & 75.42±0.03        & 74.84±0.03        & 76.81±0.03       & 76.07±0.02        & 75.4±0.03         & 74.83±0.03        & 76.75±0.03       & 76.09±0.02        & 75.49±0.04        & 74.94±0.04        \\ \hline
\textit{C2}            & \textit{C11}           & 76.76±0.02       & 76.16±0.01        & 75.68±0.03        & 75.31±0.02        & 76.76±0.03       & 76.19±0.01        & 75.7±0.02         & 75.34±0.03        & 76.76±0.04       & 76.22±0.02        & 75.79±0.02        & 75.44±0.02        \\ \hline
\textit{C2}            & \textit{C13}           & 76.74±0.03       & 76.11±0.02        & 75.58±0.01        & 75.18±0.02        & 76.74±0.02       & 76.12±0.02        & 75.59±0.02        & 75.19±0.01        & 76.7±0.02        & 76.13±0.03        & 75.64±0.03        & 75.25±0.02        \\ \hline
\textit{C3}            & \textit{C7}            & 77.34±0.03       & 76.83±0.03        & 76.36±0.01        & 75.9±0.01         & 77.31±0.02       & 76.8±0.02         & 76.35±0.01        & 75.9±0.01         & 77.33±0.04       & 76.9±0.02         & 76.47±0.02        & 76.04±0.01        \\ \hline
\textit{C3}            & \textit{C10}           & 77.17±0.02       & 76.5±0.02         & 75.88±0.03        & 75.37±0.04        & 77.12±0.03       & 76.45±0.02        & 75.83±0.04        & 75.35±0.05        & 77.25±0.02       & 76.71±0.02        & 76.21±0.04        & 75.75±0.02        \\ \hline
\textit{C3}            & \textit{C11}           & 77.32±0.02       & 76.78±0.02        & 76.28±0.01        & 75.82±0.02        & 77.32±0.02       & 76.79±0.02        & 76.3±0.01         & 75.84±0.02        & 77.34±0.02       & 76.88±0.01        & 76.42±0.01        & 75.99±0.02        \\ \hline
\textit{C3}            & \textit{C13}           & 77.37±0.02       & 76.84±0.02        & 76.32±0.02        & 75.84±0.02        & 77.36±0.02       & 76.84±0.02        & 76.34±0.03        & 75.89±0.02        & 77.37±0.03       & 76.9±0.03         & 76.43±0.03        & 76.0±0.01         \\ \hline
\textit{C4}            & \textit{C7}            & 77.37±0.02       & 76.89±0.02        & 76.46±0.01        & 76.08±0.03        & 77.34±0.02       & 76.88±0.02        & 76.47±0.02        & 76.1±0.01         & 77.4±0.02        & 77.0±0.02         & 76.6±0.02         & 76.24±0.02        \\ \hline
\textit{C4}            & \textit{C10}           & 77.25±0.02       & 76.66±0.01        & 76.11±0.02        & 75.6±0.03         & 77.18±0.02       & 76.59±0.01        & 76.03±0.02        & 75.57±0.02        & 77.28±0.02       & 76.82±0.01        & 76.37±0.01        & 75.98±0.01        \\ \hline
\textit{C4}            & \textit{C11}           & 77.32±0.02       & 76.85±0.02        & 76.43±0.01        & 76.08±0.03        & 77.3±0.02        & 76.83±0.02        & 76.41±0.02        & 76.06±0.01        & 77.36±0.02       & 76.94±0.02        & 76.55±0.03        & 76.21±0.02        \\ \hline
\textit{C4}            & \textit{C13}           & 77.31±0.02       & 76.85±0.02        & 76.43±0.02        & 76.09±0.02        & 77.28±0.03       & 76.81±0.03        & 76.4±0.02         & 76.07±0.02        & 77.34±0.03       & 76.92±0.03        & 76.51±0.02        & 76.15±0.03        \\ \hline
\textit{C4}            & \textit{C15}           & 75.75±0.02       & 74.93±0.04        & 74.38±0.04        & 74.03±0.04        & 75.65±0.02       & 74.81±0.03        & 74.25±0.04        & 73.91±0.03        & 76.35±0.03       & 75.74±0.03        & 75.29±0.03        & 74.95±0.03        \\ \hline
\textit{C6}            & \textit{C7}            & 76.47±0.03       & 75.53±0.01        & 74.66±0.02        & 73.97±0.05        & 76.53±0.02       & 75.61±0.01        & 74.74±0.03        & 74.06±0.02        & 76.51±0.03       & 75.76±0.03        & 75.05±0.03        & 74.45±0.04        \\ \hline
\textit{C6}            & \textit{C10}           & 76.82±0.04       & 75.94±0.03        & 74.95±0.02        & 73.98±0.01        & 76.8±0.03        & 75.94±0.03        & 74.96±0.02        & 73.99±0.02        & 76.67±0.02       & 75.89±0.02        & 75.01±0.03        & 74.12±0.01        \\ \hline
\textit{C7}            & \textit{C8}            & 77.01±0.03       & 76.15±0.02        & 75.12±0.03        & 74.09±0.02        & 77.03±0.03       & 76.23±0.02        & 75.25±0.04        & 74.25±0.01        & 76.84±0.03       & 76.12±0.03        & 75.31±0.03        & 74.52±0.03        \\ \hline
\textit{C7}            & \textit{C10}           & 76.41±0.03       & 75.43±0.03        & 74.51±0.03        & 73.78±0.02        & 76.42±0.02       & 75.45±0.03        & 74.51±0.02        & 73.78±0.03        & 76.38±0.03       & 75.54±0.03        & 74.8±0.02         & 74.14±0.01        \\ \hline
\textit{C7}            & \textit{C12}           & 77.34±0.01       & 76.82±0.02        & 76.33±0.01        & 75.88±0.01        & 77.31±0.02       & 76.82±0.02        & 76.33±0.01        & 75.91±0.01        & 77.35±0.03       & 76.92±0.02        & 76.5±0.01         & 76.09±0.02        \\ \hline
\textit{C7}            & \textit{C14}           & 76.61±0.02       & 75.78±0.02        & 75.03±0.02        & 74.45±0.03        & 76.64±0.01       & 75.83±0.01        & 75.11±0.03        & 74.54±0.02        & 76.6±0.01        & 75.87±0.02        & 75.28±0.03        & 74.78±0.05        \\ \hline
\textit{C7}            & \textit{C15}           & 77.11±0.01       & 76.65±0.02        & 76.27±0.02        & 76.01±0.04        & 77.11±0.02       & 76.68±0.01        & 76.31±0.01        & 76.04±0.03        & 77.18±0.03       & 76.8±0.03         & 76.48±0.02        & 76.19±0.03        \\ \hline
\textit{C7}            & \textit{C16}           & 77.35±0.03       & 76.85±0.03        & 76.39±0.02        & 75.96±0.01        & 77.32±0.03       & 76.84±0.02        & 76.4±0.02         & 75.98±0.02        & 77.37±0.02       & 76.94±0.03        & 76.52±0.01        & 76.13±0.02        \\ \hline
\textit{C7}            & \textit{C18}           & 76.97±0.01       & 76.48±0.01        & 76.14±0.02        & 75.86±0.01        & 76.98±0.02       & 76.5±0.03         & 76.17±0.03        & 75.9±0.02         & 77.04±0.02       & 76.63±0.01        & 76.33±0.02        & 76.01±0.03        \\ \hline
\textit{C7}            & \textit{C20}           & 76.79±0.03       & 76.09±0.04        & 75.44±0.03        & 74.96±0.03        & 76.79±0.03       & 76.1±0.04         & 75.47±0.04        & 74.99±0.04        & 76.73±0.03       & 76.14±0.03        & 75.59±0.03        & 75.19±0.04        \\ \hline
\textit{C7}            & \textit{C21}           & 77.33±0.02       & 76.82±0.02        & 76.36±0.03        & 75.96±0.02        & 77.32±0.02       & 76.83±0.02        & 76.38±0.04        & 75.97±0.03        & 77.36±0.02       & 76.95±0.03        & 76.54±0.02        & 76.15±0.01        \\ \hline
\textit{C7}            & \textit{C24}           & 77.18±0.01       & 76.69±0.02        & 76.26±0.03        & 75.9±0.03         & 77.18±0.02       & 76.7±0.03         & 76.28±0.03        & 75.92±0.03        & 77.23±0.01       & 76.81±0.02        & 76.43±0.02        & 76.07±0.02        \\ \hline
\textit{C7}            & \textit{C26}           & 77.13±0.02       & 76.54±0.01        & 75.97±0.02        & 75.48±0.02        & 77.11±0.02       & 76.53±0.01        & 75.95±0.02        & 75.46±0.01        & 77.15±0.02       & 76.67±0.01        & 76.21±0.02        & 75.81±0.02        \\ \hline
\textit{C10}           & \textit{C12}           & 77.18±0.03       & 76.53±0.03        & 75.94±0.02        & 75.44±0.02        & 77.11±0.04       & 76.46±0.03        & 75.87±0.04        & 75.38±0.02        & 77.24±0.03       & 76.74±0.02        & 76.27±0.02        & 75.83±0.04        \\ \hline
\textit{C10}           & \textit{C14}           & 76.74±0.02       & 75.83±0.02        & 74.84±0.02        & 73.96±0.03        & 76.71±0.02       & 75.82±0.02        & 74.86±0.02        & 73.98±0.03        & 76.61±0.03       & 75.81±0.03        & 74.95±0.04        & 74.19±0.02        \\ \hline
\textit{C10}           & \textit{C15}           & 76.93±0.03       & 76.36±0.02        & 75.94±0.03        & 75.59±0.02        & 76.85±0.03       & 76.3±0.02         & 75.88±0.03        & 75.58±0.03        & 76.94±0.02       & 76.51±0.03        & 76.16±0.02        & 75.83±0.04        \\ \hline
\textit{C10}           & \textit{C16}           & 77.19±0.03       & 76.56±0.03        & 75.96±0.02        & 75.44±0.03        & 77.13±0.03       & 76.5±0.03         & 75.9±0.03         & 75.39±0.04        & 77.26±0.03       & 76.74±0.03        & 76.24±0.02        & 75.8±0.04         \\ \hline
\textit{C10}           & \textit{C17}           & 76.84±0.02       & 75.94±0.02        & 74.89±0.03        & 73.73±0.03        & 76.82±0.02       & 75.9±0.02         & 74.85±0.01        & 73.74±0.03        & 76.69±0.02       & 75.85±0.02        & 74.95±0.04        & 73.98±0.04        \\ \hline
\textit{C10}           & \textit{C18}           & 76.76±0.01       & 76.09±0.02        & 75.57±0.02        & 75.08±0.03        & 76.71±0.02       & 76.06±0.01        & 75.54±0.02        & 75.07±0.03        & 76.8±0.02        & 76.26±0.03        & 75.8±0.03         & 75.4±0.03         \\ \hline
\textit{C10}           & \textit{C20}           & 76.92±0.03       & 76.12±0.03        & 75.24±0.03        & 74.44±0.01        & 76.87±0.03       & 76.07±0.02        & 75.22±0.04        & 74.41±0.04        & 76.79±0.02       & 76.07±0.03        & 75.33±0.03        & 74.65±0.02        \\ \hline
\textit{C10}           & \textit{C21}           & 77.15±0.03       & 76.52±0.03        & 75.94±0.04        & 75.42±0.03        & 77.09±0.03       & 76.44±0.03        & 75.86±0.04        & 75.34±0.03        & 77.21±0.03       & 76.71±0.04        & 76.23±0.03        & 75.76±0.04        \\ \hline
\textit{C10}           & \textit{C24}           & 76.92±0.02       & 76.2±0.02         & 75.63±0.03        & 75.13±0.02        & 76.81±0.03       & 76.11±0.03        & 75.52±0.04        & 75.06±0.01        & 77.05±0.02       & 76.52±0.04        & 76.08±0.03        & 75.69±0.04        \\ \hline
\textit{C10}           & \textit{C26}           & 77.14±0.02       & 76.48±0.02        & 75.78±0.02        & 75.14±0.02        & 77.1±0.02        & 76.46±0.01        & 75.78±0.02        & 75.16±0.03        & 77.13±0.02       & 76.6±0.02         & 76.06±0.02        & 75.56±0.03        \\ \hline
\textit{C11}           & \textit{C12}           & 77.33±0.03       & 76.82±0.04        & 76.33±0.02        & 75.89±0.03        & 77.32±0.03       & 76.81±0.03        & 76.34±0.02        & 75.91±0.02        & 77.38±0.03       & 76.94±0.04        & 76.52±0.03        & 76.09±0.01        \\ \hline
\textit{C11}           & \textit{C15}           & 77.1±0.01        & 76.62±0.05        & 76.26±0.02        & 76.02±0.04        & 77.08±0.02       & 76.62±0.01        & 76.29±0.03        & 76.03±0.03        & 77.13±0.02       & 76.77±0.02        & 76.46±0.03        & 76.22±0.04        \\ \hline
\textit{C11}           & \textit{C16}           & 77.28±0.01       & 76.76±0.03        & 76.33±0.01        & 75.94±0.01        & 77.26±0.02       & 76.75±0.03        & 76.31±0.0         & 75.92±0.01        & 77.32±0.03       & 76.87±0.03        & 76.47±0.02        & 76.12±0.01        \\ \hline
\textit{C11}           & \textit{C18}           & 76.96±0.02       & 76.47±0.02        & 76.09±0.03        & 75.76±0.01        & 76.95±0.02       & 76.49±0.02        & 76.11±0.03        & 75.8±0.01         & 76.98±0.02       & 76.56±0.03        & 76.17±0.02        & 75.88±0.02        \\ \hline
\textit{C11}           & \textit{C21}           & 77.31±0.02       & 76.78±0.02        & 76.31±0.02        & 75.91±0.02        & 77.31±0.02       & 76.79±0.02        & 76.33±0.01        & 75.92±0.02        & 77.33±0.03       & 76.88±0.02        & 76.45±0.01        & 76.09±0.03        \\ \hline
\textit{C11}           & \textit{C24}           & 77.13±0.02       & 76.62±0.03        & 76.2±0.01         & 75.87±0.02        & 77.11±0.01       & 76.61±0.02        & 76.19±0.02        & 75.86±0.02        & 77.19±0.02       & 76.75±0.02        & 76.37±0.02        & 76.04±0.03        \\ \hline
\textit{C11}           & \textit{C26}           & 77.1±0.02        & 76.49±0.03        & 75.95±0.02        & 75.52±0.02        & 77.1±0.02        & 76.5±0.02         & 75.97±0.02        & 75.53±0.02        & 77.12±0.02       & 76.62±0.02        & 76.19±0.02        & 75.77±0.01        \\ \hline
\textit{C12}           & \textit{C13}           & 77.37±0.02       & 76.86±0.02        & 76.39±0.02        & 75.95±0.02        & 77.36±0.02       & 76.87±0.02        & 76.42±0.01        & 76.0±0.01         & 77.36±0.03       & 76.92±0.02        & 76.5±0.02         & 76.08±0.02        \\ \hline
\textit{C13}           & \textit{C15}           & 77.02±0.02       & 76.58±0.03        & 76.21±0.02        & 75.98±0.01        & 76.98±0.01       & 76.54±0.03        & 76.21±0.01        & 75.97±0.02        & 77.07±0.02       & 76.69±0.01        & 76.39±0.01        & 76.12±0.02        \\ \hline
\textit{C13}           & \textit{C16}           & 77.31±0.03       & 76.8±0.02         & 76.35±0.01        & 75.98±0.02        & 77.3±0.03        & 76.8±0.02         & 76.37±0.03        & 75.99±0.02        & 77.33±0.03       & 76.88±0.02        & 76.45±0.03        & 76.09±0.02        \\ \hline
\textit{C13}           & \textit{C18}           & 76.93±0.02       & 76.42±0.02        & 76.03±0.04        & 75.74±0.04        & 76.9±0.02        & 76.42±0.02        & 76.04±0.03        & 75.75±0.03        & 76.95±0.03       & 76.53±0.02        & 76.17±0.03        & 75.86±0.01        \\ \hline
\textit{C13}           & \textit{C21}           & 77.27±0.02       & 76.75±0.02        & 76.29±0.01        & 75.88±0.01        & 77.25±0.02       & 76.75±0.02        & 76.3±0.01         & 75.9±0.01         & 77.31±0.02       & 76.86±0.01        & 76.43±0.01        & 76.04±0.03        \\ \hline
\textit{C13}           & \textit{C24}           & 77.13±0.02       & 76.61±0.02        & 76.18±0.02        & 75.85±0.02        & 77.1±0.02        & 76.58±0.02        & 76.16±0.01        & 75.84±0.01        & 77.15±0.03       & 76.7±0.03         & 76.32±0.02        & 75.98±0.02        \\ \hline
\textit{C13}           & \textit{C26}           & 77.03±0.01       & 76.4±0.02         & 75.83±0.02        & 75.36±0.02        & 77.01±0.02       & 76.4±0.02         & 75.85±0.01        & 75.39±0.02        & 77.06±0.01       & 76.53±0.01        & 76.04±0.02        & 75.64±0.02        \\ \hline
\end{tabular}
}
\end{table}

==> table_feature_random_autoint.tex <==
\begin{table}[]
\caption{Feature Random bags training results using AutoInt}
\label{tab:feature_rand_autoint}
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textit{\textbf{Col1}} & \textit{\textbf{Col2}} & \textbf{BCE, 64} & \textbf{BCE, 128} & \textbf{BCE, 256} & \textbf{BCE, 512} & \textbf{MSE, 64} & \textbf{MSE, 128} & \textbf{MSE, 256} & \textbf{MSE, 512} & \textbf{MAE, 64} & \textbf{MAE, 128} & \textbf{MAE, 256} & \textbf{MAE, 512} \\ \hline
\textit{C1}            & \textit{C10}           & 75.49±0.55       & 74.48±0.91        & 71.83±0.33        & 68.43±1.36        & 75.58±0.66       & 72.81±0.38        & 70.81±0.36        & 68.39±0.62        & 76.39±0.37       & 75.13±0.2         & 72.69±0.41        & 69.62±0.44        \\ \hline
\textit{C2}            & \textit{C7}            & 73.71±1.7        & 70.52±2.05        & 68.83±1.6         & 66.59±1.46        & 73.96±0.34       & 72.42±0.53        & 68.37±2.13        & 67.38±1.2         & 74.97±0.41       & 72.89±0.56        & 70.79±1.38        & 68.62±1.21        \\ \hline
\textit{C2}            & \textit{C10}           & 75.12±0.6        & 73.08±0.91        & 71.27±0.16        & 68.74±0.9         & 75.19±0.26       & 73.35±0.29        & 70.6±0.89         & 68.61±0.47        & 75.59±0.39       & 72.71±0.73        & 71.55±1.05        & 69.79±0.6         \\ \hline
\textit{C2}            & \textit{C11}           & 74.91±0.2        & 72.92±0.34        & 69.78±1.34        & 68.44±0.65        & 74.68±0.39       & 72.71±0.4         & 70.49±0.82        & 68.35±0.42        & 75.06±0.4        & 73.21±0.5         & 71.17±0.56        & 69.34±0.86        \\ \hline
\textit{C2}            & \textit{C13}           & 73.53±1.41       & 72.39±0.54        & 70.55±0.15        & 68.12±1.02        & 74.19±0.55       & 70.98±1.45        & 69.73±1.33        & 68.38±0.18        & 73.82±1.4        & 73.1±0.11         & 71.29±0.29        & 68.85±0.85        \\ \hline
\textit{C3}            & \textit{C7}            & 76.13±0.07       & 74.16±0.52        & 71.6±0.9          & 69.56±1.05        & 76.19±0.09       & 74.06±0.63        & 72.22±1.45        & 70.06±0.33        & 76.15±0.58       & 74.03±1.38        & 73.19±0.46        & 71.27±0.47        \\ \hline
\textit{C3}            & \textit{C10}           & 75.48±0.69       & 73.38±0.92        & 71.3±1.19         & 69.57±0.78        & 75.71±0.62       & 72.75±1.41        & 70.97±0.55        & 68.5±0.77         & 76.63±0.14       & 73.8±0.69         & 72.3±0.98         & 70.32±0.95        \\ \hline
\textit{C3}            & \textit{C11}           & 75.42±0.8        & 74.62±0.22        & 72.32±0.42        & 70.23±0.33        & 75.75±0.86       & 74.59±0.43        & 71.89±1.11        & 69.97±0.9         & 76.51±0.05       & 74.94±0.54        & 73.0±0.6          & 70.12±1.57        \\ \hline
\textit{C3}            & \textit{C13}           & 76.19±0.12       & 74.2±0.54         & 71.66±1.52        & 70.39±0.65        & 76.36±0.1        & 74.67±0.07        & 72.74±0.41        & 70.56±0.34        & 76.05±0.74       & 75.18±0.16        & 73.14±1.12        & 71.39±0.6         \\ \hline
\textit{C4}            & \textit{C7}            & 75.91±0.24       & 73.97±0.62        & 71.98±0.67        & 70.37±0.39        & 75.89±0.24       & 74.39±0.58        & 71.55±1.55        & 69.77±1.16        & 76.34±0.11       & 74.78±0.79        & 72.32±1.02        & 71.42±0.65        \\ \hline
\textit{C4}            & \textit{C10}           & 76.57±0.16       & 74.54±0.63        & 72.36±0.97        & 68.93±1.13        & 76.44±0.1        & 74.35±0.93        & 72.38±0.25        & 69.46±0.64        & 76.43±0.29       & 74.92±0.58        & 72.99±0.99        & 71.51±0.77        \\ \hline
\textit{C4}            & \textit{C11}           & 75.84±0.14       & 74.33±0.38        & 72.24±0.48        & 70.28±0.65        & 76.09±0.15       & 74.21±0.35        & 72.53±0.61        & 70.54±0.57        & 76.01±0.49       & 74.13±0.85        & 72.83±1.03        & 71.62±0.74        \\ \hline
\textit{C4}            & \textit{C13}           & 75.91±0.26       & 74.0±1.0          & 71.37±0.79        & 69.61±1.26        & 76.01±0.53       & 74.25±0.6         & 72.2±0.93         & 71.02±0.32        & 75.81±0.95       & 75.14±0.47        & 72.72±1.08        & 71.44±0.77        \\ \hline
\textit{C4}            & \textit{C15}           & 73.28±0.83       & 71.82±0.34        & 70.29±0.36        & 68.5±0.49         & 73.77±0.19       & 71.44±0.68        & 69.37±0.48        & 67.51±0.41        & 74.57±0.37       & 72.61±0.35        & 70.92±0.46        & 69.56±0.65        \\ \hline
\textit{C6}            & \textit{C7}            & 75.81±0.1        & 73.46±0.25        & 69.8±2.64         & 67.14±1.14        & 75.27±0.16       & 71.61±2.53        & 70.39±0.11        & 66.92±1.42        & 75.22±1.05       & 72.47±1.95        & 69.44±1.38        & 68.34±1.42        \\ \hline
\textit{C6}            & \textit{C10}           & 75.74±1.07       & 73.73±1.09        & 71.08±0.92        & 69.33±0.48        & 75.78±0.32       & 73.36±0.36        & 70.51±0.78        & 68.22±0.7         & 76.33±0.09       & 74.2±1.08         & 72.65±0.45        & 70.1±0.38         \\ \hline
\textit{C7}            & \textit{C8}            & 75.97±0.22       & 73.79±0.17        & 70.06±1.51        & 64.48±1.77        & 75.59±0.26       & 71.54±2.76        & 70.33±0.56        & 67.42±0.73        & 75.45±0.29       & 72.75±2.57        & 68.75±2.82        & 68.82±0.57        \\ \hline
\textit{C7}            & \textit{C10}           & 73.91±1.29       & 72.02±2.62        & 68.57±2.84        & 65.91±2.53        & 74.76±0.76       & 71.79±2.71        & 69.96±0.29        & 65.35±2.37        & 75.68±0.14       & 71.72±1.77        & 69.54±3.39        & 67.54±2.51        \\ \hline
\textit{C7}            & \textit{C12}           & 75.45±0.37       & 73.25±1.12        & 71.39±1.3         & 69.35±1.46        & 75.52±0.4        & 72.25±0.81        & 70.5±1.8          & 69.27±1.1         & 75.12±0.84       & 73.79±1.35        & 71.23±1.14        & 70.12±1.42        \\ \hline
\textit{C7}            & \textit{C14}           & 73.26±2.73       & 71.65±3.12        & 67.89±2.71        & 68.08±1.86        & 74.93±0.23       & 68.97±3.42        & 67.07±2.8         & 67.14±1.95        & 74.25±1.3        & 71.34±2.8         & 68.81±3.0         & 67.88±1.6         \\ \hline
\textit{C7}            & \textit{C15}           & 74.74±0.38       & 73.35±0.36        & 70.48±0.74        & 68.56±1.22        & 74.99±0.33       & 73.37±0.18        & 70.63±0.59        & 69.37±0.66        & 74.73±0.73       & 73.42±0.99        & 71.41±0.98        & 68.6±0.98         \\ \hline
\textit{C7}            & \textit{C16}           & 75.9±0.28        & 73.46±0.78        & 72.14±0.76        & 69.95±0.87        & 75.88±0.3        & 73.86±0.56        & 71.02±0.5         & 69.08±1.27        & 75.26±0.73       & 73.94±1.08        & 72.5±1.24         & 70.87±1.51        \\ \hline
\textit{C7}            & \textit{C18}           & 75.21±0.13       & 70.95±1.27        & 70.46±0.98        & 68.84±0.88        & 75.29±0.12       & 72.52±0.44        & 70.47±0.49        & 69.73±0.57        & 74.42±1.31       & 73.53±0.91        & 71.72±0.18        & 69.49±0.61        \\ \hline
\textit{C7}            & \textit{C20}           & 75.03±0.2        & 72.22±1.31        & 70.25±1.42        & 67.73±1.46        & 74.02±0.71       & 72.53±0.23        & 68.16±2.62        & 68.14±0.24        & 75.05±0.69       & 73.36±0.56        & 71.36±0.6         & 69.48±0.31        \\ \hline
\textit{C7}            & \textit{C21}           & 75.66±0.61       & 73.81±0.92        & 71.76±1.92        & 69.57±1.41        & 76.16±0.2        & 74.66±0.23        & 72.12±0.84        & 69.63±1.27        & 76.18±0.4        & 74.04±1.13        & 72.94±1.13        & 71.52±0.69        \\ \hline
\textit{C7}            & \textit{C24}           & 74.6±0.53        & 73.3±0.45         & 70.38±1.77        & 68.51±1.16        & 74.96±0.35       & 73.22±0.54        & 70.88±1.37        & 69.03±1.29        & 75.65±0.15       & 72.93±1.05        & 70.9±0.9          & 70.64±1.39        \\ \hline
\textit{C7}            & \textit{C26}           & 75.57±0.4        & 73.79±0.16        & 71.55±0.45        & 69.98±0.31        & 75.74±0.1        & 72.81±2.11        & 71.66±0.2         & 69.52±0.44        & 75.77±0.71       & 74.11±0.9         & 72.37±0.47        & 70.79±0.42        \\ \hline
\textit{C10}           & \textit{C12}           & 76.14±0.11       & 73.71±1.08        & 72.17±0.94        & 69.49±0.99        & 76.06±0.22       & 74.47±0.36        & 71.53±1.03        & 68.82±0.83        & 76.24±0.68       & 75.04±0.39        & 72.97±1.2         & 71.04±0.99        \\ \hline
\textit{C10}           & \textit{C14}           & 75.04±0.82       & 73.07±1.14        & 69.89±1.1         & 69.0±0.95         & 75.73±0.36       & 73.48±1.05        & 69.64±0.96        & 68.42±0.88        & 75.78±0.83       & 73.99±1.01        & 72.93±0.18        & 69.61±0.77        \\ \hline
\textit{C10}           & \textit{C15}           & 75.48±0.2        & 73.37±0.47        & 69.11±1.48        & 68.71±0.93        & 75.18±0.1        & 73.26±0.57        & 71.17±0.45        & 68.88±0.7         & 75.57±0.22       & 73.68±1.12        & 71.74±1.2         & 69.34±1.0         \\ \hline
\textit{C10}           & \textit{C16}           & 76.21±0.2        & 74.38±0.29        & 71.69±0.54        & 69.5±0.23         & 76.15±0.16       & 73.71±0.71        & 71.87±0.55        & 69.02±0.68        & 76.44±0.21       & 74.91±0.7         & 72.77±1.15        & 71.45±0.32        \\ \hline
\textit{C10}           & \textit{C17}           & 75.0±1.37        & 71.64±2.23        & 67.86±1.88        & 64.24±2.35        & 73.15±1.53       & 71.53±1.57        & 69.15±1.95        & 66.85±2.28        & 74.44±1.25       & 72.57±1.69        & 71.75±1.61        & 67.68±1.72        \\ \hline
\textit{C10}           & \textit{C18}           & 74.99±0.46       & 73.16±0.49        & 69.71±1.38        & 69.21±0.23        & 74.84±0.2        & 72.79±0.65        & 70.15±0.79        & 68.53±0.52        & 75.6±0.13        & 73.58±0.73        & 71.93±1.16        & 69.1±0.85         \\ \hline
\textit{C10}           & \textit{C20}           & 75.83±0.96       & 74.2±0.64         & 70.92±0.81        & 68.38±0.55        & 76.03±0.11       & 72.9±1.13         & 69.99±0.37        & 68.61±0.7         & 75.98±0.44       & 74.39±0.7         & 72.13±1.09        & 70.27±0.91        \\ \hline
\textit{C10}           & \textit{C21}           & 76.45±0.06       & 74.64±0.46        & 72.19±1.05        & 69.92±0.6         & 76.42±0.15       & 74.42±0.61        & 71.95±0.6         & 69.42±0.64        & 76.51±0.23       & 74.48±1.0         & 73.11±0.71        & 71.02±0.89        \\ \hline
\textit{C10}           & \textit{C24}           & 76.24±0.04       & 74.09±0.79        & 71.82±0.71        & 69.76±0.6         & 75.9±0.34        & 74.46±0.26        & 71.76±0.9         & 69.22±0.3         & 76.09±0.55       & 74.87±1.01        & 72.59±1.01        & 70.61±1.0         \\ \hline
\textit{C10}           & \textit{C26}           & 75.25±1.17       & 73.23±1.51        & 71.47±1.41        & 69.72±0.8         & 75.07±0.96       & 73.68±1.11        & 69.99±1.12        & 69.42±0.8         & 75.62±0.4        & 73.61±1.34        & 71.95±1.5         & 69.47±1.41        \\ \hline
\textit{C11}           & \textit{C12}           & 75.97±0.69       & 74.12±1.23        & 72.89±0.64        & 69.78±1.14        & 75.79±0.53       & 73.74±1.06        & 71.86±1.26        & 70.34±0.46        & 75.81±0.92       & 74.5±0.96         & 72.34±1.36        & 71.15±1.05        \\ \hline
\textit{C11}           & \textit{C15}           & 74.33±0.59       & 72.0±0.6          & 71.33±0.4         & 67.37±0.65        & 75.05±0.24       & 71.73±0.13        & 69.65±1.52        & 68.83±0.41        & 74.82±0.71       & 71.7±0.47         & 70.37±0.96        & 68.95±1.43        \\ \hline
\textit{C11}           & \textit{C16}           & 75.66±0.4        & 74.16±0.49        & 71.54±1.3         & 69.89±0.66        & 76.14±0.11       & 74.66±0.37        & 71.97±0.84        & 69.76±0.67        & 76.21±0.55       & 73.21±0.9         & 72.16±0.96        & 70.78±1.17        \\ \hline
\textit{C11}           & \textit{C18}           & 74.94±0.38       & 72.78±0.54        & 69.53±1.79        & 68.93±0.45        & 74.7±0.24        & 72.5±0.59         & 70.38±0.4         & 68.58±0.69        & 75.11±0.69       & 73.39±0.86        & 70.99±1.3         & 70.03±0.18        \\ \hline
\textit{C11}           & \textit{C21}           & 76.06±0.18       & 73.85±0.58        & 72.06±0.58        & 70.07±1.01        & 76.07±0.42       & 74.44±0.51        & 71.65±0.7         & 70.8±0.45         & 75.4±0.74        & 73.77±1.08        & 73.25±0.36        & 71.59±0.43        \\ \hline
\textit{C11}           & \textit{C24}           & 74.44±0.56       & 73.77±0.55        & 71.22±1.09        & 69.46±0.69        & 75.25±0.32       & 73.35±0.6         & 71.51±0.64        & 69.83±0.4         & 74.81±1.16       & 74.0±0.79         & 72.74±0.3         & 70.47±1.1         \\ \hline
\textit{C11}           & \textit{C26}           & 75.42±0.45       & 73.63±0.78        & 70.14±2.01        & 69.47±1.29        & 75.21±0.37       & 73.39±0.55        & 70.63±1.56        & 69.45±0.58        & 75.82±0.19       & 74.52±0.33        & 72.76±0.42        & 70.11±0.86        \\ \hline
\textit{C12}           & \textit{C13}           & 74.96±1.21       & 72.87±1.33        & 71.32±1.18        & 69.83±0.82        & 75.55±0.93       & 73.72±1.29        & 71.55±1.35        & 70.02±0.72        & 75.38±0.85       & 75.27±0.07        & 71.35±0.94        & 70.66±0.68        \\ \hline
\textit{C13}           & \textit{C15}           & 74.01±1.15       & 71.37±0.68        & 70.13±0.79        & 68.27±1.22        & 74.01±1.0        & 71.45±1.15        & 70.8±0.56         & 68.22±0.85        & 73.82±0.95       & 72.18±1.39        & 70.05±1.24        & 69.23±1.28        \\ \hline
\textit{C13}           & \textit{C16}           & 75.35±0.89       & 73.52±0.3         & 72.02±0.99        & 69.22±1.2         & 75.67±0.69       & 74.08±0.55        & 72.32±0.53        & 70.69±0.39        & 75.81±0.73       & 74.11±1.29        & 71.9±1.36         & 70.93±1.14        \\ \hline
\textit{C13}           & \textit{C18}           & 74.14±0.57       & 72.19±1.25        & 70.44±0.82        & 68.38±0.73        & 74.51±0.47       & 72.74±0.56        & 70.38±0.81        & 68.58±0.51        & 74.37±0.45       & 72.79±0.75        & 70.32±1.47        & 69.6±1.15         \\ \hline
\textit{C13}           & \textit{C21}           & 75.07±0.73       & 74.02±0.73        & 72.64±0.34        & 69.45±1.15        & 76.08±0.12       & 74.29±0.76        & 71.94±1.06        & 70.14±0.78        & 75.24±0.86       & 74.56±0.6         & 71.88±1.09        & 71.47±0.71        \\ \hline
\textit{C13}           & \textit{C24}           & 75.37±0.29       & 74.09±0.48        & 71.74±0.79        & 69.68±0.84        & 75.61±0.19       & 73.59±0.72        & 72.17±0.26        & 69.63±0.71        & 75.56±0.85       & 73.86±1.06        & 72.95±0.29        & 70.5±0.47         \\ \hline
\textit{C13}           & \textit{C26}           & 75.59±0.31       & 73.8±0.12         & 71.66±0.42        & 69.49±0.69        & 75.56±0.2        & 73.52±0.44        & 71.17±0.44        & 69.29±0.74        & 76.06±0.06       & 74.56±0.28        & 72.57±0.52        & 71.13±0.26        \\ \hline
\end{tabular}
}
\end{table}

==> table_feature_random_autoint_llp_bench.tex <==
\begin{table*}[]
\caption{AUC scores of AutoInt on fixed size bags for LLP-Bench}
\label{tab:feature_rand_autoint_llp_bench}
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|l|llll|llll|llll|}
\hline
{\textit{\textbf{Col1}}} & {\textit{\textbf{Col2}}} & \multicolumn{4}{c|}{\textbf{BCE}}                                                                                                            & \multicolumn{4}{c|}{\textbf{MSE}}                                                                                                            & \multicolumn{4}{c|}{\textbf{MAE}}                                                                                                            \\ \cline{3-14} 
                                        &                                         & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{\textbf{128}} & \multicolumn{1}{c|}{\textbf{256}} & \multicolumn{1}{c|}{\textbf{512}} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{\textbf{128}} & \multicolumn{1}{c|}{\textbf{256}} & \multicolumn{1}{c|}{\textbf{512}} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{\textbf{128}} & \multicolumn{1}{c|}{\textbf{256}} & \multicolumn{1}{c|}{\textbf{512}} \\ \hline
\textit{C1}                             & \textit{C10}                            & \multicolumn{1}{l|}{75.49±0.55}  & \multicolumn{1}{l|}{74.48±0.91}   & \multicolumn{1}{l|}{71.83±0.33}   & 68.43±1.36                        & \multicolumn{1}{l|}{75.58±0.66}  & \multicolumn{1}{l|}{72.81±0.38}   & \multicolumn{1}{l|}{70.81±0.36}   & 68.39±0.62                        & \multicolumn{1}{l|}{76.39±0.37}  & \multicolumn{1}{l|}{75.13±0.2}    & \multicolumn{1}{l|}{72.69±0.41}   & 69.62±0.44                        \\ \hline
\textit{C2}                             & \textit{C13}                            & \multicolumn{1}{l|}{73.53±1.41}  & \multicolumn{1}{l|}{72.39±0.54}   & \multicolumn{1}{l|}{70.55±0.15}   & 68.12±1.02                        & \multicolumn{1}{l|}{74.19±0.55}  & \multicolumn{1}{l|}{70.98±1.45}   & \multicolumn{1}{l|}{69.73±1.33}   & 68.38±0.18                        & \multicolumn{1}{l|}{73.82±1.4}   & \multicolumn{1}{l|}{73.1±0.11}    & \multicolumn{1}{l|}{71.29±0.29}   & 68.85±0.85                        \\ \hline
\textit{C6}                             & \textit{C10}                            & \multicolumn{1}{l|}{75.74±1.07}  & \multicolumn{1}{l|}{73.73±1.09}   & \multicolumn{1}{l|}{71.08±0.92}   & 69.33±0.48                        & \multicolumn{1}{l|}{75.78±0.32}  & \multicolumn{1}{l|}{73.36±0.36}   & \multicolumn{1}{l|}{70.51±0.78}   & 68.22±0.7                         & \multicolumn{1}{l|}{76.33±0.09}  & \multicolumn{1}{l|}{74.2±1.08}    & \multicolumn{1}{l|}{72.65±0.45}   & 70.1±0.38                         \\ \hline
\textit{C7}                             & \textit{C10}                            & \multicolumn{1}{l|}{73.91±1.29}  & \multicolumn{1}{l|}{72.02±2.62}   & \multicolumn{1}{l|}{68.57±2.84}   & 65.91±2.53                        & \multicolumn{1}{l|}{74.76±0.76}  & \multicolumn{1}{l|}{71.79±2.71}   & \multicolumn{1}{l|}{69.96±0.29}   & 65.35±2.37                        & \multicolumn{1}{l|}{75.68±0.14}  & \multicolumn{1}{l|}{71.72±1.77}   & \multicolumn{1}{l|}{69.54±3.39}   & 67.54±2.51                        \\ \hline
\textit{C7}                             & \textit{C20}                            & \multicolumn{1}{l|}{75.03±0.2}   & \multicolumn{1}{l|}{72.22±1.31}   & \multicolumn{1}{l|}{70.25±1.42}   & 67.73±1.46                        & \multicolumn{1}{l|}{74.02±0.71}  & \multicolumn{1}{l|}{72.53±0.23}   & \multicolumn{1}{l|}{68.16±2.62}   & 68.14±0.24                        & \multicolumn{1}{l|}{75.05±0.69}  & \multicolumn{1}{l|}{73.36±0.56}   & \multicolumn{1}{l|}{71.36±0.6}    & 69.48±0.31                        \\ \hline
\textit{C7}                             & \textit{C21}                            & \multicolumn{1}{l|}{75.66±0.61}  & \multicolumn{1}{l|}{73.81±0.92}   & \multicolumn{1}{l|}{71.76±1.92}   & 69.57±1.41                        & \multicolumn{1}{l|}{76.16±0.2}   & \multicolumn{1}{l|}{74.66±0.23}   & \multicolumn{1}{l|}{72.12±0.84}   & 69.63±1.27                        & \multicolumn{1}{l|}{76.18±0.4}   & \multicolumn{1}{l|}{74.04±1.13}   & \multicolumn{1}{l|}{72.94±1.13}   & 71.52±0.69                        \\ \hline
\textit{C10}                            & \textit{C15}                            & \multicolumn{1}{l|}{75.48±0.2}   & \multicolumn{1}{l|}{73.37±0.47}   & \multicolumn{1}{l|}{69.11±1.48}   & 68.71±0.93                        & \multicolumn{1}{l|}{75.18±0.1}   & \multicolumn{1}{l|}{73.26±0.57}   & \multicolumn{1}{l|}{71.17±0.45}   & 68.88±0.7                         & \multicolumn{1}{l|}{75.57±0.22}  & \multicolumn{1}{l|}{73.68±1.12}   & \multicolumn{1}{l|}{71.74±1.2}    & 69.34±1.0                         \\ \hline
\end{tabular}
}
\end{table*}

==> table_feature_random_mlp_llp_bench.tex <==
\begin{table*}[]
\caption{AUC scores of 2-Layer MLP on fixed size bags for LLP-Bench}
\label{tab:feature_rand_mlp_llp_bench}
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|l|llll|llll|llll|}
\hline
{\textit{\textbf{Col1}}} & {\textit{\textbf{Col2}}} & \multicolumn{4}{c|}{\textbf{BCE}}                                                                                                            & \multicolumn{4}{c|}{\textbf{MSE}}                                                                                                            & \multicolumn{4}{c|}{\textbf{MAE}}                                                                                                            \\ \cline{3-14} 
                                        &                                         & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{\textbf{128}} & \multicolumn{1}{c|}{\textbf{256}} & \multicolumn{1}{c|}{\textbf{512}} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{\textbf{128}} & \multicolumn{1}{c|}{\textbf{256}} & \multicolumn{1}{c|}{\textbf{512}} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{\textbf{128}} & \multicolumn{1}{c|}{\textbf{256}} & \multicolumn{1}{c|}{\textbf{512}} \\ \hline
\textit{C1}                             & \textit{C10}                            & \multicolumn{1}{l|}{77.11±0.01}  & \multicolumn{1}{l|}{76.3±0.02}    & \multicolumn{1}{l|}{75.25±0.02}   & 74.1±0.03                         & \multicolumn{1}{l|}{77.06±0.03}  & \multicolumn{1}{l|}{76.3±0.02}    & \multicolumn{1}{l|}{75.28±0.02}   & 74.14±0.04                        & \multicolumn{1}{l|}{76.87±0.03}  & \multicolumn{1}{l|}{76.12±0.03}   & \multicolumn{1}{l|}{75.16±0.02}   & 74.14±0.06                        \\ \hline
\textit{C2}                             & \textit{C13}                            & \multicolumn{1}{l|}{76.74±0.03}  & \multicolumn{1}{l|}{76.11±0.02}   & \multicolumn{1}{l|}{75.58±0.01}   & 75.18±0.02                        & \multicolumn{1}{l|}{76.74±0.02}  & \multicolumn{1}{l|}{76.12±0.02}   & \multicolumn{1}{l|}{75.59±0.02}   & 75.19±0.01                        & \multicolumn{1}{l|}{76.7±0.02}   & \multicolumn{1}{l|}{76.13±0.03}   & \multicolumn{1}{l|}{75.64±0.03}   & 75.25±0.02                        \\ \hline
\textit{C6}                             & \textit{C10}                            & \multicolumn{1}{l|}{76.82±0.04}  & \multicolumn{1}{l|}{75.94±0.03}   & \multicolumn{1}{l|}{74.95±0.02}   & 73.98±0.01                        & \multicolumn{1}{l|}{76.8±0.03}   & \multicolumn{1}{l|}{75.94±0.03}   & \multicolumn{1}{l|}{74.96±0.02}   & 73.99±0.02                        & \multicolumn{1}{l|}{76.67±0.02}  & \multicolumn{1}{l|}{75.89±0.02}   & \multicolumn{1}{l|}{75.01±0.03}   & 74.12±0.01                        \\ \hline
\textit{C7}                             & \textit{C10}                            & \multicolumn{1}{l|}{76.41±0.03}  & \multicolumn{1}{l|}{75.43±0.03}   & \multicolumn{1}{l|}{74.51±0.03}   & 73.78±0.02                        & \multicolumn{1}{l|}{76.42±0.02}  & \multicolumn{1}{l|}{75.45±0.03}   & \multicolumn{1}{l|}{74.51±0.02}   & 73.78±0.03                        & \multicolumn{1}{l|}{76.38±0.03}  & \multicolumn{1}{l|}{75.54±0.03}   & \multicolumn{1}{l|}{74.8±0.02}    & 74.14±0.01                        \\ \hline
\textit{C7}                             & \textit{C20}                            & \multicolumn{1}{l|}{76.79±0.03}  & \multicolumn{1}{l|}{76.09±0.04}   & \multicolumn{1}{l|}{75.44±0.03}   & 74.96±0.03                        & \multicolumn{1}{l|}{76.79±0.03}  & \multicolumn{1}{l|}{76.1±0.04}    & \multicolumn{1}{l|}{75.47±0.04}   & 74.99±0.04                        & \multicolumn{1}{l|}{76.73±0.03}  & \multicolumn{1}{l|}{76.14±0.03}   & \multicolumn{1}{l|}{75.59±0.03}   & 75.19±0.04                        \\ \hline
\textit{C7}                             & \textit{C21}                            & \multicolumn{1}{l|}{77.33±0.02}  & \multicolumn{1}{l|}{76.82±0.02}   & \multicolumn{1}{l|}{76.36±0.03}   & 75.96±0.02                        & \multicolumn{1}{l|}{77.32±0.02}  & \multicolumn{1}{l|}{76.83±0.02}   & \multicolumn{1}{l|}{76.38±0.04}   & 75.97±0.03                        & \multicolumn{1}{l|}{77.36±0.02}  & \multicolumn{1}{l|}{76.95±0.03}   & \multicolumn{1}{l|}{76.54±0.02}   & 76.15±0.01                        \\ \hline
\textit{C10}                            & \textit{C15}                            & \multicolumn{1}{l|}{76.93±0.03}  & \multicolumn{1}{l|}{76.36±0.02}   & \multicolumn{1}{l|}{75.94±0.03}   & 75.59±0.02                        & \multicolumn{1}{l|}{76.85±0.03}  & \multicolumn{1}{l|}{76.3±0.02}    & \multicolumn{1}{l|}{75.88±0.03}   & 75.58±0.03                        & \multicolumn{1}{l|}{76.94±0.02}  & \multicolumn{1}{l|}{76.51±0.03}   & \multicolumn{1}{l|}{76.16±0.02}   & 75.83±0.04                        \\ \hline
\end{tabular}
}
\end{table*}

==> table_flagship_groupings.tex <==
\begin{table*}[]

\normalsize
\centering
\caption{\small LLP-Bench Groupings. Bold : Analyzed for model training.}
\label{tab:flagship_stats_and_clusters}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Col1}         & \textbf{Col2}         & \textbf{\begin{tabular}[c]{@{}l@{}}No. Bags\\ After\\ Clipping\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Percentage\\ Inst. After\\ Clipping\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Mean\\ Bag Size\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Bag Distribution\\ Clusters\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Label Prop Dist.\\ Clsuters\end{tabular}} & \textbf{Inter/Intra Ratio Clusters} \\ \hline
\textit{C5}           & \textit{C8}           & 2486                                                                         & 1.44                                                                                & 265.84                                                          & \textit{Very Short-tailed}                                                   & \textit{High}                                                         & \textit{Less-separated}      \\ \hline
\textit{\textbf{C1}}  & \textit{\textbf{C10}} & \textbf{55528}                                                               & \textbf{32.44}                                                                       & \textbf{267.81}                                                 & \textit{\textbf{Very Short-tailed}}                                          & \textit{\textbf{High}}                                                & \textit{\textbf{Medium-separated}}  \\ \hline
\textit{C19}          & \textit{C22}          & 3893                                                                         & 3.69                                                                                & 434.23                                                          & \textit{Long-tailed}                                                         & \textit{High}                                                         & \textit{Less-separated}      \\ \hline
\textit{\textbf{C6}}  & \textit{\textbf{C10}} & \textbf{46981}                                                               & \textbf{31.8}                                                                      & \textbf{310.24}                                                 & \textit{\textbf{Short-tailed}}                                               & \textit{\textbf{Medium}}                                                     & \textit{\textbf{Medium-separated}}  \\ \hline
\textit{\textbf{C2}}  & \textit{\textbf{C13}} & \textbf{45206}                                                               & \textbf{34.87}                                                                       & \textbf{353.59}                                                 & \textit{\textbf{Short-tailed}}                                               & \textit{\textbf{Low}}                                               & \textit{\textbf{Medium-Separated}}  \\ \hline
\textit{\textbf{C7}}  & \textit{\textbf{C10}} & \textbf{56575}                                                               & \textbf{40.52}                                                                      & \textbf{328.31}                                                 & \textit{\textbf{Short-tailed}}                                               & \textit{\textbf{Medium}}                                                     & \textit{\textbf{Far-separated}}    \\ \hline
\textit{\textbf{C10}} & \textit{\textbf{C15}} & \textbf{102841}                                                              & \textbf{44.66}                                                                       & \textbf{199.07}                                                  & \textit{\textbf{Very Short-tailed}}                                          & \textit{\textbf{Medium}}                                                     & \textit{\textbf{Well-separated}}         \\ \hline
\textit{\textbf{C7}}  & \textit{\textbf{C21}} & \textbf{88970}                                                               & \textbf{40.43}                                                                      & \textbf{208.31}                                                 & \textit{\textbf{Very Short-tailed}}                                          & \textit{\textbf{Low}}                                               & \textit{\textbf{Far-separated}}    \\ \hline
\textit{C13}          & \textit{-}            & 1221                                                                         & 2.98                                                                                & 1120.01                                                         & \textit{Very Long-tailed}                                                    & \textit{Very Low}                                                   & \textit{Less-separated}      \\ \hline
\textit{C9}           & \textit{C19}          & 2214                                                                         & 2.6                                                                                & 538.05                                                          & \textit{Long-tailed}                                                         & \textit{Medium}                                                              & \textit{Far-separated}             \\ \hline
\textit{C9}           & \textit{C11}          & 3221                                                                         & 5.71                                                                                & 812.21                                                          & \textit{Very Long-tailed}                                                    & \textit{Very Low}                                                   & \textit{Far-separated}             \\ \hline
\textit{\textbf{C7}}  & \textit{\textbf{C20}} & \textbf{30420}                                                               & \textbf{31.85}                                                                       & \textbf{479.96}                                                 & \textit{\textbf{Long-tailed}}                                                & \textit{\textbf{Low}}                                               & \textit{\textbf{Well-separated}}         \\ \hline
\end{tabular}
\end{table*}

==> table_mean_bag_size_percentile.tex <==
\begin{table*}[]
\normalsize
\centering
\caption{\small Mean bag sizes at which groupings achieve respective percentile in each cluster}
\label{tab:mean_bag_size_percentile}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Bag Size Cluster} & \textbf{\begin{tabular}[c]{@{}l@{}}\# Groupings\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Mean bag size:\\ 50 Percentile\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Mean bag size:\\ 70 Percentile\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Mean bag size:\\ 85 Percentile\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Mean bag size:\\ 95 Percentile\end{tabular}} \\ \hline
\textit{Very Short-tailed} & 171 & 107.77 & 189.05 & 375.94 & 905.66 \\ \hline
\textit{Short-tailed} & 82 & 155.40 & 314.83 & 672.02 & 1434.77 \\ \hline
\textit{Long-tailed} & 41 & 269.22 & 571.24 & 1094.90 & 1831.78 \\ \hline
\textit{Very Long-tailed} & 14 & 590.79 & 1053 & 1599.57 & 2145.93 \\ \hline
\end{tabular}
\end{table*}

==> table_ratio_ranges.tex <==
\begin{table}
\caption{\small Clustering on ${\sf InterIntraRatio}$.}
\normalsize
\centering
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Cluster} & \textbf{\begin{tabular}[c]{@{}l@{}}\# Groupings\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Min\\ Ratio\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Max\\ Ratio\end{tabular}} \\ \hline
\textit{Less-separated} & 37 & 1.02 & 1.10 \\ \hline
\textit{Medium-separated} & 196 & 1.12 & 1.24 \\ \hline
\textit{Well-separated} & 58 & 1.25 & 1.40 \\ \hline
\textit{Far-separated} & 17 & 1.41 & 1.56 \\ \hline
\end{tabular}
\label{tab:ratio_ranges}
\end{table}
